Modeling the spread of infectious disease in urban areas with travel contagion

In this study, we develop the mathematical model to understand the coupling between the spreading dynamics of infectious diseases and the mobility dynamics through urban transportation systems. We first describe the mobility dynamics of the urban population as the process of leaving from home, traveling to and from the activity locations, and engaging in activities. We then embed the susceptible-exposed-infectious-recovered (SEIR) process over the mobility dynamics and develops the spatial SEIR model with travel contagion (Trans-SEIR), which explicitly accounts for contagions both during travel and during daily activities. We investigate the theoretical properties of the proposed model and show how activity contagion and travel contagion contribute to the average number of secondary infections. In the numerical experiments, we explore how the urban transportation system may alter the fundamental dynamics of the infectious disease, change the number of secondary infections, promote the synchronization of the disease across the city, and affect the peak of the disease outbreaks. The Trans-SEIR model is further applied to the understand the disease dynamics during the COVID-19 outbreak in New York City, where we show how the activity and travel contagion may be distributed and how effective travel control can be implemented with only limited resources. The Trans-SEIR model along with the findings in our study may have significant contributions to improving our understanding of the coupling between urban transportation and disease dynamics, the development of quarantine and control measures of disease system, and promoting the idea of disease-resilient urban transportation networks.

==> method.tex <==
\section{Modeling disease spreading with travel contagion}
\subsection{The basic model}
\subsubsection{Notation}
We summarize the list of variables used in this section as follows
\begin{table}[htbp!]
	\setstretch{1.2}
	\centering
	\caption{Table of notation}
	\label{notation}
	\begin{tabular}{p{2cm}p{13.5cm}}
		\hline
		Notation & Description \\ \hline
		&\textbf{Variables}\\ \hline
		$S_{ij}$ & Susceptible population who are residents of patch $i$ and currently in patch $j$. \\
		$E_{ij}$ & Exposed (latent) population who are residents of patch $i$ and currently in patch $j$.\\
		$I_{ij}$ & Infected population who are residents of patch $i$ and currently in patch $j$. \\
		$R_{ij}$ & Recovered population who are residents of patch $i$ and currently in patch $j$.\\
		$t_{ij}^m$ & Induced travel time for moving from patch $i$ to patch $j$ using mode $m$. \\
		$N_i^p$ & Population at patch $i$. \\
		$N_{ij}$ & The amount of people currently at patch $j$ who are the residents of patch $i$. \\
		\hline
		&\textbf{Fixed parameters}\\ \hline
        $M$ & Total number of travel modes available. \\
        $m$ & Travel mode $m$, where $m=1,2,...,M$. \\
		$\beta_{inn}$ & Within zone disease transmission rate. \\
		$\beta_{tra}^m$ & Disease transmission rate for travel mode $m$. \\ 
		$c_{ij}^m$ & The ratio of people who choose travel mode $m$ between patch $i$ and patch $j$. \\
		$d_l^m$ & Rate of remaining infected people for travel mode $m$ at control level $l$. \\
		 \hline
	\end{tabular}
\end{table}

\subsubsection{System dynamics}
An important component missing from the previously discussed SEIR model is the spatial interaction. The model only considers local dynamics, but it is essential for urban areas to model explicitly how population flow moving around the city. In particular, these flows are driven by various activities, such as work, school, or entertainment. And people get in contact with others by taking different activities through various transportation tools. As long as some individuals are infected, their activities and the urban transportation mobility will take the disease to every corner of the city. This motivates us to understand the the spread of infectious disease in urban area by modeling the system with the following 6 dynamics: 
\begin{enumerate}
\item The mobility dynamics of urban population follows the model as discussed in section 3.2.
\item Similar to the SEIR model, we consider $S_{ij}$ being affected by $I_{ij}$ with the inner-patch contagion rate $\beta_{inn}$. 
\item In addition to the spread due to within patch activities, we also consider people get infected during travel. That is, $S_{ij}$ may be infected by contacting with $I_{ij}$ if they use the same travel mode $m$, with the contagion rate of $\beta_{tra}^m$. 
\item Once people in $S_{ij}$ are infected, they become $E_{ij}$. They are not infectious until the end of the latent period, and the length of latent period is characterized by $1/\sigma$.
\item People in $E_{ij}$ become $I_{ij}$ at the end of the latent period. And the length of the infectious period is characterized by $1/\gamma$. 
\item At the end of their infectious period, people in $I_{ij}$ become $R_{ij}$. For simplicity, we consider that they gain permanent immunity to the disease and will be no longer infected.  
\end{enumerate}

In particular, the contagion process between susceptible and infected population can be illustrated by the example of a 3-patch network as shown in Figure~\ref{fig:examp}
\begin{figure}[h!]
	\centering
	\includegraphics[width=150mm]{results/contaillust.pdf}
	\caption{Illustration of the disease contagion process in a 3-patch network}
	\label{fig:examp}
\end{figure}
There are 3 patches in the network, with two travel links 1-2 and 2-3 and three possible routes: from patch 1 to patch 2, from patch 1 to patch 3, and from patch 2 to patch 3. And we have two different contagions in this network. One is the inner-patch contagion which takes place between $S$ and $I$ population in the same patch. Additionally, there is travel contagion (shown in dashed line), which may happen if two population share overlay segments in their travel routes. Consequently, we have two possible travel contagions: between people travel from 1 to 2 and 1 to 3, and between people travel from 1 to 3 and 2 to 3. While this is only an illustration, the overlay segment will be later differentiated based on the travel modes as well.


\subsubsection{Formulation}

where we have the contagion at home, at activity location and during travel as:
\begin{equation}
    f_{ij}(S,I)=\beta^{A}_j\kappa_{ij}\frac{S_{ij}\sum_{k=1}^{N}I_{kj}}{N_j^p}
\end{equation}
\begin{equation}
    f_{ii}(S,I)=\beta^{A}_i\kappa_{ii}\frac{S_{ii}\sum_{k=1}^{N}I_{ki}}{N_i^p}
\end{equation}
\begin{equation}
    h_{\la{ij}}(S,I)=\sum_{j=1,j\neq i}^P\sum_{d=1}^D c_{ij}^{d} \beta_d^T {S}_{\la{ij}} [\sum_{k=1}^P\sum_{l=1,l\neq k}^P \frac{\kappa_{\la{kl},\la{ij}}^d I_{\la{kl}}}{N_{\la{kl}}}+\frac{\kappa_{\ra{kl},\la{ij}}^d I_{\ra{kl}}}{N_{\ra{kl}}}]
    \label{eq:travel_return_infect}
\end{equation}
\begin{equation}
    h_{\ra{ij}}(S,I)=\sum_{j=1,j\neq i}^P\sum_{d=1}^D c_{ij}^{d} \beta_d^T {S}_{\ra{ij}} [\sum_{k=1}^P\sum_{l=1,l\neq k}^P \frac{\kappa_{\la{kl},\ra{ij}}^d I_{\la{kl}}}{N_{\la{kl}}}+\frac{\kappa_{\ra{kl},\ra{ij}}^d I_{\ra{kl}}}{N_{\ra{kl}}}]
    \label{eq:travel_out_infect}
\end{equation}

Equation~\ref{eq:travel_return_infect} summarizes the S population who returns to home $i$ and get infected during travel, by encountering I population to-and-from resident location in other places. Specifically, $c_{ij}^dg_im_{ij}S_{ii}$ captures the ratio of $S_{ii}$ who leaves for destination $j$ using transportation mode $d$. $\frac{\kappa_{kl,ij}^d I_{kl}}{N_{kl}}$ denotes the contact rate with infectious population returning from $l$ to $k$, which is simplified from:
\begin{equation}
    \frac{\kappa_{kl,ij}^d c_{kl}^dr_{kl} I_{kl}}{c_{kl}^dr_{kl} N_{kl}}
\end{equation}
and $\kappa_{kl,ij}^d$ refers to the number of contacts on average between ODs $kl$ and $ij$, and is a function of the travel time. Similarly, $\frac{\kappa_{kl,ij}^d I_{kk}}{N_{kk}}$ represents the contact rate with the infectious population leaving from $k$ to $l$, which is simplified from:
\begin{equation}
    \frac{\kappa_{kl,ij}^d c_{kl}^dg_km_{kl}I_{kk}}{c_{kl}^dg_km_{kl}N_{kk}}
\end{equation}
With the above four different incidences for possible disease transmission, we can formally express the mathematical formulations that describe the transportation disease spreading process in urban area as follows:
\begin{eqnarray}
\begin{aligned}
\dot{E}_{ii}=&-g_{i}E_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}E_{ij}-\sigma E_{ii}+f_{ii}(S,I)+h_{ii}(S,I)-\mu E_{ii}\\
\dot{E}_{ij}=&-r_{ij}E_{ij}+g_i m_{ij}E_{ii}-\sigma E_{ij}+f_{ij}(S,I)+h_{ij}(S,I)-\mu E_{ij}\\
\dot{I}_{ii}=&-g_{i}I_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}I_{ij}+\sigma E_{ii}-\gamma I_{ii}-\mu I_{ii}\\
\dot{I}_{ij}=&-r_{ij}I_{ij}+g_i m_{ij}I_{ii}+\sigma E_{ij}-\gamma I_{ij}-\mu I_{ij}\\
\dot{S}_{ii}=&-g_{i}S_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}S_{ij}-f_{ii}(S,I)-h_{ii}(S,I)+\mu(N_i^r-S_{ii})\\
\dot{S}_{ij}=&-r_{ij}S_{ij}+g_im_{ij}S_{ii}-f_{ij}(S,I)-h_{ij}(S,I)-\mu S_{ij}\\
\dot{R}_{ii}=&-g_{i}R_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}R_{ij}+\gamma I_{ii}-\mu R_{ii}\\
\dot{R}_{ij}=&-r_{ij}R_{ij}+g_i m_{ij}R_{ii}+\gamma I_{ij}-\mu R_{ij}
\end{aligned}
\label{eq:seir_system}
\end{eqnarray}

The system described by equation~\ref{eq:seir_system} can be easily understood by decomposing each equation into the part of mobility dynamics and the part of disease dynamics. In particular, for equations characterizing the dynamics of $S_{ii},E_{ii},I_{ii}, R_{ii}$, the first four terms on the right-hand-side (RHS) capture the mobility dynamics, which are consistent with equation~\ref{eq:st}. Similarly, the first three terms on the RHS of equations for $S_{ij},E_{ij},I_{ij}, R_{ij}$ can be analogous to equation~\ref{eq:bt}.   

% The disease dynamics of equation~\ref{eq:sii} has two components. The first component with the coefficient $\beta_{inn}$ characterizes the within patch spread of diseases, where $\sum_jI_{ji}$ refers to total infected population in patch $i$ and the contagion has the bilinear incident form which is consistent with the SEIR model. The second component which is associated with the coefficient $\beta_{tra}$ denote the spread of diseases during travel. Specifically, this term describes how susceptible people who return from $j$ to $i$ get in contact with infectious population. For the contagion to take place, $S$ and $I$ must be in the same travel mode and share trip segment(s) in common. And the indicator variable $\delta_{ki,ji}^m$ is introduced to indicate if trips made from $k$ to $i$ and from $j$ to $i$ using travel mode $m$ have overlapping parts. And the infected $S_{ii}$ are added to $E_{ii}$ as shown in equation~\ref{eq:eii}. Moreover, $E_{ii}$ and $I_{ii}$ (or equation~\ref{eq:eii} and~\ref{eq:iii}) are connected by the term $\sigma E_{ii}$, which implies the end of latent period. Similarly, $I_{ii}$ and $R_{ii}$ (or equation~\ref{eq:iii} and~\ref{eq:rii}) are correlated by the term $\gamma I_{ii}$.

% On the other hand, the disease dynamics for equation~\ref{eq:sij} also involves two components. The first component with the coefficient $\beta_{inn}$ captures how $S_{ij}$ gets infected during the contagion with other infected population. The second component with the coefficient $\beta_{tra}$ describes the spread of diseases while people are traveling from $i$ to $j$. That is, only departed population $g_jm_{ij}S_{ii}$ may have the chance of being infected during their travel to $j$. And the contagion may happen when they get in contact with departed infectious population who have the same destination using the same mode, which is captured by $\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m g_km_{kj}I_{kk}$. And both parts of infected $S_{ij}$ are added to $E_{ij}$ as shown in equation~\ref{eq:eij}. Finally, we have the same correlations between $E_{ij}$ and $I_{ij}$, and between $I_{ij}$ and $R_{ij}$, as discussed in the previous paragraph. This concludes the basic model for characterizing disease dynamics with travel contagion. 

\begin{prop}
Based on equation~\ref{eq:seir_system}, we can decompose the system into $\mathcal{F}-\mathcal{V}$ where we have
\begin{equation}
\mathcal{F}=
\begin{bmatrix}
      f_{ii}+h_{ii}\\
      f_{ij}+h_{ij}\\
      0\\
      0\\
      0\\
      0\\
      0\\
      0
\end{bmatrix}
, \mathcal{V}=
\begin{bmatrix}
    (g_{i}+\mu+\sigma)E_{ii}-\sum_{j=1,j\neq i}^{P}r_{ij}E_{ij}\\
    (r_{ij}+\mu+\sigma)E_{ij}-g_i m_{ij}E_{ii} \\
    (g_{i}+\mu+\gamma)I_{ii}-\sum_{j=1,j\neq i}^{P}r_{ij}I_{ij}-\sigma E_{ii}\\
    (r_{ij}+\mu+\gamma)I_{ij}-g_i m_{ij}I_{ii}-\sigma E_{ij}\\
    (g_{i}+\mu)S_{ii}-\sum_{j=1,j\neq i}^{P}r_{ij}S_{ij}-\mu N_i^r\\
    (r_{ij}+\mu)S_{ij}-g_i m_{ij}S_{ii} \\
    (g_{i}+\mu)R_{ii}-\sum_{j=1,j\neq i}^{P}r_{ij}R_{ij}-\gamma I_{ii}\\
    (r_{ij}+\mu)R_{ij}-g_i m_{ij}R_{ii}-\gamma I_{ij} 
    \end{bmatrix}
\end{equation}
\end{prop}




Considering that an infectious disease has been introduced, and people are aware of the disease patterns in the city. An essential question to answer is that if the disease will eventually invade the population. This requires the understanding of the stability of disease free equilibrium (DFE). In other words, if the DFE is stable, then the disease will be absent from the population, otherwise it is always possible for disease outbreak. 
 \begin{defn}
 	The disease dynamic system characterized by equation 5.1-5.8 has two equilibrium points. The first equilibrium point $x_0$ is the disease free equilibrium (DFE):
 	\begin{equation}
 	S_{ij}=N_{ij},E_{ij}=I_{ij}=R_{ij}=0
 	\end{equation}
 	\begin{equation}
 	    x_0=(0,0,N,0)
 	\end{equation}
 	The second equilibrium point is the endemic equilibrium:
 	\begin{equation}
 	\sum_{ij} S_{ij}=0
 	\end{equation}
 	such that no susceptible population available and all people are eventually infected. 
 \end{defn}
 
\subsection{Model analysis}

If we linearize the system at $x_0$, we have $D\mathcal{F}(x_0)$ as:
\begin{equation}
    D\mathcal{F}(x_0)=\begin{bmatrix}
        0 & 0 & \frac{df_{ii}(x_0)}{d I_{ii}}+\frac{dh_{ii}(x_0)}{d I_{ii}} & \frac{df_{ii}(x_0)}{d I_{ij}}+\frac{dh_{ii}(x_0)}{d I_{ij}} & 0 & 0 & 0 & 0\\
        0 & 0 &\frac{df_{ij}(x_0)}{d I_{ii}}+\frac{dh_{ij}(x_0)}{d I_{ii}} & \frac{df_{ij}(x_0)}{d I_{ij}}+\frac{dh_{ij}(x_0)}{d I_{ij}} & 0 & 0 & 0 & 0\\
        0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
        0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
    \end{bmatrix}
\end{equation}

We can further partition matrix $V$ as in the following format:
\begin{equation}
    D\mathcal{V}(x_0)=\left[\begin{array}{@{}c|c@{}}
  \begin{matrix}
  V_E^A & V_E^B \\
  V_E^C & V_E^D
  \end{matrix}
  & \bigzero \\
\hline
  -\Sigma &
  \begin{matrix}
  V_I^A & V_I^B \\
  V_I^C & V_I^D
  \end{matrix}
\end{array}\right]
\end{equation}

where $\Sigma$ represents the diagonal matrix of $\sigma$, and we have
\begin{equation}
    V^A_E=\begin{bmatrix} 
    g_1+\mu+\sigma & & \\
    & \ddots & \\ 
     & & g_n+\mu+\sigma 
    \end{bmatrix}, 
        V^D_E=\begin{bmatrix} 
    r_{12}+\mu+\sigma & & \\
    & \ddots & \\ 
     & & r_{nn-1}+\mu+\sigma 
    \end{bmatrix}
\end{equation}

\begin{equation}
    V^B_E=\begin{bmatrix} 
    r_{12},\dots,r_{1n} & & \\
     &  \ddots &\\ 
     & &  r_{n1},\dots,r_{nn-1}
    \end{bmatrix}, 
        V^{C\intercal}_E=\begin{bmatrix} 
    -g_1m_{12},\dots,-g_1m_{1n} & & \\
     & \ddots &\\ 
     & & -g_nm_{n1},\dots,-g_nm_{nn-1}
    \end{bmatrix}
\end{equation}
And similarly, for compartments of $I$ population, we have
\begin{equation}
    V^A_I=\begin{bmatrix} 
    g_1+\mu+\gamma & & \\
    & \ddots & \\ 
     & & g_n+\mu+\gamma 
    \end{bmatrix}, 
        V^D_I=\begin{bmatrix} 
    r_{12}+\mu+\gamma & & \\
    & \ddots & \\ 
     & & r_{nn-1}+\mu+\gamma
    \end{bmatrix}
\end{equation}
\begin{equation}
    V^B_I=\begin{bmatrix} 
    r_{12},\dots,r_{1n} & & \\
     &  \ddots &\\ 
     & &  r_{n1},\dots,r_{nn-1}
    \end{bmatrix}, 
        V^{C\intercal}_I=\begin{bmatrix} 
    -g_1m_{12},\dots,-g_1m_{1n} & & \\
     & \ddots &\\ 
     & & -g_nm_{n1},\dots,-g_nm_{nn-1}
    \end{bmatrix}
\end{equation}


Let $F,V$ be the $2N^2\times2N^2$ matrix that corresponding to the infectious compartment (E,I) of the disease model, we should have:

\begin{equation}
    F=\left[\begin{array}{@{}c|c@{}}
 \bigzero &  f+h \\
\hline
  \bigzero & \bigzero 
\end{array}\right]
\end{equation}
with 
\begin{equation}
    f=\begin{bmatrix}
        f_{1} & \dots & f_{1} \\
        f_{2} & \dots  &f_{2} \\
        \vdots & \ddots & \vdots\\
        f_{n} & \dots  & f_{n}
    \end{bmatrix},
    f_i=\begin{bmatrix}
        \beta_1^A\kappa_{i1}\frac{N_{i1}}{N_1^p} & & \\
        & \ddots & \\
        & & \beta_n^A\kappa_{in}\frac{N_{in}}{N_n^p}
    \end{bmatrix}
\end{equation}
with each $f_i$ is a $n \times n$ diagonal matrix. 
And $h$ is a $n^2 \times n^2$ full matrix with each of its entry being represented as:
\begin{equation}
h_{ij,kl}=\begin{cases}
\sum_{j=1,j\neq i}^P \sum_{d=1}^D c_{ij}^d\beta_d^Tr_{ij}\kappa_{ij,kl}\frac{N_{ij}}{N_{kl}}, \text{if $i=j$}\\
\sum_{d=1}^D c_{ij}^d\beta_d^Tg_im_{ij}\kappa_{ij,kl}\frac{N_{ii}}{N_{kl}}, \text{if $i\neq j$}
\end{cases}
\end{equation}


Finally, we can rewrite $\mathcal{V}$ as following:
\begin{equation}
    V=\left[\begin{array}{@{}c|c@{}}
  \begin{matrix}
  V_E^A & V_E^B \\
  V_E^C & V_E^D
  \end{matrix}
  & \bigzero \\
\hline
  -\Sigma &
  \begin{matrix}
  V_I^A & V_I^B \\
  V_I^C & V_I^D
  \end{matrix}
\end{array}\right]
\end{equation}


\begin{prop}
    F is non-negative, V is non-singular M-matrix and all eigenvalues of J4 have positive real part. 
\end{prop}

Then $V$ is invertible and $V^{-1}$ is non-negative.

We can write the inverse of $V$ as following:
\begin{equation}
    V^{-1}=\begin{bmatrix}
        V_E^{-1} & 0 \\
        V_I^{-1}\Sigma V_E^{-1} & V_I^{-1}\\
    \end{bmatrix}
\end{equation}

And $FV^{-1}$ is expressed as:
\begin{equation}
    FV^{-1}=\begin{bmatrix}
        (f+h) B^{-1}\Sigma A^{-1} & CB^{-1} \\
        0 & 0
    \end{bmatrix}
\end{equation}

The basic reproduction number ($R_0$) is given by 
\begin{equation}
    R_0=\sigma \rho((f+h) (AB)^{-1})
\end{equation}
where $(AB)^{-1}$ is a block diagonal matrix. 
\begin{prop}
    The basic reproduction number is bounded by ....
\end{prop}
\begin{proof}
    We denote $R$ as
    \begin{equation}
        R=f (AB)^{-1}+ h(AB)^{-1}
    \end{equation}
    
Since the spectral radius corresponds to the largest eigenvalue, based on the Perron-Frobenius theorem, we know that eigenvalues of $R$ is bounded by its smallest of the largest row sums and column sums, and the greatest of the smallest  row sums and column sums. Since $R$ is a $n^2 \times n^2$ matrix, we term $C_{ij}$ as the $ij$th column sum of $R$, and we have:
\begin{equation}
    C_{ij}=\mathbbm{1}^{\intercal}(f (AB)^{-1}_{ij}+h (AB)^{-1}_{ij})
\end{equation}
Without loss of generality, we know that for the column sum of $A$ is $\mu+\sigma$, and the column sum of $B$ is $\mu+\gamma$. Consequently, the row sum of each column in $(AB)^{-1}$ is given by $\frac{1}{(\mu+\gamma)(\mu+\sigma)}$. 

Since $(AB)$ is a block diagonal matrix, so is $(AB)^{-1}$. Then for the $ij$th column, only the entries between $i1,...,in$ may be no zero and all other entries of the column are strictly 0. Then we can write out the column sum $C_{ij}$ explicitly as:
\begin{eqnarray}
\begin{aligned}
    C_{ij}&=\mathbbm{1}^{\intercal}(\sum_i f_i (AB)^{-1}_{ij}+h (AB)^{-1}_{ij})\\
    & = \beta_1^A\kappa_{11}\frac{N_{11}}{N_1^p}v_{i1}+\dots+\beta_n^A\kappa_{1n}\frac{N_{1n}}{N_n^p}v_{in}+\beta_1^A\kappa_{21}\frac{N_{21}}{N_1^p}v_{i1}+\dots+\beta_n^A\kappa_{2n}\frac{N_{2n}}{N_n^p}v_{in}+\dots+ \beta_n^A\kappa_{nn}\frac{N_{nn}}{N_n^p}v_{in}\label{zone_inf}\\
    & +h_{11,i1}v_{i1}+\dots+h_{11,in}v_{in}+h_{12,i1}v_{i1}+\dots+h_{12,in}v_{in}+\dots+h_{nn,in}v_{in}\\
    & =(\beta_1^A\kappa_{11}\frac{N_{11}}{N_1^p}+\dots+\beta_1^A\kappa_{n1}\frac{N_{n1}}{N_1^p}+\sum_k\sum_l h_{kl,i1})v_{i1}+\dots+(\beta_n^A\kappa_{1n}\frac{N_{1n}}{N_n^p}+\dots+\beta_n^A\kappa_{nn}\frac{N_{nn}}{N_n^p}+\sum_k\sum_l h_{kl,in})v_{in}\\
\end{aligned}
\end{eqnarray}

So that
\begin{equation}
  \min_{m=1,\dots,n}  \frac{\beta_m^A\kappa_{1m}\frac{N_{1m}}{N_1^p}+\dots+\beta_m^A\kappa_{nm}\frac{N_{nm}}{N_m^p}+\sum_k\sum_l h_{kl,im}}{(\mu+\gamma)(\mu+\sigma)} \leq C \leq \max_{m=1,\dots,n}   \frac{\beta_m^A\kappa_{1m}\frac{N_{1m}}{N_1^p}+\dots+\beta_m^A\kappa_{nm}\frac{N_{nm}}{N_m^p}+\sum_k\sum_l h_{kl,im}}{(\mu+\gamma)(\mu+\sigma)}
  \label{eq:bound_r0}
\end{equation}

and
\begin{equation}
    \min_{i=1,\dots,n} \sigma C_{i}\leq R_0\leq  \max_{i=1,\dots,n} \sigma C_{i}
\end{equation}
This completes the proof. 
\end{proof}

\begin{prop}
    Let $\beta_{max}^A\kappa_{max}$ be the highest out of all zones, and $\beta_{min}^A\kappa_{min}$  be the lowest of all zones. If we assume $\kappa_{ij}$ being the same at all activity locations, then $R_0$ is bounded by the travel segments with the highest contagion rate. 
\end{prop} 
\begin{proof}
    Based on equation~\ref{eq:bound_r0}, when $\kappa_{ij}$ is homogeneous across all zones, the formulation reduces to 
    \begin{equation}
        C_{m}= \frac{\beta_m^A\kappa+\sum_k\sum_l h_{kl,mj}}{(\mu+\gamma)(\mu+\sigma)} \leq \frac{\beta_m^A\kappa+\max_{m,j=1,...,N} \sum_k\sum_l h_{kl,mj}}{(\mu+\gamma)(\mu+\sigma)}
    \end{equation}
    
    Moreover, we know that when $R_0<1$, the disease will be DFE. As a consequence, if 
    \begin{equation}
        \beta_{max}^A\kappa_{max}+\max_{m,j=1,...,N} \sum_k\sum_l h_{kl,mj} < \frac{(\mu+\sigma)(\mu+\gamma)}{\sigma}
    \end{equation}
    Then the disease will be DFE. 
    And if 
    \begin{equation}
        \beta_{min}^A\kappa_{min}+\min_{m,j=1,...,N} \sum_k\sum_l h_{kl,mj} > \frac{(\mu+\sigma)(\mu+\gamma)}{\sigma}
    \end{equation}
    Then the disease is unstable. 
\end{proof}
% \subsection{Stability of the transportation system}

% In this section we analyze the properties of the epidemic model with travel contagion, and discuss the condition under which the DFE will be stable. Due to the existence of bilinear terms, there are more than one equilibrium point in the system, and the equilibrium points are unlikely to be G.A.S due to the nonlinearity of the system. We first introduce the definition of reproduction rate $R_0$, which is arguably the most important quantity in infectious disease modeling.

% \begin{defn} [\textbf{Basic Reproduction Number}]
% 	The basic reproduction rate is the the number of cases one case generates on average over the course of its infectious period, in an otherwise uninfected population. 
% \end{defn}

% If $R_0<1$, it indicates that on average each new infected person will affect less than one uninfected person during his or her infection. Therefore, the disease will die out in the long run, and reach the DFE point asymptotically. Consequently, in order to show that the transportation system is stable at DFE, it is equivalent to show that the $R_0$ of the system is smaller than 1. 

% According to~\cite{diekmann2009construction,van2002reproduction}, the reproduction ratio $R_0$ can be measured by the dominant eigenvalue of the next generation matrix (NGM)~\cite{diekmann1990definition}, which is denoted by $K$. In particular, the NGM can be calculated as:

% \begin{equation}
% K=-T\Sigma^{-1}
% \end{equation}

% where $T$ is called the transmission matrix and $\Sigma$ is the transition matrix~\cite{diekmann2009construction}. Note that for both $T$ and $\Sigma$, only states associated with infections are taken into consideration. As for our study, the states that will affect the NGM are $E_{11},E_{12},...E_{ij},I_{11},I_{12},...I_{ij}$. If there are $P$ patches, the NGM takes the dimension $2P^2\times 2P^2$. For the transmission matrix, it captures all the dynamics related to newly infected population, while the rest of the dynamics of the system are included in the transition matrix $\Sigma$. 

% If we linearize the transportation model at the DFE point (considering that all $S_{ij}$s are constant), the matrix $T$ can be written as four blocks:

% \begin{equation}
%   \mathbf{T}=
%   \begin{blockarray}{*{3}{c} l}
%     \begin{block}{*{3}{>{$\footnotesize}c<{$}} l}
%       \textbf{E} & \textbf{I} & \textbf{$N^r$} & \\
%     \end{block}
%     \begin{block}{[*{3}{c}]>{$\footnotesize}l<{$}}
%       0 & E\rightarrow I & 0 & \textbf{E} \\
%       0 & I \rightarrow I & N^r\rightarrow I & \textbf{I} \\
%       0 & 0 & 0 & \textbf{$N^r$} \\
%     \end{block}
%   \end{blockarray}
% \end{equation}

% where $E\rightarrow I$ and $I\rightarrow I$ are $P^2 \times P^2$ matrices, whose entry denotes the coefficient values that matches an element of $E$ or $I$ to an element in $I$. Considering two variables $E_{i,j}$ and $I_{k,l}$, then the matrix $E\rightarrow I$ can be formally expressed by distinguishing the following 4 scenarios:
% \begin{enumerate}
% 	\item $i\neq j$, $k\neq l$.
% 	\item $i\neq j$, $k=l$.
% 	\item $i=j$, $k\neq l$.
% 	\item $i=j$, $k=l$
% \end{enumerate}
% and
% \begin{equation}
% E\rightarrow I (ij,kl)=\begin{cases}
% \beta_{inn}\frac{N_{ij}}{N_j^{P}}+ \frac{\sum_{m=1}^M c_{ij}^{m} \beta_{tra}^m g_im_{ij}N_{ii} c_{lk}^m \delta_{lk,ij}^m r_{kl}}{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m (g_km_{kj}N_{kk}+r_{jk}N_{jk})}, \text{case 1}\\
% \beta_{inn}\frac{N_{ij}}{N_j^{P}}+ \frac{\sum_{m=1}^M c_{ij}^{m} \beta_{tra}^m g_im_{ij}N_{ii} c_{lk}^m \delta_{lk,ij}^m g_km_{kj}}{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m (g_km_{kj}N_{kk}+r_{jk}N_{jk})}, \text{case 2}\\
% \beta_{inn}\frac{N_{ij}}{N_j^{P}}+\frac{\sum_{j=1,j\neq i}^P\sum_{m=1}^M c_{ji}^{m} \beta_{tra}^m r_{ij}S_{ij}c_{lk}^m \delta_{lk,ji}^m r_{kl}}{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m (r_{ik}N_{ik}+g_km_{ki}N_{kk})},\text{case 3}\\
% \beta_{inn}\frac{N_{ij}}{N_j^{P}}+\frac{\sum_{j=1,j\neq i}^P\sum_{m=1}^M c_{ji}^{m} \beta_{tra}^m r_{ij}S_{ij}c_{lk}^m \delta_{lk,ji}^m g_km_{ki}}{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m (r_{ik}N_{ik}+g_km_{ki}N_{kk})},\text{case 4}\\
% \end{cases}
% \end{equation}

% Similarly, we can express the entries of $I\rightarrow I$ by distinguishing the following scenarios:
% \begin{enumerate}
% 	\item $i\neq j$, $k=l=i$.
% 	\item $i=j$, $k\neq l$, $k=i$.
% \end{enumerate}
% and 
% \begin{equation}
% I \rightarrow I (ij,kl)=\begin{cases}
% g_im_{ij}, \text{case 1}\\
% r_{kl}, \text{case 2}\\
% 0,\text{otherwise}
% \end{cases}
% \end{equation} 

% Finally, for the matrix $N^r\rightarrow I$, we have:
% \begin{equation}
% N^r \rightarrow I (k,ij)=\begin{cases}
% \alpha_i^I, \text{if $i=j$ and $k=i$}\\
% 0,\text{otherwise}
% \end{cases}
% \end{equation} 

% This concludes the transmission matrix. And we next discuss the structure of the transition matrix, as follows.

% For the transition matrix $\Sigma$, it is more complicated and can be written as the following block form:
% \begin{equation}
% \mathbf{\Sigma}=
% \begin{blockarray}{*{3}{c} l}
% \begin{block}{*{3}{>{$\footnotesize}c<{$}} l}
% \textbf{E} & \textbf{I} & \textbf{$N^r$} & \\
% \end{block}
% \begin{block}{[*{3}{c}]>{$\footnotesize}l<{$}}
% E\rightarrow E & 0 & N^r\rightarrow E & \textbf{E} \\
% E\rightarrow I & I\rightarrow I & 0 & \textbf{I} \\
% \delta_E & \delta_I & 0 & \textbf{$N^r$} \\
% \end{block}
% \end{blockarray}
% \end{equation}

% And each block matrices take the following form:
% \begin{equation}
% E\rightarrow E(ij,kl)=\begin{cases}
% -g_i-\sigma-\alpha_i, \text{ if $i=j$ and $kl=ij$}\\
% r_{kl},\text{ if $i=j$ and $k=i$}\\
% -r_{ij}-\sigma-\alpha_i, \text{ if $i\neq j$ and $ij=kl$} \\
% g_im_{ij}, \text{if $i\neq j$ and $k=l=i$}\\
% 0, \text{otherwise} 
% \end{cases}
% \end{equation}

% \begin{equation}
% N^r \rightarrow E (k,ij)=\begin{cases}
% \alpha_i^E, \text{if $i=j$ and $k=i$}\\
% 0,\text{otherwise}
% \end{cases}
% \end{equation} 


% \begin{equation}
% E\rightarrow I(ij,kl)=\begin{cases}
% \sigma, \text{ if $ij=kl$}\\
% 0, \text{otherwise} 
% \end{cases}
% \end{equation}

% \begin{equation}
% I\rightarrow I(ij,kl)=\begin{cases}
% -g_i-\alpha_i-\gamma, \text{ if $i=j$ and $ij=kl$}\\
% -r_{ij}-\alpha_i-\gamma,\text{if $i\neq j$ and $ij=kl$}\\
% 0, \text{otherwise} 
% \end{cases}
% \end{equation}


% \begin{proposition}
% 	If $\rho(K)<1$, then the DFE is stable. If $\rho(K)>1$, the DFE is unstable. $\rho$ refers to the spectrum radius of a matrix.  
% \end{proposition}
% \begin{proof}
% 	The proof comes naturally from the definition of $R_0$. 
% \end{proof}


\section{Control the spread of disease within transportation system}
Since we have developed the model for infectious disease within transportation system, the next question to ask is that if we can control the spread of disease by placing entrance screening for transportation system. In particular, we have seen the implementation of radiation thermometers during the 2003 SARS outbreak for subway and bus systems, which aimed to screen out risky passengers with high body temperature. And additional measures such as distributing masks and random inspection by medical workers may also be efficient to reduce the risk exposure during travel. Meanwhile, placing entrance screening will also decrease system efficiency by introducing entry delays, which in return affecting the travel behavior of passengers in mode selection. This relationship is illustrated in Figure~\ref{fig:travel_equilibrium}. Specifically, we assume that the efforts (e.g., time and resource) required grows faster than the increments in control effectiveness, so that a high detection rate of infected people will result in a much higher entry delay. 
\begin{figure}[h!]
	\centering
	\includegraphics[width=80mm]{results/travel_equi.png}
	\caption{Illustration of the passenger dynamics}
	\label{fig:travel_equilibrium}
\end{figure}

While deriving the optimal control strategy will be intrinsically complicated for the proposed model, we make the first attempt to understand if it is possible to avoid the outbreaks of disease by placing controls on transportation system. In other words, our objective is to assess if a given control strategy may eventually lead to DFE state, and the problem falls into the field of safety verification. In the realistic transportation system, it is hardly possible to place the entry control for all travel modes. Instead, it is only viable to conduct such control over the medium and high capacity travel modes, such as buses and metros. As a consequence, in our study, we consider that passengers may choose from one or the following three travel modes:
\begin{enumerate}
	\item \textbf{Low capacity mode} such as private vehicles and taxis
	\item \textbf{Medium capacity mode} such as vans and buses
	\item \textbf{High capacity mode} such as metro system
\end{enumerate}

And passengers will choose the mode which maximize their utility (or the one with the least travel time). We consider rational behavior of passengers, and introduce the logistic function to quantify the model split ratio as:
\begin{equation}
S_{ij}^m=m_{ij}S_i\frac{e^{t_{ij}^m}}{\sum_{i=1}^M e^{t_{ij}^i}}
\end{equation}
\begin{equation}
I_{ij}^m=m_{ij}I_i\frac{e^{t_{ij}^m}}{\sum_{i=1}^M e^{t_{ij}^i}}
\end{equation}
We assume that the low capacity mode is not controllable, but typically having fewer passengers per vehicle and passengers having less chance of getting infected. On the contrary, passengers using medium or high capacity mode are usually exposed to much more people in a small compartment for a longer time, and are therefore having much higher chances of being infected. This assumption leads to the following requirement for the effective contact rate:
\begin{equation}
\beta_{tra}^{med}>\beta_{tra}^{large}>>\beta_{tra}^{small}
\end{equation}

Based on the discussion above, we arrive at the model which explicitly incorporates control over transportation system:

\begin{equation}
\begin{split}
	\dot{S}_{ii}=-g_{i}S_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}S_{ij}+\alpha_i^SN_i^r-\alpha_i S_{ii}-\beta_{inn}\frac{S_{ii}\sum_{j=1}^{P}I_{ji}}{N_i^p}\\
    -\sum_{j=1,j\neq i}^P\sum_{m=1}^M c_{ji}^{m} \beta_{tra}^m r_{ij}S_{ij} \frac{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m d_l^m(r_{ik}I_{ik}+g_km_{ki}I_{kk})}{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m (r_{ik}N_{ik}+g_km_{ki}N_{kk})}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
	\dot{S}_{ij}=-r_{ij}S_{ij}+g_im_{ij}S_{ii}-\alpha_i S_{ij}-\beta_{inn}\frac{S_{ij}\sum_{k=1}^{P}I_{kj}}{N_j^p}\\
    -\sum_{m=1}^M c_{ij}^{m} \beta_{tra}^m g_im_{ij}S_{ii} \frac{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m d_l^m(g_km_{kj}I_{kk}+r_{jk}I_{jk})}{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m (g_km_{kj}N_{kk}+r_{jk}N_{jk})}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
	\dot{E}_{ii}=-g_{i}E_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}E_{ij}+\alpha_i^EN_i^r-\alpha_i E_{ii}-\sigma E_{ii}+\beta_{inn}\frac{S_{ii}\sum_{j=1}^{P}I_{ji}}{N_i^p}\\
    +\sum_{j=1,j\neq i}^P\sum_{m=1}^M c_{ji}^{m} \beta_{tra}^m r_{ij}S_{ij} \frac{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m d_l^m(r_{ik}I_{ik}+g_km_{ki}I_{kk})}{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m (r_{ik}N_{ik}+g_km_{ki}N_{kk})}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
	\dot{E}_{ij}=-r_{ij}E_{ij}+g_i m_{ij}E_{ii}-\alpha_i E_{ij}-\sigma E_{ij}+\beta_{inn}\frac{S_{ij}\sum_{k=1}^{P}I_{kj}}{N_j^p}\\
    +\sum_{m=1}^M c_{ij}^{m} \beta_{tra}^m g_im_{ij}S_{ii} \frac{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m d_l^m(g_km_{kj}I_{kk}+r_{jk}I_{jk})}{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m (g_km_{kj}N_{kk}+r_{jk}N_{jk})}
\end{split}
\end{equation}

\begin{equation}
	\dot{I}_{ii}=-g_{i}I_{ii}+\alpha_i^IN_i^r-\alpha_i I_{ii}+\sum_{j=1,j\neq i}^{P}\sum_m r_{ij}d_l^mc_{ij}^mI_{ij}+\sigma E_{ii}-\gamma I_{ii}
\end{equation} 

\begin{equation}
	\dot{I}_{ij}=-r_{ij}I_{ij}-\alpha_i I_{ij}+\sum_m g_i m_{ij} c_{ij}^m d_l^m I_{ii}+\sigma E_{ij}-\gamma I_{ij}
\end{equation}

\begin{equation}
	\dot{R}_{ii}=-g_{i}R_{ii}+\alpha_i^RN_i^r-\alpha_i S_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}R_{ij}+\gamma I_{ii}+\sum_{j=1,j\neq i}^{P}\sum_m r_{ij}c_{ij}^m(1-d_l^m)I_{ij}
\end{equation}

\begin{equation}
	\dot{R}_{ij}=-r_{ij}R_{ij}+g_i m_{ij}R_{ii}-\alpha_i R_{ij}+\gamma I_{ij} +\sum_m g_i m_{ij} c_{ij}^m (1-d_l^m) I_{ii}
\end{equation}


==> part B disease_network/intro.tex <==
\section{Introduction}
As of 2018, there were over 4.2 billion people living in urban areas and the number is estimated to reach 6.3 billion (70\% of the total world population) in 2050~\cite{wordlpopu18}. The rapid growth of the urban population gives rise to the prosperity of the urban economy with much more travel and intensive daily activities. A notable example is the development of urban mass transit systems. As the only affordable mobility solution to the general urban public, it has grown to enormous scale in large cities with buses and metros serving over 53 billion passengers worldwide as of 2017~\cite{urban_trans_2018}. Behind the giant number, however, is an environment that favors the spread of infectious diseases which constitutes a significant health risk to the entire urban community. On the one hand, the urban population is making more trips and traveling a longer distance, with the average annual person-mile traveled in the United States increased by 169\% from 1969 to 2009~\cite{chambers2015passenger}. On the other hand, people are spending more time in the transportation system especially in urban areas. For New York City, the average commuting to work time exceeds 40 minutes for 69\% of the city's neighborhoods, and 59\% of New York commuters use mass transit as the tool for commuting. To meet the growing mobility needs with limited mobility resources, the mass transit systems are developed to carry as many passengers, leading to enclosed compartments with high population density, close proximity, and long duration. This represents sufficient exposure duration and a close-enough distance that allows for the pathogens to migrate among unprotected daily commuters. A direct consequence is the recent outbreaks of the COVID-19 in major cities worldwide~\cite{dong2020interactive} with over 4 million confirmed cases and 270 thousand deaths as of May 2020. Despite the significant risks associated with the urban transportation system and the outrageous consequences caused by numerous infectious diseases, the role played by the urban transportation system during the outbreaks of infectious diseases in urban areas remains largely unexplored. This motivates us to make the initial attempt to model the contagion process during travel and further explore possible mitigation measures that may help to curb the spread of infectious diseases. 

There are two main approaches in the literature for characterizing the dynamics of infectious diseases. The first approach comprises of the compartment model, where the initial SIR model (also known as Kermack-McKendrick model) divides the population into compartments of susceptible, infected, and recovered, and non-linear ordinary differential equations (ODE) are used to model the dynamics among the compartments~\cite{kermack1927contribution}. Based on the SIR model, a variety of models have been developed to account for more realistic disease nature, including models which consider the incubation period~\cite{li1995global}, the vertical transmission~\cite{smith2001global}, the age structure~\cite{castillo1989epidemiological}, and the vaccine strategy~\cite{shulgin1998pulse,d2005pulse}. And extensive efforts were made to understand the property of the model and analyze the local and global stability of the non-linear ODEs, where surveys of related works can be found in~\cite{hethcote1981periodicity,liu1987dynamical}. One major criticism for the compartment model is the oversimplified assumptions, where the population in each compartment is assumed to be fully mixed and therefore each individual has the same behavior. Therefore, the model may fail to represent the complex mobility and contact patterns for many real-world diseases. To address this shortcoming, the second approach models the disease propagation at the individual level over large-scale networks, where each individual is represented by a node and their contact structure is captured by the set of edges~\cite{newman2002spread,meyers2007contact}. The approach was developed based on the method of bond percolation model, and the generation function was used for deriving the important attributes of a certain contact network, including the average degree and excessive degree, which later used to calculate the size of the disease outbreaks. Danon et al.~\cite{danon2011networks} conducted a comprehensive review of the works in this approach. The contact network model helps to capture diverse interactions among individuals with given distribution and contributes to the understanding between disease dynamics and the network topology. However, it is not applicable to understand the spread of infectious disease in densely populated urban areas: it is computationally intractable to construct the individual contact network for all urban populations and it is also impossible to obtain the necessary input for the contact network as evaluating the individual's contact pattern will be very expensive. 

In light of the existing efforts and issues,  to model the spread of infectious diseases for the urban areas, the compartment model is still the ideal choice due to its well-explored mathematical properties and the scalability when it comes to model the mass urban population. However, the simplistic assumption of homogeneous population mixing needs to be corrected as the population dynamics are highly heterogeneous in large cities. In particular, since human mobility is the driving factor for the spread of infectious diseases, it is necessary for the compartment model to account for the mobility dynamics around the city. And the needs of mobility dynamics assert two additional challenges for developing appropriate compartment models to represent the urban disease dynamics. First, the diverse land use and activity patterns in urban areas suggest the necessity to incorporate the spatial-varying mobility patterns and activity patterns into each of the original disease-related compartments, so that the rate of transmission and the amount of population should be differentiated at individual subareas of a city. On the other hand, while the spatial movements bring people to their activity locations, it also results in massive contact and contagion during travel which is negligible given the existence of urban mass transit systems. This together with the spatial heterogeneity require additional consideration to explicitly capture the contact and the disease transmission during travel as separate compartments. To address these challenges, we propose the spatial SEIR model with travel contagion (Trans-SEIR) to characterize the spread of infectious diseases in urban areas. The proposed model overcomes the first challenge by developing an urban mobility model to represent the mobility dynamics of leaving home, traveling to-and-from activity locations and activity engagements. Then the SEIR process can then be overlaid with the mobility model to reflect the spatial heterogeneity of the disease dynamics. In addition, the Trans-SEIR model considers two types of contagion, namely the activity contagion and travel contagion, to explicitly separate the infections due to urban travel activities and the infections that arise from daily activities such as work and entertainment. Based on the Trans-SEIR model, we further explore the implementation of entrance control in the urban transportation system and develop the optimal resource allocation problem which determined the distribution of limited medical resources and manpower over the travel segments in urban areas to minimize the risk from the infectious diseases. To this end, the proposed Trans-SEIR model represents a realistic modeling framework to understand the complete trajectories of disease outbreaks in urban areas, and serves as the essential modeling components for devising optimal control strategies and policies, which have significant implications to both preventative prevention as well as disease mitigation from the urban transportation system perspective.

The rest of the study is organized as follows. In the next section, we briefly introduce the background of epidemic modeling with compartment models and establish the basics for modeling the mobility dynamics. In Section 3, we present the mathematical formulations for the Trans-SEIR model and analyze the theoretical properties of the model, followed by the optimal entrance control model for urban transportation systems in Section 4. In Section 5, we present the numerical experiments of both toy networks and the real-world case study for the COVID-19 outbreak in New York City (NYC). Finally, we conclude our study with major findings and insights in Section 6. 

==> part B disease_network/method.tex <==
\section{Modeling disease spreading with travel contagion}
\subsection{The basic model}
\subsubsection{Notation}
We summarize the list of variables used in this section as follows
\begin{table}[htbp!]
	\setstretch{1.2}
	\centering
	\caption{Table of notation}
	\label{notation}
	\begin{tabular}{p{2cm}p{13.5cm}}
		\hline
		Notation & Description \\ \hline
		&\textbf{Variables}\\ \hline
		$S_{ij}$ & Susceptible population who are residents of patch $i$ and currently in patch $j$. \\
		$E_{ij}$ & Exposed (latent) population who are residents of patch $i$ and currently in patch $j$.\\
		$I_{ij}$ & Infected population who are residents of patch $i$ and currently in patch $j$. \\
		$R_{ij}$ & Recovered population who are residents of patch $i$ and currently in patch $j$.\\
		$t_{ij}^m$ & Induced travel time for moving from patch $i$ to patch $j$ using mode $m$. \\
		$N_i^p$ & Population at patch $i$. \\
		$N_{ij}$ & The amount of people currently at patch $j$ who are the residents of patch $i$. \\
		\hline
		&\textbf{Fixed parameters}\\ \hline
        $M$ & Total number of travel modes available. \\
        $m$ & Travel mode $m$, where $m=1,2,...,M$. \\
		$\beta_{inn}$ & Within zone disease transmission rate. \\
		$\beta_{tra}^m$ & Disease transmission rate for travel mode $m$. \\ 
		$c_{ij}^m$ & The ratio of people who choose travel mode $m$ between patch $i$ and patch $j$. \\
		$d_l^m$ & Rate of remaining infected people for travel mode $m$ at control level $l$. \\
		 \hline
	\end{tabular}
\end{table}

\subsubsection{System dynamics}
An important component missing from the previously discussed SEIR model is the spatial interaction. The model only considers local dynamics, but it is essential for urban areas to model explicitly how population flow moving around the city. In particular, these flows are driven by various activities, such as work, school, or entertainment. And people get in contact with others by taking different activities through various transportation tools. As long as some individuals are infected, their activities and the urban transportation mobility will take the disease to every corner of the city. This motivates us to understand the the spread of infectious disease in urban area by modeling the system with the following 6 dynamics: 
\begin{enumerate}
\item The mobility dynamics of urban population follows the model as discussed in section 3.2.
\item Similar to the SEIR model, we consider $S_{ij}$ being affected by $I_{ij}$ with the inner-patch contagion rate $\beta_{inn}$. 
\item In addition to the spread due to within patch activities, we also consider people get infected during travel. That is, $S_{ij}$ may be infected by contacting with $I_{ij}$ if they use the same travel mode $m$, with the contagion rate of $\beta_{tra}^m$. 
\item Once people in $S_{ij}$ are infected, they become $E_{ij}$. They are not infectious until the end of the latent period, and the length of latent period is characterized by $1/\sigma$.
\item People in $E_{ij}$ become $I_{ij}$ at the end of the latent period. And the length of the infectious period is characterized by $1/\gamma$. 
\item At the end of their infectious period, people in $I_{ij}$ become $R_{ij}$. For simplicity, we consider that they gain permanent immunity to the disease and will be no longer infected.  
\end{enumerate}

In particular, the contagion process between susceptible and infected population can be illustrated by the example of a 3-patch network as shown in Figure~\ref{fig:examp}
\begin{figure}[h!]
	\centering
	\includegraphics[width=150mm]{results/contaillust.pdf}
	\caption{Illustration of the disease contagion process in a 3-patch network}
	\label{fig:examp}
\end{figure}
There are 3 patches in the network, with two travel links 1-2 and 2-3 and three possible routes: from patch 1 to patch 2, from patch 1 to patch 3, and from patch 2 to patch 3. And we have two different contagions in this network. One is the inner-patch contagion which takes place between $S$ and $I$ population in the same patch. Additionally, there is travel contagion (shown in dashed line), which may happen if two population share overlay segments in their travel routes. Consequently, we have two possible travel contagions: between people travel from 1 to 2 and 1 to 3, and between people travel from 1 to 3 and 2 to 3. While this is only an illustration, the overlay segment will be later differentiated based on the travel modes as well.


\subsubsection{Formulation}

where we have the contagion at home, at activity location and during travel as:
\begin{equation}
    f_{ij}(S,I)=\beta^{A}_j\kappa_{ij}\frac{S_{ij}\sum_{k=1}^{N}I_{kj}}{N_j^p}
\end{equation}
\begin{equation}
    f_{ii}(S,I)=\beta^{A}_i\kappa_{ii}\frac{S_{ii}\sum_{k=1}^{N}I_{ki}}{N_i^p}
\end{equation}
\begin{equation}
    h_{\la{ij}}(S,I)=\sum_{j=1,j\neq i}^P\sum_{d=1}^D c_{ij}^{d} \beta_d^T {S}_{\la{ij}} [\sum_{k=1}^P\sum_{l=1,l\neq k}^P \frac{\kappa_{\la{kl},\la{ij}}^d I_{\la{kl}}}{N_{\la{kl}}}+\frac{\kappa_{\ra{kl},\la{ij}}^d I_{\ra{kl}}}{N_{\ra{kl}}}]
    \label{eq:travel_return_infect}
\end{equation}
\begin{equation}
    h_{\ra{ij}}(S,I)=\sum_{j=1,j\neq i}^P\sum_{d=1}^D c_{ij}^{d} \beta_d^T {S}_{\ra{ij}} [\sum_{k=1}^P\sum_{l=1,l\neq k}^P \frac{\kappa_{\la{kl},\ra{ij}}^d I_{\la{kl}}}{N_{\la{kl}}}+\frac{\kappa_{\ra{kl},\ra{ij}}^d I_{\ra{kl}}}{N_{\ra{kl}}}]
    \label{eq:travel_out_infect}
\end{equation}

Equation~\ref{eq:travel_return_infect} summarizes the S population who returns to home $i$ and get infected during travel, by encountering I population to-and-from resident location in other places. Specifically, $c_{ij}^dg_im_{ij}S_{ii}$ captures the ratio of $S_{ii}$ who leaves for destination $j$ using transportation mode $d$. $\frac{\kappa_{kl,ij}^d I_{kl}}{N_{kl}}$ denotes the contact rate with infectious population returning from $l$ to $k$, which is simplified from:
\begin{equation}
    \frac{\kappa_{kl,ij}^d c_{kl}^dr_{kl} I_{kl}}{c_{kl}^dr_{kl} N_{kl}}
\end{equation}
and $\kappa_{kl,ij}^d$ refers to the number of contacts on average between ODs $kl$ and $ij$, and is a function of the travel time. Similarly, $\frac{\kappa_{kl,ij}^d I_{kk}}{N_{kk}}$ represents the contact rate with the infectious population leaving from $k$ to $l$, which is simplified from:
\begin{equation}
    \frac{\kappa_{kl,ij}^d c_{kl}^dg_km_{kl}I_{kk}}{c_{kl}^dg_km_{kl}N_{kk}}
\end{equation}
With the above four different incidences for possible disease transmission, we can formally express the mathematical formulations that describe the transportation disease spreading process in urban area as follows:
\begin{eqnarray}
\begin{aligned}
\dot{E}_{ii}=&-g_{i}E_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}E_{ij}-\sigma E_{ii}+f_{ii}(S,I)+h_{ii}(S,I)-\mu E_{ii}\\
\dot{E}_{ij}=&-r_{ij}E_{ij}+g_i m_{ij}E_{ii}-\sigma E_{ij}+f_{ij}(S,I)+h_{ij}(S,I)-\mu E_{ij}\\
\dot{I}_{ii}=&-g_{i}I_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}I_{ij}+\sigma E_{ii}-\gamma I_{ii}-\mu I_{ii}\\
\dot{I}_{ij}=&-r_{ij}I_{ij}+g_i m_{ij}I_{ii}+\sigma E_{ij}-\gamma I_{ij}-\mu I_{ij}\\
\dot{S}_{ii}=&-g_{i}S_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}S_{ij}-f_{ii}(S,I)-h_{ii}(S,I)+\mu(N_i^r-S_{ii})\\
\dot{S}_{ij}=&-r_{ij}S_{ij}+g_im_{ij}S_{ii}-f_{ij}(S,I)-h_{ij}(S,I)-\mu S_{ij}\\
\dot{R}_{ii}=&-g_{i}R_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}R_{ij}+\gamma I_{ii}-\mu R_{ii}\\
\dot{R}_{ij}=&-r_{ij}R_{ij}+g_i m_{ij}R_{ii}+\gamma I_{ij}-\mu R_{ij}
\end{aligned}
\label{eq:seir_system}
\end{eqnarray}

The system described by equation~\ref{eq:seir_system} can be easily understood by decomposing each equation into the part of mobility dynamics and the part of disease dynamics. In particular, for equations characterizing the dynamics of $S_{ii},E_{ii},I_{ii}, R_{ii}$, the first four terms on the right-hand-side (RHS) capture the mobility dynamics, which are consistent with equation~\ref{eq:st}. Similarly, the first three terms on the RHS of equations for $S_{ij},E_{ij},I_{ij}, R_{ij}$ can be analogous to equation~\ref{eq:bt}.   

% The disease dynamics of equation~\ref{eq:sii} has two components. The first component with the coefficient $\beta_{inn}$ characterizes the within patch spread of diseases, where $\sum_jI_{ji}$ refers to total infected population in patch $i$ and the contagion has the bilinear incident form which is consistent with the SEIR model. The second component which is associated with the coefficient $\beta_{tra}$ denote the spread of diseases during travel. Specifically, this term describes how susceptible people who return from $j$ to $i$ get in contact with infectious population. For the contagion to take place, $S$ and $I$ must be in the same travel mode and share trip segment(s) in common. And the indicator variable $\delta_{ki,ji}^m$ is introduced to indicate if trips made from $k$ to $i$ and from $j$ to $i$ using travel mode $m$ have overlapping parts. And the infected $S_{ii}$ are added to $E_{ii}$ as shown in equation~\ref{eq:eii}. Moreover, $E_{ii}$ and $I_{ii}$ (or equation~\ref{eq:eii} and~\ref{eq:iii}) are connected by the term $\sigma E_{ii}$, which implies the end of latent period. Similarly, $I_{ii}$ and $R_{ii}$ (or equation~\ref{eq:iii} and~\ref{eq:rii}) are correlated by the term $\gamma I_{ii}$.

% On the other hand, the disease dynamics for equation~\ref{eq:sij} also involves two components. The first component with the coefficient $\beta_{inn}$ captures how $S_{ij}$ gets infected during the contagion with other infected population. The second component with the coefficient $\beta_{tra}$ describes the spread of diseases while people are traveling from $i$ to $j$. That is, only departed population $g_jm_{ij}S_{ii}$ may have the chance of being infected during their travel to $j$. And the contagion may happen when they get in contact with departed infectious population who have the same destination using the same mode, which is captured by $\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m g_km_{kj}I_{kk}$. And both parts of infected $S_{ij}$ are added to $E_{ij}$ as shown in equation~\ref{eq:eij}. Finally, we have the same correlations between $E_{ij}$ and $I_{ij}$, and between $I_{ij}$ and $R_{ij}$, as discussed in the previous paragraph. This concludes the basic model for characterizing disease dynamics with travel contagion. 

\begin{prop}
Based on equation~\ref{eq:seir_system}, we can decompose the system into $\mathcal{F}-\mathcal{V}$ where we have
\begin{equation}
\mathcal{F}=
\begin{bmatrix}
      f_{ii}+h_{ii}\\
      f_{ij}+h_{ij}\\
      0\\
      0\\
      0\\
      0\\
      0\\
      0
\end{bmatrix}
, \mathcal{V}=
\begin{bmatrix}
    (g_{i}+\mu+\sigma)E_{ii}-\sum_{j=1,j\neq i}^{P}r_{ij}E_{ij}\\
    (r_{ij}+\mu+\sigma)E_{ij}-g_i m_{ij}E_{ii} \\
    (g_{i}+\mu+\gamma)I_{ii}-\sum_{j=1,j\neq i}^{P}r_{ij}I_{ij}-\sigma E_{ii}\\
    (r_{ij}+\mu+\gamma)I_{ij}-g_i m_{ij}I_{ii}-\sigma E_{ij}\\
    (g_{i}+\mu)S_{ii}-\sum_{j=1,j\neq i}^{P}r_{ij}S_{ij}-\mu N_i^r\\
    (r_{ij}+\mu)S_{ij}-g_i m_{ij}S_{ii} \\
    (g_{i}+\mu)R_{ii}-\sum_{j=1,j\neq i}^{P}r_{ij}R_{ij}-\gamma I_{ii}\\
    (r_{ij}+\mu)R_{ij}-g_i m_{ij}R_{ii}-\gamma I_{ij} 
    \end{bmatrix}
\end{equation}
\end{prop}




Considering that an infectious disease has been introduced, and people are aware of the disease patterns in the city. An essential question to answer is that if the disease will eventually invade the population. This requires the understanding of the stability of disease free equilibrium (DFE). In other words, if the DFE is stable, then the disease will be absent from the population, otherwise it is always possible for disease outbreak. 
 \begin{defn}
 	The disease dynamic system characterized by equation 5.1-5.8 has two equilibrium points. The first equilibrium point $x_0$ is the disease free equilibrium (DFE):
 	\begin{equation}
 	S_{ij}=N_{ij},E_{ij}=I_{ij}=R_{ij}=0
 	\end{equation}
 	\begin{equation}
 	    x_0=(0,0,N,0)
 	\end{equation}
 	The second equilibrium point is the endemic equilibrium:
 	\begin{equation}
 	\sum_{ij} S_{ij}=0
 	\end{equation}
 	such that no susceptible population available and all people are eventually infected. 
 \end{defn}
 
\subsection{Model analysis}

If we linearize the system at $x_0$, we have $D\mathcal{F}(x_0)$ as:
\begin{equation}
    D\mathcal{F}(x_0)=\begin{bmatrix}
        0 & 0 & \frac{df_{ii}(x_0)}{d I_{ii}}+\frac{dh_{ii}(x_0)}{d I_{ii}} & \frac{df_{ii}(x_0)}{d I_{ij}}+\frac{dh_{ii}(x_0)}{d I_{ij}} & 0 & 0 & 0 & 0\\
        0 & 0 &\frac{df_{ij}(x_0)}{d I_{ii}}+\frac{dh_{ij}(x_0)}{d I_{ii}} & \frac{df_{ij}(x_0)}{d I_{ij}}+\frac{dh_{ij}(x_0)}{d I_{ij}} & 0 & 0 & 0 & 0\\
        0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
        0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
    \end{bmatrix}
\end{equation}

We can further partition matrix $V$ as in the following format:
\begin{equation}
    D\mathcal{V}(x_0)=\left[\begin{array}{@{}c|c@{}}
  \begin{matrix}
  V_E^A & V_E^B \\
  V_E^C & V_E^D
  \end{matrix}
  & \bigzero \\
\hline
  -\Sigma &
  \begin{matrix}
  V_I^A & V_I^B \\
  V_I^C & V_I^D
  \end{matrix}
\end{array}\right]
\end{equation}

where $\Sigma$ represents the diagonal matrix of $\sigma$, and we have
\begin{equation}
    V^A_E=\begin{bmatrix} 
    g_1+\mu+\sigma & & \\
    & \ddots & \\ 
     & & g_n+\mu+\sigma 
    \end{bmatrix}, 
        V^D_E=\begin{bmatrix} 
    r_{12}+\mu+\sigma & & \\
    & \ddots & \\ 
     & & r_{nn-1}+\mu+\sigma 
    \end{bmatrix}
\end{equation}

\begin{equation}
    V^B_E=\begin{bmatrix} 
    r_{12},\dots,r_{1n} & & \\
     &  \ddots &\\ 
     & &  r_{n1},\dots,r_{nn-1}
    \end{bmatrix}, 
        V^{C\intercal}_E=\begin{bmatrix} 
    -g_1m_{12},\dots,-g_1m_{1n} & & \\
     & \ddots &\\ 
     & & -g_nm_{n1},\dots,-g_nm_{nn-1}
    \end{bmatrix}
\end{equation}
And similarly, for compartments of $I$ population, we have
\begin{equation}
    V^A_I=\begin{bmatrix} 
    g_1+\mu+\gamma & & \\
    & \ddots & \\ 
     & & g_n+\mu+\gamma 
    \end{bmatrix}, 
        V^D_I=\begin{bmatrix} 
    r_{12}+\mu+\gamma & & \\
    & \ddots & \\ 
     & & r_{nn-1}+\mu+\gamma
    \end{bmatrix}
\end{equation}
\begin{equation}
    V^B_I=\begin{bmatrix} 
    r_{12},\dots,r_{1n} & & \\
     &  \ddots &\\ 
     & &  r_{n1},\dots,r_{nn-1}
    \end{bmatrix}, 
        V^{C\intercal}_I=\begin{bmatrix} 
    -g_1m_{12},\dots,-g_1m_{1n} & & \\
     & \ddots &\\ 
     & & -g_nm_{n1},\dots,-g_nm_{nn-1}
    \end{bmatrix}
\end{equation}


Let $F,V$ be the $2N^2\times2N^2$ matrix that corresponding to the infectious compartment (E,I) of the disease model, we should have:

\begin{equation}
    F=\left[\begin{array}{@{}c|c@{}}
 \bigzero &  f+h \\
\hline
  \bigzero & \bigzero 
\end{array}\right]
\end{equation}
with 
\begin{equation}
    f=\begin{bmatrix}
        f_{1} & \dots & f_{1} \\
        f_{2} & \dots  &f_{2} \\
        \vdots & \ddots & \vdots\\
        f_{n} & \dots  & f_{n}
    \end{bmatrix},
    f_i=\begin{bmatrix}
        \beta_1^A\kappa_{i1}\frac{N_{i1}}{N_1^p} & & \\
        & \ddots & \\
        & & \beta_n^A\kappa_{in}\frac{N_{in}}{N_n^p}
    \end{bmatrix}
\end{equation}
with each $f_i$ is a $n \times n$ diagonal matrix. 
And $h$ is a $n^2 \times n^2$ full matrix with each of its entry being represented as:
\begin{equation}
h_{ij,kl}=\begin{cases}
\sum_{j=1,j\neq i}^P \sum_{d=1}^D c_{ij}^d\beta_d^Tr_{ij}\kappa_{ij,kl}\frac{N_{ij}}{N_{kl}}, \text{if $i=j$}\\
\sum_{d=1}^D c_{ij}^d\beta_d^Tg_im_{ij}\kappa_{ij,kl}\frac{N_{ii}}{N_{kl}}, \text{if $i\neq j$}
\end{cases}
\end{equation}


Finally, we can rewrite $\mathcal{V}$ as following:
\begin{equation}
    V=\left[\begin{array}{@{}c|c@{}}
  \begin{matrix}
  V_E^A & V_E^B \\
  V_E^C & V_E^D
  \end{matrix}
  & \bigzero \\
\hline
  -\Sigma &
  \begin{matrix}
  V_I^A & V_I^B \\
  V_I^C & V_I^D
  \end{matrix}
\end{array}\right]
\end{equation}


\begin{prop}
    F is non-negative, V is non-singular M-matrix and all eigenvalues of J4 have positive real part. 
\end{prop}

Then $V$ is invertible and $V^{-1}$ is non-negative.

We can write the inverse of $V$ as following:
\begin{equation}
    V^{-1}=\begin{bmatrix}
        V_E^{-1} & 0 \\
        V_I^{-1}\Sigma V_E^{-1} & V_I^{-1}\\
    \end{bmatrix}
\end{equation}

And $FV^{-1}$ is expressed as:
\begin{equation}
    FV^{-1}=\begin{bmatrix}
        (f+h) B^{-1}\Sigma A^{-1} & CB^{-1} \\
        0 & 0
    \end{bmatrix}
\end{equation}

The basic reproduction number ($R_0$) is given by 
\begin{equation}
    R_0=\sigma \rho((f+h) (AB)^{-1})
\end{equation}
where $(AB)^{-1}$ is a block diagonal matrix. 
\begin{prop}
    The basic reproduction number is bounded by ....
\end{prop}
\begin{proof}
    We denote $R$ as
    \begin{equation}
        R=f (AB)^{-1}+ h(AB)^{-1}
    \end{equation}
    
Since the spectral radius corresponds to the largest eigenvalue, based on the Perron-Frobenius theorem, we know that eigenvalues of $R$ is bounded by its smallest of the largest row sums and column sums, and the greatest of the smallest  row sums and column sums. Since $R$ is a $n^2 \times n^2$ matrix, we term $C_{ij}$ as the $ij$th column sum of $R$, and we have:
\begin{equation}
    C_{ij}=\mathbbm{1}^{\intercal}(f (AB)^{-1}_{ij}+h (AB)^{-1}_{ij})
\end{equation}
Without loss of generality, we know that for the column sum of $A$ is $\mu+\sigma$, and the column sum of $B$ is $\mu+\gamma$. Consequently, the row sum of each column in $(AB)^{-1}$ is given by $\frac{1}{(\mu+\gamma)(\mu+\sigma)}$. 

Since $(AB)$ is a block diagonal matrix, so is $(AB)^{-1}$. Then for the $ij$th column, only the entries between $i1,...,in$ may be no zero and all other entries of the column are strictly 0. Then we can write out the column sum $C_{ij}$ explicitly as:
\begin{eqnarray}
\begin{aligned}
    C_{ij}&=\mathbbm{1}^{\intercal}(\sum_i f_i (AB)^{-1}_{ij}+h (AB)^{-1}_{ij})\\
    & = \beta_1^A\kappa_{11}\frac{N_{11}}{N_1^p}v_{i1}+\dots+\beta_n^A\kappa_{1n}\frac{N_{1n}}{N_n^p}v_{in}+\beta_1^A\kappa_{21}\frac{N_{21}}{N_1^p}v_{i1}+\dots+\beta_n^A\kappa_{2n}\frac{N_{2n}}{N_n^p}v_{in}+\dots+ \beta_n^A\kappa_{nn}\frac{N_{nn}}{N_n^p}v_{in}\label{zone_inf}\\
    & +h_{11,i1}v_{i1}+\dots+h_{11,in}v_{in}+h_{12,i1}v_{i1}+\dots+h_{12,in}v_{in}+\dots+h_{nn,in}v_{in}\\
    & =(\beta_1^A\kappa_{11}\frac{N_{11}}{N_1^p}+\dots+\beta_1^A\kappa_{n1}\frac{N_{n1}}{N_1^p}+\sum_k\sum_l h_{kl,i1})v_{i1}+\dots+(\beta_n^A\kappa_{1n}\frac{N_{1n}}{N_n^p}+\dots+\beta_n^A\kappa_{nn}\frac{N_{nn}}{N_n^p}+\sum_k\sum_l h_{kl,in})v_{in}\\
\end{aligned}
\end{eqnarray}

So that
\begin{equation}
  \min_{m=1,\dots,n}  \frac{\beta_m^A\kappa_{1m}\frac{N_{1m}}{N_1^p}+\dots+\beta_m^A\kappa_{nm}\frac{N_{nm}}{N_m^p}+\sum_k\sum_l h_{kl,im}}{(\mu+\gamma)(\mu+\sigma)} \leq C \leq \max_{m=1,\dots,n}   \frac{\beta_m^A\kappa_{1m}\frac{N_{1m}}{N_1^p}+\dots+\beta_m^A\kappa_{nm}\frac{N_{nm}}{N_m^p}+\sum_k\sum_l h_{kl,im}}{(\mu+\gamma)(\mu+\sigma)}
  \label{eq:bound_r0}
\end{equation}

and
\begin{equation}
    \min_{i=1,\dots,n} \sigma C_{i}\leq R_0\leq  \max_{i=1,\dots,n} \sigma C_{i}
\end{equation}
This completes the proof. 
\end{proof}

\begin{prop}
    Let $\beta_{max}^A\kappa_{max}$ be the highest out of all zones, and $\beta_{min}^A\kappa_{min}$  be the lowest of all zones. If we assume $\kappa_{ij}$ being the same at all activity locations, then $R_0$ is bounded by the travel segments with the highest contagion rate. 
\end{prop} 
\begin{proof}
    Based on equation~\ref{eq:bound_r0}, when $\kappa_{ij}$ is homogeneous across all zones, the formulation reduces to 
    \begin{equation}
        C_{m}= \frac{\beta_m^A\kappa+\sum_k\sum_l h_{kl,mj}}{(\mu+\gamma)(\mu+\sigma)} \leq \frac{\beta_m^A\kappa+\max_{m,j=1,...,N} \sum_k\sum_l h_{kl,mj}}{(\mu+\gamma)(\mu+\sigma)}
    \end{equation}
    
    Moreover, we know that when $R_0<1$, the disease will be DFE. As a consequence, if 
    \begin{equation}
        \beta_{max}^A\kappa_{max}+\max_{m,j=1,...,N} \sum_k\sum_l h_{kl,mj} < \frac{(\mu+\sigma)(\mu+\gamma)}{\sigma}
    \end{equation}
    Then the disease will be DFE. 
    And if 
    \begin{equation}
        \beta_{min}^A\kappa_{min}+\min_{m,j=1,...,N} \sum_k\sum_l h_{kl,mj} > \frac{(\mu+\sigma)(\mu+\gamma)}{\sigma}
    \end{equation}
    Then the disease is unstable. 
\end{proof}
% \subsection{Stability of the transportation system}

% In this section we analyze the properties of the epidemic model with travel contagion, and discuss the condition under which the DFE will be stable. Due to the existence of bilinear terms, there are more than one equilibrium point in the system, and the equilibrium points are unlikely to be G.A.S due to the nonlinearity of the system. We first introduce the definition of reproduction rate $R_0$, which is arguably the most important quantity in infectious disease modeling.

% \begin{defn} [\textbf{Basic Reproduction Number}]
% 	The basic reproduction rate is the the number of cases one case generates on average over the course of its infectious period, in an otherwise uninfected population. 
% \end{defn}

% If $R_0<1$, it indicates that on average each new infected person will affect less than one uninfected person during his or her infection. Therefore, the disease will die out in the long run, and reach the DFE point asymptotically. Consequently, in order to show that the transportation system is stable at DFE, it is equivalent to show that the $R_0$ of the system is smaller than 1. 

% According to~\cite{diekmann2009construction,van2002reproduction}, the reproduction ratio $R_0$ can be measured by the dominant eigenvalue of the next generation matrix (NGM)~\cite{diekmann1990definition}, which is denoted by $K$. In particular, the NGM can be calculated as:

% \begin{equation}
% K=-T\Sigma^{-1}
% \end{equation}

% where $T$ is called the transmission matrix and $\Sigma$ is the transition matrix~\cite{diekmann2009construction}. Note that for both $T$ and $\Sigma$, only states associated with infections are taken into consideration. As for our study, the states that will affect the NGM are $E_{11},E_{12},...E_{ij},I_{11},I_{12},...I_{ij}$. If there are $P$ patches, the NGM takes the dimension $2P^2\times 2P^2$. For the transmission matrix, it captures all the dynamics related to newly infected population, while the rest of the dynamics of the system are included in the transition matrix $\Sigma$. 

% If we linearize the transportation model at the DFE point (considering that all $S_{ij}$s are constant), the matrix $T$ can be written as four blocks:

% \begin{equation}
%   \mathbf{T}=
%   \begin{blockarray}{*{3}{c} l}
%     \begin{block}{*{3}{>{$\footnotesize}c<{$}} l}
%       \textbf{E} & \textbf{I} & \textbf{$N^r$} & \\
%     \end{block}
%     \begin{block}{[*{3}{c}]>{$\footnotesize}l<{$}}
%       0 & E\rightarrow I & 0 & \textbf{E} \\
%       0 & I \rightarrow I & N^r\rightarrow I & \textbf{I} \\
%       0 & 0 & 0 & \textbf{$N^r$} \\
%     \end{block}
%   \end{blockarray}
% \end{equation}

% where $E\rightarrow I$ and $I\rightarrow I$ are $P^2 \times P^2$ matrices, whose entry denotes the coefficient values that matches an element of $E$ or $I$ to an element in $I$. Considering two variables $E_{i,j}$ and $I_{k,l}$, then the matrix $E\rightarrow I$ can be formally expressed by distinguishing the following 4 scenarios:
% \begin{enumerate}
% 	\item $i\neq j$, $k\neq l$.
% 	\item $i\neq j$, $k=l$.
% 	\item $i=j$, $k\neq l$.
% 	\item $i=j$, $k=l$
% \end{enumerate}
% and
% \begin{equation}
% E\rightarrow I (ij,kl)=\begin{cases}
% \beta_{inn}\frac{N_{ij}}{N_j^{P}}+ \frac{\sum_{m=1}^M c_{ij}^{m} \beta_{tra}^m g_im_{ij}N_{ii} c_{lk}^m \delta_{lk,ij}^m r_{kl}}{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m (g_km_{kj}N_{kk}+r_{jk}N_{jk})}, \text{case 1}\\
% \beta_{inn}\frac{N_{ij}}{N_j^{P}}+ \frac{\sum_{m=1}^M c_{ij}^{m} \beta_{tra}^m g_im_{ij}N_{ii} c_{lk}^m \delta_{lk,ij}^m g_km_{kj}}{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m (g_km_{kj}N_{kk}+r_{jk}N_{jk})}, \text{case 2}\\
% \beta_{inn}\frac{N_{ij}}{N_j^{P}}+\frac{\sum_{j=1,j\neq i}^P\sum_{m=1}^M c_{ji}^{m} \beta_{tra}^m r_{ij}S_{ij}c_{lk}^m \delta_{lk,ji}^m r_{kl}}{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m (r_{ik}N_{ik}+g_km_{ki}N_{kk})},\text{case 3}\\
% \beta_{inn}\frac{N_{ij}}{N_j^{P}}+\frac{\sum_{j=1,j\neq i}^P\sum_{m=1}^M c_{ji}^{m} \beta_{tra}^m r_{ij}S_{ij}c_{lk}^m \delta_{lk,ji}^m g_km_{ki}}{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m (r_{ik}N_{ik}+g_km_{ki}N_{kk})},\text{case 4}\\
% \end{cases}
% \end{equation}

% Similarly, we can express the entries of $I\rightarrow I$ by distinguishing the following scenarios:
% \begin{enumerate}
% 	\item $i\neq j$, $k=l=i$.
% 	\item $i=j$, $k\neq l$, $k=i$.
% \end{enumerate}
% and 
% \begin{equation}
% I \rightarrow I (ij,kl)=\begin{cases}
% g_im_{ij}, \text{case 1}\\
% r_{kl}, \text{case 2}\\
% 0,\text{otherwise}
% \end{cases}
% \end{equation} 

% Finally, for the matrix $N^r\rightarrow I$, we have:
% \begin{equation}
% N^r \rightarrow I (k,ij)=\begin{cases}
% \alpha_i^I, \text{if $i=j$ and $k=i$}\\
% 0,\text{otherwise}
% \end{cases}
% \end{equation} 

% This concludes the transmission matrix. And we next discuss the structure of the transition matrix, as follows.

% For the transition matrix $\Sigma$, it is more complicated and can be written as the following block form:
% \begin{equation}
% \mathbf{\Sigma}=
% \begin{blockarray}{*{3}{c} l}
% \begin{block}{*{3}{>{$\footnotesize}c<{$}} l}
% \textbf{E} & \textbf{I} & \textbf{$N^r$} & \\
% \end{block}
% \begin{block}{[*{3}{c}]>{$\footnotesize}l<{$}}
% E\rightarrow E & 0 & N^r\rightarrow E & \textbf{E} \\
% E\rightarrow I & I\rightarrow I & 0 & \textbf{I} \\
% \delta_E & \delta_I & 0 & \textbf{$N^r$} \\
% \end{block}
% \end{blockarray}
% \end{equation}

% And each block matrices take the following form:
% \begin{equation}
% E\rightarrow E(ij,kl)=\begin{cases}
% -g_i-\sigma-\alpha_i, \text{ if $i=j$ and $kl=ij$}\\
% r_{kl},\text{ if $i=j$ and $k=i$}\\
% -r_{ij}-\sigma-\alpha_i, \text{ if $i\neq j$ and $ij=kl$} \\
% g_im_{ij}, \text{if $i\neq j$ and $k=l=i$}\\
% 0, \text{otherwise} 
% \end{cases}
% \end{equation}

% \begin{equation}
% N^r \rightarrow E (k,ij)=\begin{cases}
% \alpha_i^E, \text{if $i=j$ and $k=i$}\\
% 0,\text{otherwise}
% \end{cases}
% \end{equation} 


% \begin{equation}
% E\rightarrow I(ij,kl)=\begin{cases}
% \sigma, \text{ if $ij=kl$}\\
% 0, \text{otherwise} 
% \end{cases}
% \end{equation}

% \begin{equation}
% I\rightarrow I(ij,kl)=\begin{cases}
% -g_i-\alpha_i-\gamma, \text{ if $i=j$ and $ij=kl$}\\
% -r_{ij}-\alpha_i-\gamma,\text{if $i\neq j$ and $ij=kl$}\\
% 0, \text{otherwise} 
% \end{cases}
% \end{equation}


% \begin{proposition}
% 	If $\rho(K)<1$, then the DFE is stable. If $\rho(K)>1$, the DFE is unstable. $\rho$ refers to the spectrum radius of a matrix.  
% \end{proposition}
% \begin{proof}
% 	The proof comes naturally from the definition of $R_0$. 
% \end{proof}


\section{Control the spread of disease within transportation system}
Since we have developed the model for infectious disease within transportation system, the next question to ask is that if we can control the spread of disease by placing entrance screening for transportation system. In particular, we have seen the implementation of radiation thermometers during the 2003 SARS outbreak for subway and bus systems, which aimed to screen out risky passengers with high body temperature. And additional measures such as distributing masks and random inspection by medical workers may also be efficient to reduce the risk exposure during travel. Meanwhile, placing entrance screening will also decrease system efficiency by introducing entry delays, which in return affecting the travel behavior of passengers in mode selection. This relationship is illustrated in Figure~\ref{fig:travel_equilibrium}. Specifically, we assume that the efforts (e.g., time and resource) required grows faster than the increments in control effectiveness, so that a high detection rate of infected people will result in a much higher entry delay. 
\begin{figure}[h!]
	\centering
	\includegraphics[width=80mm]{results/travel_equi.png}
	\caption{Illustration of the passenger dynamics}
	\label{fig:travel_equilibrium}
\end{figure}

While deriving the optimal control strategy will be intrinsically complicated for the proposed model, we make the first attempt to understand if it is possible to avoid the outbreaks of disease by placing controls on transportation system. In other words, our objective is to assess if a given control strategy may eventually lead to DFE state, and the problem falls into the field of safety verification. In the realistic transportation system, it is hardly possible to place the entry control for all travel modes. Instead, it is only viable to conduct such control over the medium and high capacity travel modes, such as buses and metros. As a consequence, in our study, we consider that passengers may choose from one or the following three travel modes:
\begin{enumerate}
	\item \textbf{Low capacity mode} such as private vehicles and taxis
	\item \textbf{Medium capacity mode} such as vans and buses
	\item \textbf{High capacity mode} such as metro system
\end{enumerate}

And passengers will choose the mode which maximize their utility (or the one with the least travel time). We consider rational behavior of passengers, and introduce the logistic function to quantify the model split ratio as:
\begin{equation}
S_{ij}^m=m_{ij}S_i\frac{e^{t_{ij}^m}}{\sum_{i=1}^M e^{t_{ij}^i}}
\end{equation}
\begin{equation}
I_{ij}^m=m_{ij}I_i\frac{e^{t_{ij}^m}}{\sum_{i=1}^M e^{t_{ij}^i}}
\end{equation}
We assume that the low capacity mode is not controllable, but typically having fewer passengers per vehicle and passengers having less chance of getting infected. On the contrary, passengers using medium or high capacity mode are usually exposed to much more people in a small compartment for a longer time, and are therefore having much higher chances of being infected. This assumption leads to the following requirement for the effective contact rate:
\begin{equation}
\beta_{tra}^{med}>\beta_{tra}^{large}>>\beta_{tra}^{small}
\end{equation}

Based on the discussion above, we arrive at the model which explicitly incorporates control over transportation system:

\begin{equation}
\begin{split}
	\dot{S}_{ii}=-g_{i}S_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}S_{ij}+\alpha_i^SN_i^r-\alpha_i S_{ii}-\beta_{inn}\frac{S_{ii}\sum_{j=1}^{P}I_{ji}}{N_i^p}\\
    -\sum_{j=1,j\neq i}^P\sum_{m=1}^M c_{ji}^{m} \beta_{tra}^m r_{ij}S_{ij} \frac{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m d_l^m(r_{ik}I_{ik}+g_km_{ki}I_{kk})}{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m (r_{ik}N_{ik}+g_km_{ki}N_{kk})}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
	\dot{S}_{ij}=-r_{ij}S_{ij}+g_im_{ij}S_{ii}-\alpha_i S_{ij}-\beta_{inn}\frac{S_{ij}\sum_{k=1}^{P}I_{kj}}{N_j^p}\\
    -\sum_{m=1}^M c_{ij}^{m} \beta_{tra}^m g_im_{ij}S_{ii} \frac{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m d_l^m(g_km_{kj}I_{kk}+r_{jk}I_{jk})}{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m (g_km_{kj}N_{kk}+r_{jk}N_{jk})}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
	\dot{E}_{ii}=-g_{i}E_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}E_{ij}+\alpha_i^EN_i^r-\alpha_i E_{ii}-\sigma E_{ii}+\beta_{inn}\frac{S_{ii}\sum_{j=1}^{P}I_{ji}}{N_i^p}\\
    +\sum_{j=1,j\neq i}^P\sum_{m=1}^M c_{ji}^{m} \beta_{tra}^m r_{ij}S_{ij} \frac{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m d_l^m(r_{ik}I_{ik}+g_km_{ki}I_{kk})}{\sum_{k=1,k\neq i}^P c_{ki}^m \delta_{ki,ji}^m (r_{ik}N_{ik}+g_km_{ki}N_{kk})}
\end{split}
\end{equation}

\begin{equation}
\begin{split}
	\dot{E}_{ij}=-r_{ij}E_{ij}+g_i m_{ij}E_{ii}-\alpha_i E_{ij}-\sigma E_{ij}+\beta_{inn}\frac{S_{ij}\sum_{k=1}^{P}I_{kj}}{N_j^p}\\
    +\sum_{m=1}^M c_{ij}^{m} \beta_{tra}^m g_im_{ij}S_{ii} \frac{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m d_l^m(g_km_{kj}I_{kk}+r_{jk}I_{jk})}{\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m (g_km_{kj}N_{kk}+r_{jk}N_{jk})}
\end{split}
\end{equation}

\begin{equation}
	\dot{I}_{ii}=-g_{i}I_{ii}+\alpha_i^IN_i^r-\alpha_i I_{ii}+\sum_{j=1,j\neq i}^{P}\sum_m r_{ij}d_l^mc_{ij}^mI_{ij}+\sigma E_{ii}-\gamma I_{ii}
\end{equation} 

\begin{equation}
	\dot{I}_{ij}=-r_{ij}I_{ij}-\alpha_i I_{ij}+\sum_m g_i m_{ij} c_{ij}^m d_l^m I_{ii}+\sigma E_{ij}-\gamma I_{ij}
\end{equation}

\begin{equation}
	\dot{R}_{ii}=-g_{i}R_{ii}+\alpha_i^RN_i^r-\alpha_i S_{ii}+\sum_{j=1,j\neq i}^{P}r_{ij}R_{ij}+\gamma I_{ii}+\sum_{j=1,j\neq i}^{P}\sum_m r_{ij}c_{ij}^m(1-d_l^m)I_{ij}
\end{equation}

\begin{equation}
	\dot{R}_{ij}=-r_{ij}R_{ij}+g_i m_{ij}R_{ii}-\alpha_i R_{ij}+\gamma I_{ij} +\sum_m g_i m_{ij} c_{ij}^m (1-d_l^m) I_{ii}
\end{equation}


==> part B disease_network/method_new.tex <==
\section{Modeling disease spreading with travel contagion}
\subsection{Notation}
We summarize the list of variables used in this section as follows
\begin{table}[htbp!]
	\setstretch{1.2}
	\centering
	\caption{Table of notation}
	\label{notation}
	\begin{tabular}{p{2cm}p{13.5cm}}
		\hline
		Notation & Description \\ \hline
		&\textbf{Variables}\\ \hline
		$S_{ij}$ & Susceptible population who are residents of zone $i$ and currently in zone $j$. \\
		$E_{ij}$ & Exposed (latent) population who are residents of zone $i$ and currently in zone $j$.\\
		$I_{ij}$ & Infected population who are residents of zone $i$ and currently in zone $j$. \\
		$R_{ij}$ & Recovered population who are residents of zone $i$ and currently in zone $j$.\\
		$S_{\ra{ij}},S_{\la{ij}}$ & Susceptible population in travel from $i$ to $j$ and from $j$ to $i$ respectively. Similar notations are used for $E,I$ and $R$ population.\\
		$N_i^p$ & Population at zone $i$. \\
		$N_{ij}$ & The amount of people currently at zone $j$ who are the residents of zone $i$. \\
		\hline
		&\textbf{Fixed parameters}\\ \hline
		$D$ & Total number of travel modes available. \\
		$d$ & Travel mode $d$, where $d=1,2,...,D$. \\
		$\beta^A$ & Disease transmission rate per valid contact at the activity location. \\
		$\beta_{d}^T$ & Disease transmission rate per valid contact during travel using mode $d$. \\ 
		$c_{ij}^d$ & The ratio of people who choose travel mode $d$ between zone $i$ and zone $j$. \\
		$1/\sigma$ & The expected latent duration remaining in $E$ before moving to $I$. \\ 
		$1/\gamma$ & The expected recover duration remaining in $I$ before moving to $R$. \\
		$\kappa_{ij}$ & Expected number of valid contacts for residents of $i$ who are currently at zone $j$. \\ 
		$\kappa_{ij,kl}^d$ & Expected number of valid contacts for travelers from $i$ to $j$ who come across with travelers from $k$ to $l$ using the same travel mode $d$. \\ 
		
		\hline
	\end{tabular}
\end{table}

\subsection{System dynamics}
Important components missing from the previously discussed SEIR model are the spatial movement of urban population and the transmission of infectious diseases due to contacts during travel. The model only considers local dynamics, but it is essential for urban areas to model explicitly how population flow moving around the city. In particular, these flows are driven by various activities, such as work, school, or entertainment. And people get in contact with others by taking different activities through various transportation tools. As long as some individuals are infected, their activities and the urban transportation mobility will take the disease to every corner of the city. This motivates us to understand the the spread of infectious disease in urban area by modeling the system with the following 6 dynamics: 
\begin{enumerate}
	\item The mobility dynamics of urban population follows the model as discussed in Section~\ref{sec:mobility}.
	\item Similar to the SEIR model, we consider $S_{ij}$ being affected by $I_{ij}$ with the inner-zone activity contagion rate $\beta^{A}$. 
	\item In addition to the spread of diseases due to activity engagement, we also consider people get infected during travel. That is, $S_{ij}$ may be infected by contacting with $I_{ij}$ if they use the same travel mode $d$, with the contagion rate of $\beta^T_d$. 
	\item Once people in $S_{ij}$ are infected, they become $E_{ij}$. They are not infectious until the end of the latent period, and the length of latent period is characterized by $1/\sigma$.
	\item People in $E_{ij}$ become $I_{ij}$ at the end of the latent period. And the length of the infectious period is characterized by $1/\gamma$. 
	\item At the end of their infectious period, people in $I_{ij}$ become $R_{ij}$. For simplicity, we consider that they gain permanent immunity to the disease (e.g., death, vaccinated, or fully treated) and will no longer be infected.  
\end{enumerate}

In particular, the contagion process between susceptible and infected population can be illustrated by the example of a 3-zone network as shown in Figure~\ref{fig:examp}
\begin{figure}[h!]
	\centering
	\includegraphics[width=150mm]{figure/contaillust.pdf}
	\caption{Illustration of the disease contagion process in a 3-zone network}
	\label{fig:examp}
\end{figure}
For the illustration network, there are two travel links 1-2 and 2-3 and three possible routes: from zone 1 to zone 2, from zone 1 to zone 3, and from zone 2 to zone 3. And we have two different contagions in this network. One is the inner-zone contagion which takes place between $S$ and $I$ population in the same zone (1-3). Additionally, there is travel contagion (shown in dashed line), which may happen if two population share overlay segments in their travel routes. Consequently, we have two possible travel contagions: between people travel from 1 to 2 and 1 to 3, between people travel from 1 to 3 and 2 to 3, and vice versa. While this is only an illustration, the overlay segments should also be distinguished depending on the particular mode chosen by the commuters. 

\subsection{Formulation}
With the above discussions on the system dynamics, we first differentiate the two contagion dynamics: activity contagion and travel contagion, and can be written mathematically as:
\begin{equation}
f_{ij}(S,I)=\beta^{A}_j\kappa_{ij}\frac{S_{ij}(I_j+\sum_{k=1}^{N}I_{kj})}{N_j^p}
\end{equation}
\begin{equation}
f_{i}(S,I)=\beta^{A}_i\kappa_{i}\frac{S_{i}(I_i+\sum_{k=1}^{N}I_{ki})}{N_i^p}
\end{equation}
\begin{equation}
h_{\la{ij}}(S,I)=\sum_{d=1}^D c_{ij}^{d} \beta_d^T {S}_{\la{ij}} [\sum_{k=1}^P\sum_{l=1}^P \frac{\kappa_{\la{kl},\la{ij}}^d I_{\la{kl}}}{N_{\la{kl}}}+\frac{\kappa_{\ra{kl},\la{ij}}^d I_{\ra{kl}}}{N_{\ra{kl}}}]
\label{eq:travel_return_infect}
\end{equation}
\begin{equation}
h_{\ra{ij}}(S,I)=\sum_{d=1}^D c_{ij}^{d} \beta_d^T {S}_{\ra{ij}} [\sum_{k=1}^P\sum_{l=1}^P \frac{\kappa_{\la{kl},\ra{ij}}^d I_{\la{kl}}}{N_{\la{kl}}}+\frac{\kappa_{\ra{kl},\ra{ij}}^d I_{\ra{kl}}}{N_{\ra{kl}}}]
\label{eq:travel_out_infect}
\end{equation}

Equation~\ref{eq:travel_return_infect} summarizes the S population who returns to home $i$ and get infected during travel, by encountering I population to-and-from resident location in other places. Specifically, $c_{ij}^dg_im_{ij}S_{ii}$ captures the ratio of $S_{ii}$ who leaves for destination $j$ using transportation mode $d$. $\frac{\kappa_{kl,ij}^d I_{kl}}{N_{kl}}$ denotes the contact rate with infectious population returning from $l$ to $k$, which is simplified from:
\begin{equation}
\frac{\kappa_{kl,ij}^d c_{kl}^dr_{kl} I_{kl}}{c_{kl}^dr_{kl} N_{kl}}
\end{equation}
and $\kappa_{kl,ij}^d$ refers to the number of contacts on average between ODs $kl$ and $ij$, and is a function of the travel time. Similarly, $\frac{\kappa_{kl,ij}^d I_{kk}}{N_{kk}}$ represents the contact rate with the infectious population leaving from $k$ to $l$, which is simplified from:
\begin{equation}
\frac{\kappa_{kl,ij}^d c_{kl}^dg_km_{kl}I_{kk}}{c_{kl}^dg_km_{kl}N_{kk}}
\end{equation}
With the above four different incidences for possible disease transmission, we can formally express the mathematical formulations that describe the transportation disease spreading process in urban area as follows:
\begin{eqnarray}
\begin{aligned}
\frac{E_i}{dt}=&-g_{i}E_{i}+\sum_{j=1}^{P} \alpha_{\la{ij}}E_{\la{ij}}-\sigma E_{i}+f_{i}(S,I)-\mu E_{i}\\
\frac{E_{ij}}{dt}=&-r_{ij}E_{ij}+\alpha_{\ra{ij}}E_{\ra{ij}}-\sigma E_{ij}+f_{ij}(S,I)-\mu E_{ij}\\
\frac{{E}_{\ra{ij}}}{dt}=&g_{i}m_{ij}E_{i}+h_{\ra{ij}}(S,I)-\alpha_{\ra{ij}}E_{\ra{ij}}-\sigma E_{\ra{ij}}-\mu E_{\ra{ij}}\\
\frac{{E}_{\la{ij}}}{dt}=&r_{ij}E_{ij}+h_{\la{ij}}(S,I)-\alpha_{\la{ij}}E_{\la{ij}}-\sigma E_{\la{ij}}-\mu E_{\la{ij}}\\
\frac{I_i}{dt}=&-g_{i}I_{i}+\sum_{j=1}^{P}\alpha_{\la{ij}} I_{\la{ij}}+\sigma E_{i}-\gamma I_{i}-\mu I_{i}\\
\frac{I_{ij}}{dt}=&-r_{ij}I_{ij}+\alpha_{\ra{ij}}I_{\ra{ij}}+\sigma E_{ij}-\gamma I_{ij}-\mu I_{ij}\\
\frac{{I}_{\ra{ij}}}{dt}=&g_{i}m_{ij}I_{i}-\alpha_{\ra{ij}}I_{\ra{ij}}+\sigma E_{\ra{ij}}-\gamma I_{\ra{ij}}-\mu I_{\ra{ij}}\\
\frac{{I}_{\la{ij}}}{dt}=&r_{ij}I_{ij}-\alpha_{\la{ij}}I_{\la{ij}}+\sigma E_{\la{ij}}-\gamma I_{\la{ij}}-\mu I_{\la{ij}}\\
\frac{S_i}{dt}=&-g_{i}S_{i}+\sum_{j=1}^{P}\alpha_{\la{ij}} S_{\la{ij}}-f_{i}(S,I)+\mu(N_i^r-S_{i})\\
\frac{S_{ij}}{dt}=&-r_{ij}S_{ij}+\alpha_{\ra{ij}}S_{\ra{ij}}-f_{ij}(S,I)-\mu S_{ij}\\
\frac{{S}_{\ra{ij}}}{dt}=&g_{i}m_{ij}S_{i}-h_{\ra{ij}}(S,I)-\alpha_{\ra{ij}}S_{\ra{ij}}-\mu S_{\ra{ij}}\\
\frac{{S}_{\la{ij}}}{dt}=&r_{ij}S_{ij}-h_{\la{ij}}(S,I)-\alpha_{\la{ij}}S_{\la{ij}}-\mu S_{\la{ij}}\\
\frac{R_i}{dt}=&-g_{i}R_{i}+\sum_{j=1}^{P}\alpha_{\la{ij}} R_{\la{ij}}+\gamma I_{i}-\mu R_{i}\\
\frac{R_{ij}}{dt}=&-r_{ij}R_{ij}+\alpha_{\ra{ij}}R_{\ra{ij}}+\gamma I_{ij}-\mu R_{ij}\\
\frac{{R}_{\ra{ij}}}{dt}=&g_{i}m_{ij}R_{i}-\alpha_{\ra{ij}}R_{\ra{ij}}+\gamma I_{\ra{ij}}-\mu R_{\ra{ij}}\\
\frac{{R}_{\la{ij}}}{dt}=&r_{ij}R_{ij}-\alpha_{\la{ij}}R_{\la{ij}}+\gamma I_{\la{ij}}-\mu R_{\la{ij}}\\
\end{aligned}
\label{eq:seir_system}
\end{eqnarray}

The system described by equation~\ref{eq:seir_system} can be easily understood by decomposing each equation into the part of mobility dynamics and the part of disease dynamics. For the mobility dynamics, the system of equations is consistent with the mobility model which captures the movement of $S,E,I,R$ population across the city as well as the death and birth (only into susceptible population). As for the disease dynamics, it involves the migration of population between compartments following the contagion process, the end of latent period and the end of infectious period. 

% The disease dynamics of equation~\ref{eq:sii} has two components. The first component with the coefficient $\beta_{inn}$ characterizes the within zone spread of diseases, where $\sum_jI_{ji}$ refers to total infected population in zone $i$ and the contagion has the bilinear incident form which is consistent with the SEIR model. The second component which is associated with the coefficient $\beta_{tra}$ denote the spread of diseases during travel. Specifically, this term describes how susceptible people who return from $j$ to $i$ get in contact with infectious population. For the contagion to take place, $S$ and $I$ must be in the same travel mode and share trip segment(s) in common. And the indicator variable $\delta_{ki,ji}^m$ is introduced to indicate if trips made from $k$ to $i$ and from $j$ to $i$ using travel mode $m$ have overlapping parts. And the infected $S_{ii}$ are added to $E_{ii}$ as shown in equation~\ref{eq:eii}. Moreover, $E_{ii}$ and $I_{ii}$ (or equation~\ref{eq:eii} and~\ref{eq:iii}) are connected by the term $\sigma E_{ii}$, which implies the end of latent period. Similarly, $I_{ii}$ and $R_{ii}$ (or equation~\ref{eq:iii} and~\ref{eq:rii}) are correlated by the term $\gamma I_{ii}$.

% On the other hand, the disease dynamics for equation~\ref{eq:sij} also involves two components. The first component with the coefficient $\beta_{inn}$ captures how $S_{ij}$ gets infected during the contagion with other infected population. The second component with the coefficient $\beta_{tra}$ describes the spread of diseases while people are traveling from $i$ to $j$. That is, only departed population $g_jm_{ij}S_{ii}$ may have the chance of being infected during their travel to $j$. And the contagion may happen when they get in contact with departed infectious population who have the same destination using the same mode, which is captured by $\sum_{k=1,k\neq j}^P c_{kj}^m \delta_{kj,ij}^m g_km_{kj}I_{kk}$. And both parts of infected $S_{ij}$ are added to $E_{ij}$ as shown in equation~\ref{eq:eij}. Finally, we have the same correlations between $E_{ij}$ and $I_{ij}$, and between $I_{ij}$ and $R_{ij}$, as discussed in the previous paragraph. This concludes the basic model for characterizing disease dynamics with travel contagion. 

\begin{prop}
	Based on equation~\ref{eq:seir_system}, we can decompose the system into $\mathcal{F}-\mathcal{V}$ where we have
	\begin{equation}
	\mathcal{F}=
	\begin{bmatrix}
	f_{i}\\
	f_{ij}\\
	h_{\ra{ij}}\\
	h_{\la{ij}}\\
	0\\
	0\\
	0\\
	0
	\end{bmatrix}
	, \mathcal{V}=
	\begin{bmatrix}
	(g_{i}+\mu+\sigma)E_{i}-\sum_{j=1}^{P} \alpha_{\la{ij}}E_{\la{ij}}\\
	(r_{ij}+\mu+\sigma)E_{ij}-\alpha_{\ra{ij}}E_{\ra{ij}} \\
	(\mu+\sigma+\alpha_{\ra{ij}})E_{\ra{ij}}-g_{i}m_{ij}E_{i}\\
	(\mu+\sigma+\alpha_{\la{ij}})E_{\la{ij}}-r_{ij}E_{ij}\\
	(g_{i}+\mu+\gamma)I_{i}-\sum_{j=1}^{P} I_{\la{ij}}-\sigma E_{i}\\
	(r_{ij}+\mu+\gamma)I_{ij}-\alpha_{\ra{ij}}I_{\ra{ij}}-\sigma E_{ij}\\
	(\mu+\gamma+\alpha_{\ra{ij}})I_{\ra{ij}}-g_{i}m_{ij}I_{i}-\sigma E_{\ra{ij}}\\
	(\mu+\gamma+\alpha_{\la{ij}})I_{\la{ij}}-r_{ij}I_{ij}-\sigma E_{\la{ij}}\\
	\end{bmatrix}
	\end{equation}
\end{prop}




Considering that an infectious disease has been introduced into a city and follows the system described in equation~\ref{eq:seir_system}, an essential question to be answered is that if the disease will eventually invade the population. Specifically, the above system compromises two equilibrium points as following: 
\begin{defn}
	The disease dynamic system characterized by equation 5.1-5.8 has two equilibrium points. The first equilibrium point $x_0$ is the disease free equilibrium (DFE):
	\begin{equation}
	S_{ij}=N_{ij},E_{ij}=I_{ij}=R_{ij}=0
	\end{equation}
	\begin{equation}
	x_0=(N,0,0,0)
	\end{equation}
	The second equilibrium point is the endemic equilibrium with:
	\begin{equation}
	\sum_{ij} I_{ij}>0
	\end{equation}
	such that a strictly positive fraction population will be in the infectious state.  
\end{defn}

To address the previous question, it requires the understanding of the stability of disease free equilibrium (DFE). In particular, if the DFE is stable, then the disease will be absent from the population, otherwise it is always possible for disease outbreak. We next discuss the stability of the DFE with the presented Trans-SEIR model. 


\subsection{Model analysis}
To better analyze the model properties, we first rearrange the modeling parameters in the following order:
\[
E_{1},E_{11}, E_{\ra{11}},E_{\la{11}}, E_{12}, E_{\ra{12}},E_{\la{12}},\dots,E_{\la{nn}},I_{1},I_{11} I_{\ra{11}},I_{\la{11}},\dots
\]
with $E_{\la{ii}},I_{\la{ii}},E_{\ra{ii}},I_{\ra{ii}}$ being strictly zero as we do not consider within zone travels. We denote $Z_i^E$ and $Z_i^I$ as the set of $E$ and $I$ population compartments that are associated with residents of zone $i$, e.g., $Z_i^E=\{E_{11}, E_{\ra{11}},E_{\la{11}}, E_{12},...,E_{\la{nn}}\}$. 

If we linearize the system at the DFE point $x_0$, we have $D\mathcal{F}(x_0)$ as:
\begin{equation}
D\mathcal{F}(x_0)=\begin{bmatrix}
0 & 0 & \frac{df_{ii}(x_0)}{d I_{ii}}+\frac{dh_{ii}(x_0)}{d I_{ii}} & \frac{df_{ii}(x_0)}{d I_{ij}}+\frac{dh_{ii}(x_0)}{d I_{ij}} \\
0 & 0 &\frac{df_{ij}(x_0)}{d I_{ii}}+\frac{dh_{ij}(x_0)}{d I_{ii}} & \frac{df_{ij}(x_0)}{d I_{ij}}+\frac{dh_{ij}(x_0)}{d I_{ij}} \\
0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 \\
\end{bmatrix}
\end{equation}

We can further partition matrix $V$ as in the following format:
\begin{equation}
V=\begin{bmatrix}
V_E & \bigzero \\
-\Sigma & V_I\\
\end{bmatrix}=\left[\begin{array}{@{}c|c@{}}
\begin{matrix}
V_{E}(1) &  &  \\
& \ddots & \\
& & V_{E}(n)
\end{matrix}
& \bigzero \\
\hline
-\Sigma &
\begin{matrix}
\begin{matrix}
V_{I}(1) &  &  \\
& \ddots & \\
& & V_{I}(n)
\end{matrix}
\end{matrix}
\end{array}\right]
\end{equation}

where $\Sigma$ represents the diagonal matrix of $\sigma$. We use $V_E(i)$, with dimension $3n+1\times3n+1$, to represent the block Jacobian matrix with respect to elements the corresponding population compartments in $\{i1,i2,...,in\}$. We can formally express each block of the corresponding matrix as:

\begin{equation}
V_E(i)=
\tiny
\begin{blockarray}{ccccccccccc}
\small
E_{i1} & E_{\ra{i1}} &  E_{\la{i1}} & \dots & E_{i} & \dots & E_{in} & E_{\ra{in}} &  E_{\la{in}} \\
& & & & & & & & & &\\
\begin{block}{[cccccccccc]l}
r_{i1}+\mu+\sigma &-\alpha_{\ra{i1}}& & & & & & & & & E_{i1}\\
&  \alpha_{\ra{i1}}+\mu+\sigma & &  & -g_im_{i1} & & & & & & E_{\ra{i1}}\\ 
-r_{i1} & &  \alpha_{\la{i1}}+\mu+\sigma& & \vdots & & & & & & E_{\la{i1}} \\
& & &  \ddots   & & & & & & & \vdots\\
& & -\alpha_{\la{i1}}& \dots & g_i+\mu+\sigma  & \dots & & &  -\alpha_{\la{in}} & & E_{i}\\
& & & &\vdots &  \ddots & & & & & \vdots\\
& & & & & &  r_{in}+\mu+\sigma &-\alpha_{\ra{in}} &  & & E_{in}\\
& & & &-g_im_{in} & & &   \alpha_{\ra{in}}+\mu+\sigma & & &  E_{\ra{in}} \\
& & & & & &-r_{in} &  &   \alpha_{\la{in}}+\mu+\sigma & & E_{\la{in}}\\
\end{block}
\end{blockarray}
\end{equation}

Finally, we have the same formulation for the corresponding block diagonal matrices ($V_I(i)$) of $I$, with the only differences being that all $\sigma$ are replaced by $\gamma$. As a consequence, $V$ is a lower-triangular matrix. 

As for the transmission part of the formulation which corresponds to the new generation of infectious population, we should have:

\begin{equation}
\mathcal{F}=\left[\begin{array}{@{}c|c@{}}
\bigzero &  F+H\\
\hline
\bigzero & \bigzero 
\end{array}\right]
\end{equation}
In the equation, $F$ represents the disease transmission that are related to local compartments and $H$ accounts for all transmissions that happen during travel. In this regard, we can also break $F+H$ into $n^2$ blocks of matrix with each block $(F+H)(Z_i^E,Z_j^I)$ being a $3n\times 3n$ matrix of the following form: 

\begin{equation}
F+H=\begin{bmatrix}
F+H(Z_1^E,Z_1^I) & \dots & F+H(Z_1^E,Z_n^I) \\
F+H(Z_2^E,Z_1^I) & \dots & F+H(Z_2^E,Z_n^I)  \\
\vdots & \ddots & \vdots\\
F+H(Z_n^E,Z_1^I) & \dots & F+H(Z_n^E,Z_n^I) 
\end{bmatrix},
\end{equation}

\begin{equation}
(F+H)(Z_i^E,Z_j^I)=
\tiny
\begin{blockarray}{cccccccc}
\small
I_{j1} & I_{\ra{j1}} &  I_{\la{j1}} & \dots & I_{jn} & I_{\ra{jn}} &  I_{\la{jn}} \\
& & & & & & \\
\begin{block}{[ccccccc]l}
\beta_1^A\kappa_{i1}\frac{N_{i1}}{N_1^p} & & &  & & & &   \dot{E}_{i1}\\
& h_{\ra{i1},\ra{j1}}& h_{\ra{i1},\la{j1}} & \dots & & h_{\ra{i1},\ra{jn}}& h_{\ra{i1},\la{jn}} & \dot{E}_{\ra{i1}}\\ 
& h_{\la{i1},\ra{j1}} & h_{\la{i1},\la{j1}} & \dots & & h_{\la{i1},\ra{jn}} & h_{\la{i1},\la{jn}} & \dot{E}_{\la{i1}} \\
& & &  \ddots   & & & & \vdots\\
& & &  & \beta_n^A\kappa_{in}\frac{N_{in}}{N_n^p} & & &  \dot{E}_{in}\\
& h_{\ra{in},\ra{j1}}& h_{\ra{in},\la{j1}}& \dots & & h_{\ra{in},\ra{jn}}& h_{\ra{in},\la{jn}} & \dot{E}_{\ra{in}}\\
& h_{\la{in},\ra{j1}} & h_{\la{in},\la{j1}} & \dots & & h_{\la{in},\ra{jn}} & h_{\la{in},\la{jn}} & \dot{E}_{\la{in}}\\
\end{block}
\end{blockarray}
\end{equation}

and each $h$ being represented as:
\begin{equation}
\begin{aligned}
h_{\la{ij},\ra{kl}}=\sum_{d=1}^D c_{ij}^{d} \beta_d^T\kappa_{\ra{kl},\la{ij}}^d  \frac{{N}_{\la{ij}}}{N_{\ra{kl}}}, \quad h_{\ra{ij},\ra{kl}}=\sum_{d=1}^D c_{ij}^{d} \beta_d^T\kappa_{\ra{kl},\ra{ij}}^d  \frac{{N}_{\ra{ij}}}{N_{\ra{kl}}}\\
h_{\la{ij},\la{kl}}=\sum_{d=1}^D c_{ij}^{d} \beta_d^T\kappa_{\la{kl},\la{ij}}^d  \frac{{N}_{\la{ij}}}{N_{\la{kl}}},\quad h_{\ra{ij},\la{kl}}=\sum_{d=1}^D c_{ij}^{d} \beta_d^T\kappa_{\la{kl},\ra{ij}}^d  \frac{{N}_{\ra{ij}}}{N_{\la{kl}}}\\
\end{aligned}
\end{equation}



\begin{prop}
	$V_E(i)$ and $V_I(i)$ in $V$ are invertible and $V_E(i)^{-1}$ and $V_I(i)^{-1}$ are strictly positive. 
	\label{prop:inverse}
\end{prop}
\begin{proof}
	Since $V_E(i)$ and $V_I(i)$ have similar structure, without loss of generality, we here only show that $V_E(i)$ is invertible and same argument can be applied to $V_I(i)$.
	
	We note that, for $V_E(i)$, all diagonal elements are strictly positive and all off diagonal elements are either zero or strictly negative. In this regard, $V_E(i)$ satisfies the Z-sign pattern. In addition, we have the column sum for each column of $V_E(i)$ being $\mu+\sigma$, which is also strictly positive. This suggests that all eigenvalues of $V_E(i)$ have positive real part. This combines with the Z-sign pattern imply that $V_E(i)$ is a non-singular M-matrix and this leads to $V_E(i)^{-1}>0$. 
\end{proof}

Based on Proposition~\ref{prop:inverse}, we can write the inverse of $V$ as following:
\begin{equation}
V^{-1}=\begin{bmatrix}
V_E^{-1} & 0 \\
V_I^{-1}\Sigma V_E^{-1} & V_I^{-1}\\
\end{bmatrix}
\end{equation}

And $FV^{-1}$ is expressed as:
\begin{equation}
FV^{-1}=\begin{bmatrix}
(F+H) V_I^{-1}\Sigma V_E^{-1} & HV_I^{-1} \\
0 & 0
\end{bmatrix}
\label{eq:r0final}
\end{equation}

As the (1,1) entry in equation~\ref{eq:r0final} denotes the number of secondary infections that a new entrance in $E$ will produce, we can therefore determine the basic reproduction number ($R_0$) by
\begin{equation}
R_0=\sigma \rho((F+H) (V_EV_I)^{-1})
\label{eq:R0_value}
\end{equation}
where $\rho$ refers to the spectral radius (the real part of the largest eigenvalue) and $(V_EV_I)^{-1}$ is a block diagonal matrix. 
\begin{prop}
	The average number of secondary infectious due to a single infectious person into a fully susceptible population is given by $R_0=\rho\{(F+H)V^{-1}\}$, with $\rho$ denoting the spectral radius. In addition, if $R_0<1$ then the DFE is locally asymptotically stable. Otherwise the DFE is unstable and the disease will invade the population. 
	\label{prop:r0}
\end{prop}

We omit the proof of Proposition~\ref{prop:r0} as it follows directly from Theorem 2 in~\cite{van2002reproduction}. Note that the each entry in $F+H$ has specific physical interpretations, with the $(ij,kl)$th entry representing the new infections that an additional infectious person in $kl$ compartment will produce in the $ij$ compartment. Consequently, each eigenvalue corresponds to the column of $(F+H)V^{-1}$ refers to the $R_0$ value of that particular compartment, and that the $R_0^i$ for zone $i$ is determined by the largest $R_0$ value among all compartments that are associated with the residents of $i$.

We further observe that the column sum of $V_E$ is $\mu+\sigma$, and the column sum of $V_I$ is $\mu+\gamma$. As a result, the row sum of each column in $(V_EV_I)^{-1}$ is given by $\frac{1}{(\mu+\gamma)(\mu+\sigma)}$. Since $(V_EV_I)$ is a block diagonal matrix, so is $(V_EV_I)^{-1}$. Then for the $ij$th column of the $i$th block, only the entries in rows $i1,...,\la{in}$ may be non-zero and all other entries of the column are strictly 0. Then we can write out the vector for column sum $C_{ij}$ explicitly as:
\begin{eqnarray}
\begin{aligned}
C_{ij}&=\mathbbm{1}^{\intercal}(\sum_i f_i (V_EV_I)^{-1}_{ij}+h (V_EV_I)^{-1}_{ij})\\
& = \beta_1^A\kappa_{11}\frac{N_{11}}{N_1^p}v_{ij,i1}+\dots+\beta_n^A\kappa_{1n}\frac{N_{1n}}{N_n^p}v_{ij,in}+\beta_1^A\kappa_{21}\frac{N_{21}}{N_1^p}v_{ij,i1}+\dots+\beta_n^A\kappa_{2n}\frac{N_{2n}}{N_n^p}v_{ij,in}+\dots+ \beta_n^A\kappa_{nn}\frac{N_{nn}}{N_n^p}v_{ij,in}\label{zone_inf}\\
&\,+\sum_{m=1}^n(\sum_{k=1}^n\sum_{l=1}^n h_{\ra{kl},\ra{im}}+h_{\la{kl},\ra{im}})v_{ij,\ra{im}}+(\sum_{k=1}^n\sum_{l=1}^n h_{\ra{kl},\la{im}}+h_{\la{kl},\la{im}})v_{ij,\la{im}}\\
& =\sum_{m=1}^n (\beta_m^A\kappa_{1m}\frac{N_{1m}}{N_m^p}+\dots+\beta_m^A\kappa_{nm}\frac{N_{nm}}{N_m^p})v_{ij,im}\\
&\,+\sum_{m=1}^n (\sum_{k=1}^n\sum_{l=1}^n h_{\ra{kl},\ra{im}}
+h_{\la{kl},\ra{im}})v_{ij,\ra{im}}+(\sum_{k=1}^n\sum_{l=1}^n h_{\ra{kl},\la{im}}+h_{\la{kl},\la{im}})v_{ij,\la{im}}\\
\end{aligned}
\end{eqnarray}

As the column sum of $C_{ij}$ equals $\frac{1}{(\mu+\gamma)(\mu+\sigma)}$, we then have
\begin{equation}
\sum_{m=1}^n v_{ij,im} = \frac{1}{(\mu+\gamma)(\mu+\sigma)}
\end{equation}

Denote $\beta_{min}^A\kappa_{min}$ and $\beta_{max}^A\kappa_{max}$ be the the greatest of all activity compartments, e.g., 
\begin{equation}
\beta_{max}^A\kappa_{max}=\max_{i,j=1,...,n} \beta_i^A\kappa_{ji},\quad \beta_{min}^A\kappa_{min}=\min_{i,j=1,...,n} \beta_i^A\kappa_{ji}
\end{equation}
and $h_{max}$ and $h_{min}$ as the the trip segment with the highest and lowest contagious rate:
\begin{equation}
h_{max}=\max\{\max_{i,j=1,...,n} \sum_{k=1}^n\sum_{l=1} h_{\ra{kl},\ra{ij}}
+h_{\la{kl},\ra{ij}},\max_{i,j=1,...,n} \sum_{k=1}^n\sum_{l=1} h_{\ra{kl},\la{im}}+h_{\la{kl},\la{im}}\}
\end{equation}
\begin{equation}
h_{min}=\min\{\min_{i,j=1,...,n} \sum_{k=1}^n\sum_{l=1} h_{\ra{kl},\ra{ij}}
+h_{\la{kl},\ra{ij}},\min_{i,j=1,...,n} \sum_{k=1}^n\sum_{l=1} h_{\ra{kl},\la{im}}+h_{\la{kl},\la{im}}\}
\end{equation}
Then we have \begin{equation}
\frac{\min \{\beta_{min}^A\kappa_{min},h_{min}\}}{(\mu+\sigma)(\mu+\gamma)}  \leq C \leq  \frac{\max \{\beta_{max}^A\kappa_{max},h_{max}\}}{(\mu+\sigma)(\mu+\gamma)}
\end{equation}
and
\begin{equation}
\frac{\sigma \min \{\beta_{min}^A\kappa_{min},h_{min}\}}{(\mu+\sigma)(\mu+\gamma)}  \leq R_0\leq   \frac{\sigma \max \{\beta_{max}^A\kappa_{max},h_{max}\}}{(\mu+\sigma)(\mu+\gamma)}
\end{equation}

\begin{cor}
	Let $\beta_{max}^A\kappa_{max}$ be the highest within zone contagion rate of all zones, and $\beta_{min}^A\kappa_{min}$  be the lowest within zone contagion rate of all zones. If we assume $\kappa_{ij}$ being the same at all activity locations, then $R_0$ is bounded by the travel segments with the highest contagion rate. 
	\label{col:R0}
\end{cor} 
% \begin{proof}
%     Based on equation~\ref{eq:bound_r0}, when $\kappa_{ij}$ is homogeneous across all zones, the formulation reduces to 
%     \begin{equation}
%         C_{m}= \frac{\beta_m^A\kappa+\sum_{k=1}^n\sum_{l=1}^n h_{kl,mj}}{(\mu+\gamma)(\mu+\sigma)} \leq \frac{\beta_m^A\kappa+\max_{m,j=1,...,N} \sum_{k=1}^n\sum_{l=1}^n h_{kl,mj}}{(\mu+\gamma)(\mu+\sigma)}
%     \end{equation}

%     Moreover, we know that when $R_0<1$, the disease will be DFE. As a consequence, if 
%     \begin{equation}
%         \beta_{max}^A\kappa_{max}+\max_{m,j=1,...,N} \sum_{k=1}^n\sum_{l=1}^n h_{kl,mj} < \frac{(\mu+\sigma)(\mu+\gamma)}{\sigma}
%     \end{equation}
%     Then the disease will be DFE. 
%     And if 
%     \begin{equation}
%         \beta_{min}^A\kappa_{min}+\min_{m,j=1,...,N} \sum_{k=1}^n\sum_{l=1}^n h_{kl,mj} > \frac{(\mu+\sigma)(\mu+\gamma)}{\sigma}
%     \end{equation}
%     Then the disease is unstable. 
% \end{proof}


\section{Control the spread of disease within urban transportation system}
With the Trans-SEIR model capturing the mobility and disease dynamics, we next investigate the research question on the control of infectious diseases by placing entrance screening for transportation system. In particular, we have seen the implementation of radiation thermometers during the 2003 SARS, 2012 MERS and 2020 COVID-19 outbreaks at subway and bus stations and major transportation hubs. The entrance screening aims to identify passengers at risk with abnormal body temperature or susceptible symptoms. And additional measures such as distributing masks and random inspection by medical workers at the entrance of transportation systems may also be efficient to reduce the risk exposure during travel. While entrance screening can be of great value for the preventative purpose before the actual outbreak or to slow down the invasion of diseases during an outbreak, there is a trade-off among the success rate of screening, the amount of travelers that need to be examined and the incurred externalities such as excessive entry delays and limited manpower and medical resources. In this regard, the essential issue to be addressed is how to optimally distribute the available resources over the urban transportation systems to effectively curb the spread of infectious diseases. 

For the real-world transportation system, it is hardly possible to perform the entry control for all travel modes. Instead, it is only viable to conduct such control over the medium and high capacity travel modes, such as buses and metros. As a consequence, in our study, we assume that the travel modes are divided into three categories:
\begin{enumerate}
	\item \textbf{Low capacity mode} such as private vehicles and taxis
	\item \textbf{Medium capacity mode} such as vans and buses
	\item \textbf{High capacity mode} such as metro system
\end{enumerate}
We do not consider the low capacity mode as the control target, and the low capacity mode typically has fewer passengers per vehicle and therefore constituting the lowest chance of getting infected. On the contrary, passengers using medium or high capacity mode are usually exposed to more co-riders in an enclosed compartment for longer trip duration, and are therefore prone to higher chance of being infected. To frame the optimal entrance control problem, we introduce additional parameters $\epsilon$ and $\xi$, where $\xi$ denotes the success rate of screening of infectious travelers and $\epsilon_{ij}$ represents the fraction of passengers traveling between $i$ and $j$ that will be screened, with $\epsilon_{ij}\in[0,1]$. For simply, here we only consider that the same $\xi$ and $\epsilon_{ij}$ will be applied to all different modes, which can be easily extended to account for mode-specific control parameters. 
% \begin{equation}
% \beta_{tra}^{med}>\beta_{tra}^{large}>>\beta_{tra}^{small}
% \end{equation}
% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=80mm]{results/travel_equi.png}
% 	\caption{Illustration of the passenger dynamics}
% 	\label{fig:travel_equilibrium}
% \end{figure}


As the first step of framing the optimal control problem, we focus on scenario without resource constraint and entrance control alters the disease dynamics by reducing the number of infectious passengers entering the travel compartments $I_{\ra{ij}}$ and $I_{\la{ij}}$ once they are identified to be infected at the entrance. We consider that the identified infectious passengers will be permanently quarantined until they are no longer infectious, so that they join the recovered travel compartments $R_{\ra{ij}}$ and $R_{\la{ij}}$ respectively and shall no longer produce further infections. In this regard, we can rewrite part of the disease system as: 
\begin{eqnarray}
\begin{aligned}
\frac{{I}_{\ra{ij}}}{dt}=&(1-\epsilon_{\ra{ij}})g_{i}m_{ij}I_{ii}-\alpha_{\ra{ij}}I_{\ra{ij}}+\sigma E_{\ra{ij}}-\gamma I_{\ra{ij}}-\mu I_{\ra{ij}}\\
\frac{{I}_{\la{ij}}}{dt}=&(1-\epsilon_{\la{ij}})r_{ij}I_{ij}-\alpha_{\la{ij}}I_{\la{ij}}+\sigma E_{\la{ij}}-\gamma I_{\la{ij}}-\mu I_{\la{ij}}\\
\frac{{R}_{\ra{ij}}}{dt}=&g_{i}m_{ij}(R_{ii}+\epsilon I_{ii})-\alpha_{\ra{ij}}R_{\ra{ij}}+\gamma I_{\ra{ij}}-\mu R_{\ra{ij}}\\
\frac{{R}_{\la{ij}}}{dt}=&r_{ij}(R_{ij}+\epsilon I_{ij})-\alpha_{\la{ij}}R_{\la{ij}}+\gamma I_{\la{ij}}-\mu R_{\la{ij}}\\
\end{aligned}
\label{eq:control}
\end{eqnarray}
so that the whole disease system is still well defined and the summation of all population still equals $N$. Without loss of generality, we consider the corresponding control effectiveness of the mode $m$ being $\epsilon^m$, then $\epsilon$ simply refers to
\begin{equation}
\epsilon_{ij}=\sum_{m}c_{ij}^m\epsilon^m
\end{equation}By controlling the system without resource limitation, we may let $\epsilon=1$, e.g. all travelers will be examined, and the resulting system dynamics can be decomposed into  $F-\tilde{V}$ where $\tilde{V}$ takes the form:

\begin{equation}
\tilde{V}=\begin{bmatrix}
V_E & \bigzero \\
-\Sigma & \tilde{V}_I\\
\end{bmatrix}=\left[\begin{array}{@{}c|c@{}}
\begin{matrix}
V_{E}(1) &  &  \\
& \ddots & \\
& & V_{E}(n)
\end{matrix}
& \bigzero \\
\hline
-\Sigma &
\begin{matrix}
\begin{matrix}
\tilde{V}_{I}(1) &  &  \\
& \ddots & \\
& & \tilde{V}_{I}(n)
\end{matrix}
\end{matrix}
\end{array}\right]
\end{equation}
Specifically, $\tilde{V}_{I}(i)$ has the same diagonal elements of $V_{I}(i)$ but all its off-diagonal elements are zero. In this regard, each $\tilde{V}_I(i)$ is also a diagonal matrix and hence of larger dominant eigenvalue as compared to $V_I(i)$, suggesting an overall shorter infection period for the travelers. Following the same approach as discussed in the previous section, we can derive the reproduction number after transit control as:
\begin{equation}
\tilde{R}_0=\rho(F\tilde{V}^{-1})
\end{equation}
With curbing the spread of infectious through transportation control as the primary goal, we seek to identify proper $\epsilon$ to minimize the $\tilde{R}_0$, and the gap between $R_0$ and $\tilde{R}_0$ is therefore the reduction by controlling travel contagion. We note, however, there is no clean and close representation to formulate the relationship between $\epsilon$ and $\tilde{R}_0$, which creates a barrier for devising optimal allocation strategy of limited resources. To overcome this barrier, we seek an alternate approach to avoid this complication and build the connection between the two variables through a modified next generation matrix where we have
\begin{equation}
F(\epsilon)=\left[\begin{array}{@{}c|c@{}}
\bigzero &  F+H\\
\hline
\bigzero & \bar{V_I}(\epsilon),
\end{array}\right],
\tilde{V}=\begin{bmatrix}
V_E & \bigzero \\
-\Sigma & \tilde{V}_I\\
\end{bmatrix}
\end{equation}

where $\tilde{V}_I$ contains only the diagonal elements of $V_I$ and $-\bar{V}_I$ includes all the off-diagonal entries of $V_I$:
\begin{equation}
\bar{V}_I(i,\epsilon)=\tiny
\begin{blockarray}{ccccccccccc}
\small
I_{i1} & I_{\ra{i1}} &  I_{\la{i1}} & \dots & I_{i} & \dots & I_{in} & I_{\ra{in}} &  I_{\la{in}} \\
& & & & & & & & & &\\
\begin{block}{[cccccccccc]l}
& \alpha_{\ra{i1}}& & & & & & & & & I_{i1}\\
&   & &  & (1-\epsilon_{\ra{i1}})g_im_{i1} & & & & & & I_{\ra{i1}}\\ 
(1-\epsilon_{\la{i1}})r_{i1} & &  & & \vdots & & & & & & I_{\la{i1}} \\
& & &  \ddots   & & & & & & & \vdots\\
& & \alpha_{\la{i1}}&   & \dots & & &  & \alpha_{\la{in}} & & I_{i}\\
& & & &\vdots &  \ddots & & & & & \vdots\\
& & & & & &   &\alpha_{\ra{in}} &  & & I_{in}\\
& & & &(1-\epsilon_{\ra{in}})g_im_{in} & & &    & & &  I_{\ra{in}} \\
& & & & & &(1-\epsilon_{\la{in}})r_{in} &  &    & & I_{\la{in}}\\
\end{block}
\end{blockarray}
\end{equation}

We denote $\tilde{K}$ as the next generation matrix following $F(\epsilon)\tilde{V}^{-1}$ and $K$ being the original next generation matrix. We have the following propositions
\begin{prop}
	$R_0>1$ if and only if $\tilde{R}_0>1$, $R_0$=0 if and only if $\tilde{R}_0=0$, and $R_0<1$ if and only if $\tilde{R}_0<1$
	\label{prop:equivalence}
\end{prop}
\begin{proof}
	We have that $R_0=1$ while $s(F-V)=0$, and $R_0>1$ if $s(F-V)>0$, and $R_0<1$ if $s(F-V)<0$. By deriving $\tilde{R}_0$, we see that the corresponding $F-\tilde{V}$ still holds. This completes the proof. 
\end{proof}

\begin{prop}
	A disease is controllable through entrance screening in transportation system if and only if $\rho(F(1)\tilde{V}^{-1})<1$. 
	\label{prop:control_disease}
\end{prop}
The proof for Proposition~\ref{prop:control_disease} follows from the results of Proposition~\ref{prop:equivalence}, where $\rho(F(1)\tilde{V}^{-1})$ suggests that $\tilde{R}_0<1$ when $\epsilon=1$ and $\tilde{R}_0<1$ is equivalent to $R_0<1$. Hence the proposition states that the disease is controllable through public transportation if we may have access to unlimited resources to completely quarantine all infectious travelers and reduce the $R_0$ lower than 1. 

In addition, Proposition~\ref{prop:equivalence} states that the we can focus on controlling $\tilde{R}_0$ instead of $R_0$ to mitigate the impact from infectious disease, and more importantly eliminating the disease if we can lower $\tilde{R}_0$ to be smaller than 1. Cautions should be exercised, however, as $\tilde{R}_0$ does not have the same physical meaning as $R_0$ and can not be interpreted as the number secondary infections. Based on this equivalency, we can rephrase Corollary~\ref{col:R0} to derive the corresponding value for $\tilde{R}_0$ by measuring the column sum for $F(\epsilon)\tilde{V}^{-1}$ as:
\begin{equation}
\begin{aligned}
&\tilde{C}_{ij}(\epsilon)=\mathbbm{1}^{\intercal}(\sum_i f_i (V_E\tilde{V}_I)^{-1}_{ij}+h (V_E\tilde{V}_I)^{-1}_{ij}+\bar{V}(V_E\tilde{V}_I)^{-1}_{ij})\\
& = \frac{\beta_1^A\kappa_{11}+\sum_{j=1}^p (1-\epsilon_{\ra{1j}})g_1m_{1j}}{g_1+\gamma+\mu}\frac{N_{11}}{N_1^p}\tilde{v}_{ij,i1}+\dots+\frac{\beta_n^A\kappa_{1n}+(1-\epsilon_{\la{1n}})r_{1n}}{r_{1n}+\gamma+\mu}\frac{N_{1n}}{N_n^p}\tilde{v}_{ij,in} \\
&+\frac{\beta_1^A\kappa_{21}+(1-\epsilon_{\la{21}})r_{21}}{r_{21}+\gamma+\mu}\frac{N_{21}}{N_1^p}\tilde{v}_{ij,i1}+\dots+\frac{\beta_n^A\kappa_{2n}+(1-\epsilon_{\la{2n}})r_{2n}}{r_{2n}+\gamma+\mu}\frac{N_{2n}}{N_n^p}\tilde{v}_{ij,in}+\dots+ \frac{\beta_n^A\kappa_{nn}+\sum_{j=1}^p (1-\epsilon_{\ra{nj}})g_nm_{nj}}{g_n+\gamma+\mu}\frac{N_{nn}}{N_n^p}\tilde{v}_{ij,in}\label{zone_inf}\\
&\,+\sum_{m=1}^n(\sum_{k=1}^n\sum_{l=1}^n \frac{h_{\ra{kl},\ra{im}}+h_{\la{kl},\ra{im}}+2\alpha_{\ra{im}}}{\alpha_{\ra{im}}+\gamma+\mu})\tilde{v}_{ij,\ra{im}}+(\sum_{k=1}^n\sum_{l=1}^n \frac{h_{\ra{kl},\la{im}}+h_{\la{kl},\la{im}}+2\alpha_{\la{im}}}{\alpha_{\la{im}}+\gamma+\mu})\tilde{v}_{ij,\la{im}}\\
& =\sum_{m=1}^n (\frac{\beta_m^A\kappa_{1m}+(1-\epsilon_{\la{im}})r_{im}}{r_{im}+\gamma+\mu}\frac{N_{1m}}{N_m^p}+\dots+\frac{\beta_m^A\kappa_{nm}+(1-\epsilon_{\la{nm}})r_{nm}}{r_{nm}+\gamma+\mu}\frac{N_{nm}}{N_m^p})\tilde{v}_{ij,im}\\
&\,+\sum_{m=1}^n(\sum_{k=1}^n\sum_{l=1}^n \frac{h_{\ra{kl},\ra{im}}+h_{\la{kl},\ra{im}}+2\alpha_{\ra{im}}}{\alpha_{\ra{im}}+\gamma+\mu})\tilde{v}_{ij,\ra{im}}+(\sum_{k=1}^n\sum_{l=1}^n \frac{h_{\ra{kl},\la{im}}+h_{\la{kl},\la{im}}+2\alpha_{\la{im}}}{\alpha_{\la{im}}+\gamma+\mu})\tilde{v}_{ij,\la{im}}\\
\end{aligned}
\end{equation}

where we use $\tilde{v}(ij,kl)$ to denote the corresponding the $(ij,kl)$ entry of $V_E^{-1}$. Specifically, all $\tilde{v}(ij,kl)$ values are known once the parameters for $V_E$ are set. Considering the case where the screening cost is linearly increasing with higher effort level $\epsilon{ij}$ as well as a greater number of travelers $I_{ij}$, in order to reduce the risk of infectious disease, our objective is therefore to optimally allocate a given resource $B$ such that the maximum eigenvalue of $F(\epsilon)\tilde{V}^{-1}$ is minimized. This can be well approximated by minimizing the maximum column sum $\tilde{C}_{ij}$ through optimally resource allocation. And we can therefore express the optimal resource allocation problem for controlling the disease through urban transportation system as following:
\begin{equation}
\min_{\epsilon} \max_{ij} \tilde{C}_{ij}(\epsilon)
\end{equation}
subject to
\begin{equation}
\begin{aligned}
&\epsilon_{ij}\geq 0, \forall{i,j}\\
& c\sum_{i,j} \epsilon_{\la{ij}}r_{ij}N_{ij}+ c\sum_{i}\sum_j \epsilon_{\ra{ij}}g_im_{ij}N_{i}\leq B,\forall{i,j}
\label{eq:resource_con}
\end{aligned}
\end{equation}
Specifically, equation~\ref{eq:resource_con} denotes the resource constraint as the total screened passengers across all travel segments should not exceed the available manpower.  
As a min-max linear programming problem, the optimal resource allocation problem can be easily transferred into an equivalent linear programming problem:
\begin{equation}
\min z
\end{equation}
subject to
\begin{equation}
\begin{aligned}
& z\geq \tilde{C}_{ij}(\epsilon), \forall{i,j}\\
&\epsilon_{ij}\geq 0, \forall{i,j}\\
& c\sum_{ij,i\neq j} \epsilon_{\la{ij}}r_{ij}N_{ij}+ c\sum_{i}\sum_j \epsilon_{\ra{ij}}g_im_{ij}N_{i}\leq B,\forall{i,j}
& 
\end{aligned}
\end{equation}
The system of equation can be easily solved using commercial solvers, and for the numerical experiments we use CPLEX in Matlab to obtain the optimally allocated resources. 



==> part B disease_network/prelim.tex <==
\section{Modeling preliminaries}

\subsection{Notation}
We summarize the list of variables used in this section as follows:
\begin{table}[htbp!]
	\setstretch{1.2}
	\centering
	\caption{Table of notation}
	\label{notation}
	\begin{tabular}{p{3cm}p{13cm}}
		\hline
		Notation & Description \\ \hline
		&\textbf{Variables}\\ \hline
		$S$ & Susceptible population. \\
		$E$ & Exposed (latent) population.\\
		$I$ & Infected population. \\
		$R$ & The population who recovered from disease and got immunity.\\
		$N_i^p$ & Total amount of visitors who are current present at zone $i$. \\
        $N_i^r$ & Resident population at zone $i$. \\ 
		$N_{ij}$ & The amount of people who are residents of zone $i$ and currently present at zone $j$. \\
		\hline
		&\textbf{Fixed parameters}\\ \hline
        $\beta$ & Contagion rate between $S$ and $I$. \\
        $1/\sigma$ & Length of latent period for population $E$.\\
        $1/\gamma$ & Length of infectious period for population $I$. \\
        $\mu$ & Death and birth rate. \\
        $P$ & Total number of zonees in the area. \\
        $\alpha_i$ & Arrival (departure) rate of external population for zone $i$. \\ 
		$g_i$ & Total departure rate of zone $i$.\\
		$m_{ij}$ & The rate of movement from zone $i$ to zone $j$, where $\sum_j m_{ij}=1$. \\
        $r_{ij}$ & The rate of return from zone $j$ to zone $i$\\
        $d^{M}$ & Control rate of travel mode $M$. \\
        \hline
	\end{tabular}
\end{table}

\subsection{Epidemic modeling}
The well-known compartment model for capturing the dynamics of infectious diseases was proposed by W.O.Kermack and A.G.McKendrick~\cite{kermack1927contribution}, where they consider that the population may experience three states over time: 
\begin{itemize}
\item Susceptible class or $S(t)$ is used to represent the number of individuals not yet infected with the disease at time t, or those susceptible to the disease.
\item Infected class or $I(t)$ denotes the number of individuals who have been infected with the disease and are capable of spreading the disease to those in the susceptible category.
\item Removed class or $R(t)$ is the compartment used for those individuals who have been infected and then removed from the disease, either due to immunization or due to death. Those in this category are not able to be infected again or to transmit the infection to others.
\end{itemize}

And the compartment model has several key assumptions: (1) each individual in the population has an equal probability of contracting the disease with a rate of $\beta$, (2) the population leaving the susceptible class is equal to the number of people entering the infected class, (3) people recovered from the disease with a mean recovery of $1/\gamma$ gain permanent immunity to the disease, and (4) the death rate is the same as the birth rate so that the total population is fixed. 

In reality, people who are infected by certain diseases may not present any symptoms until the end of the incubation period, and it is important to take this latent period into consideration for more accurate representation of disease dynamics. Consequently, the SEIR model was introduced with an additional compartment which is known as the latent class (E(t)) \cite{lloyd1996spatial}. The population of E are considered as exposed but not infectious, and will proceed into the infectious state with an average length of latent period of $\frac{1}{\sigma}$. Such disease dynamics can be mathematically represented as:
\begin{eqnarray}
&&\frac{dS}{dt}=-\beta SI+\mu (N-S) \\ \nonumber
\\ 
&&\frac{dE}{dt}=\beta SI-\mu E-\sigma E\\ \nonumber
\\ 
&&\frac{dI}{dt}=\sigma E-\gamma I-\mu I\\ \nonumber
\\
&&\frac{dR}{dt}=\gamma I-\mu R 
\end{eqnarray}

\subsection{Mobility model}
\label{sec:mobility}
The spread of infectious disease is closely interacted with the mobility pattern of urban population. Before discussing the mathematical model for capturing disease dynamics, we first present the mobility model that is followed by urban population. 

The mobility model used in this study is adapted from the intra-city mobility model proposed by Sattenspiel and Dietz~\cite{sattenspiel1995structured}. Different from the previous study, here we explicitly captures the mobility dynamics of population during travel which is especially important for modeling the mobility dynamics in densely populated urban areas. Specifically, we divide the urban area into a collection of $P$ zones and the population are further classified into two groups: residents and visitors. Residents of zone $i$ will be in one of the four states: staying at the resident location, travelling to the activity location, engaging in activities, and travelling back to the home location. Let $\ra{N}_{ij}$ be the population who are residents of zone $i$ and travel from $i$ to $j$, $N_{ij}$ be the population of residents of zone $i$ who are currently at zone $j$, $\la{N}_{ij}$ be the population who travel from $j$ back to $i$ and $N_i$ be the population who remain at the resident location at $i$. We have the following two equations to capture the total residents and visitors for a given zone:
\begin{equation}
N_i^r=\sum_{j=1}^{P} N_{ij}+{N}_{\ra{ij}}+{N}_{\la{ij}},\forall\,i
\label{eq:res}
\end{equation}
\begin{equation}
N_i^p=\sum_{j=1}^P N_{ji},\forall\,i
\label{eq:vis}
\end{equation} 
Equation~\ref{eq:res} suggests that the amount of residents at zone $i$ can be calculated as the summation of population who are residents of zone $i$ and currently at zone $j$. Similarly, equation~\ref{eq:vis} states that visitor population at zone $i$ consist of the residents of zone $i$ who remain in $i$, as well as the population who reach zone $i$ from other zones.

For people in different groups, we assume a constant rate of death $\mu$ and an equal rate of birth. New births of zone $i$ are assumed to join the residents of the same zone ($N_i$). For residents at zone $i$, a constant departure rate is assumed ($g_i$) and the departed population may visit zone $j$ for various daily activities (e.g., work or entertainment) with the split ratio of $m_{ij}$ and $\sum_j m_{ij}=1$. The departed population then join the population in travel and will arrive at the activity location with a rate of $\alpha_{\ra{ij}}$. The population at activity location will return to their home at the rate of $r_{ij}$, who again join the population in travel and eventually arrive at home with the rate of $\alpha_{\la{ij}}$. With the above description, we have the following system of ordinary differential equations (ODE) for computing the mobility dynamics within a urban area:
\begin{equation}
\frac{d{N}_{\ra{ij}}}{dt}=g_im_{ij}N_{i}-\alpha_{\ra{ij}} {N}_{\ra{ij}}-\mu{N}_{\ra{ij}}  %departure - arrival
\label{eq:bt1}
\end{equation}
\begin{equation}
\frac{d{N}_{\la{ij}}}{dt}=r_{ij}N_{ij}-\alpha_{\la{ij}} {N}_{\la{ij}}-\mu{N}_{\la{ij}}  %departure - arrival
\label{eq:bt2}
\end{equation}

\begin{equation}
\frac{dN_{ij}}{dt}=-r_{ij}N_{ij}+\alpha_{\ra{ij}} {N}_{\ra{ij}} -\mu N_{ij}
\label{eq:bt3}
\end{equation}
\begin{equation}
\frac{dN_{i}}{dt}=\sum_{j=1}^P \alpha_{\la{ij}} {N}_{\la{ij}}-g_iN_{i} -\mu N_i+\mu N_i^r
\label{eq:bt4}
\end{equation}

With the above system of equations, we can calculate the rates of change for resident and visitor population as:
\begin{equation}
\begin{aligned}
\frac{{N}_i^r}{dt}&=\sum_{j=1}^P \frac{{N}_{ij}}{dt}+\frac{{N}_{\la{ij}}}{dt}+\frac{{N}_{\ra{ij}}}{dt}
\end{aligned}
\label{eq:res}
\end{equation} 

\begin{equation}
\begin{aligned}
\frac{{N}_i^p}{dt} &=\sum_{j=1}^P \frac{{N}_{ji}}{dt}
\end{aligned}
\label{eq:vis}
\end{equation}
The described system of equations will reach the equilibrium if equations~\ref{eq:bt1} to~\ref{eq:bt4} equal zero, e.g., there is no change of population for each compartment. Consequently, for the equilibrium solution of the mobility dynamics, we arrive at the following proposition:
\begin{prop}
	The system described by equations~\ref{eq:bt1} to~\ref{eq:bt4} is linear and has a unique equilibrium solution, and the solution is globally asymptotically stable. In particular, at equilibrium, we have
	\begin{equation}
	N_{i}^*+\sum_{j=1}^P K_{ij}N_{ij}^*=N_i^r
    \label{eq:equilibrium_ii}
	\end{equation}
	\begin{equation}
	N_{i}^*=\frac{1}{1+\sum_{j=1}^P K_{ij}}N_i^r
    \label{eq:equilibrium_ij}
	\end{equation}
    where $K_{ij}=g_im_{ij}(\frac{1}{r_{ij}}+\frac{1}{\alpha_{\la{ij}}}+\frac{1}{\alpha_{\ra{ij}}})$.
\end{prop}
\begin{proof}
	Since the system is linear, and the matrix constitutes a strongly connected graph. The equilibrium solution of the system can be calculated by setting equation~\ref{eq:bt1} to~\ref{eq:vis} to zero. 
    We have:
    \begin{equation}
    {N}_{\ra{ij}}^*=\frac{g_im_{ij}}{\alpha_{\ra{ij}}+\mu}N_{ii}^*, N_{ij}^*=\frac{g_im_{ij}\alpha_{\ra{ij}}}{(r_{ij}-\mu)(\alpha_{\ra{ij}}+\mu)}N_{ii}^*, ,{N}_{\la{ij}}^*=\frac{g_im_{ij}\alpha_{\ra{ij}}r_{ij}}{(r_{ij}-\mu)(\alpha_{\ra{ij}}+\mu)(\alpha_{\la{ij}}+\mu)}N_{ii}^*
    \label{eq:ijii}
    \end{equation}
    Let $K_{ij}=\frac{g_im_{ij}}{\alpha_{\ra{ij}}+\mu}+\frac{g_im_{ij}\alpha_{\ra{ij}}}{(r_{ij}-\mu)(\alpha_{\ra{ij}}+\mu)}+\frac{g_im_{ij}\alpha_{\ra{ij}}r_{ij}}{(r_{ij}-\mu)(\alpha_{\ra{ij}}+\mu)(\alpha_{\la{ij}}+\mu)}$. Based on equation~\ref{eq:res} and the fact that $N_i^r$ is fixed, we have:
    \begin{equation}
    N_{ii}^*+\sum_{j=1,j\neq i}^P K_{ij}N_{ii}^*=N_i^r
    \end{equation}
    We therefore have
    \begin{equation}
    N_{ii}^*=\frac{1}{1+\sum_{j=1,j\neq i}^P K_{ij}}N_i^r
    \end{equation}
	which gives equation~\ref{eq:equilibrium_ij}. 
	
	To prove that the equilibrium solution is G.A.S, one can write the whole matrix $M$ for system $dN/dt=MN$. Since the urban areas can be viewed as a connected network, it can be easily shown that diagonal entries in $M$ are strictly negative (either $-\mu$ or $-g_i+\mu$) and the matrix $M$ has all negative real eigenvalues, which implies that the equilibrium point is G.A.S. 
\end{proof}

In the following sections, we will write $N_{ij}$ to denote equilibrium population flow $N_{ij}^*$ for notation simplicity.


==> part B disease_network/result_new.tex <==
\section{Results}
\subsection{Experiment setting}
The numerical experiments are conducted on a desktop with @3.5 GHz CPU and $32GB$ RAM. The codes are written in Matlab and the disease trajectories are simulated using the ODE 45 solver. The numerical experiments in this study consist of two parts. Based on toy networks as shown in Figure~\ref{fig:small_network}, the first part is to compare the resulting disease dynamics with and without modeling the urban transportation system, including the differences in disease trajectories, the impact on $R_0$ values and the city-wide synchronization of the diseases. We also investigate how disease outbreaks may evolve with varying urban structures and transportation systems. The networks have 5 nodes and 25 OD pairs, meaning that each node is accessible from the other. As each OD pair may have four states (S,E,I,R), the ODE system of this test network therefore has 300 state variables and 300 equations. For the second experiment, we focus on validating the effectiveness of the Trans-SEIR model with real-world networks. We choose New York City (NYC) as the study area and verify the model outputs when compared to the reported data during the COVID-19 outbreak. The NYC network is shown in Figure~\ref{fig:nyc_net}. NYC is divided into 15 zones and the network is established following the Google transit information. The 15 zones lead to a system of 2760 state variables and 2760 equations for the ODE system. 
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/Small_example.pdf}
    \caption{Network layouts of three sample networks}
    \label{fig:small_network}
\end{figure}

\subsection{Results on toy networks}
We first demonstrate the results of the Trans-SEIR model on the toy networks, and we focus on the validity of the disease threshold, the dynamics of the disease trajectories and the impacts of the travel related contagions. Figure~\ref{fig:sub_A} shows the disease of dynamics of two different scenarios in network A, where case 1 serves as the base scenario and case 2 doubles the transmission rates of those in case 1. Both cases have a total population of 10 million and start with an initial infectious population of 1,000 which are uniformly distributed among the residents of all five zones. Since case 1 has the $R_0$ value of 0.84, we observe that the number of infectious people decays exponentially fast and the system quickly moves towards the DFE state. On the contrary, case 2 has the $R_0$ value of 1.68 and exponential growth in the number of exposed and infectious populations can be immediately observed. The disease in case 2 eventually invades around 66.7\% of the total population before it dies out. While the complete trajectory was not shown here, we report that there is a strictly positive proportion of the population that remains infectious which agrees with the endemic equilibrium with $R_0>1$. For these two cases, we also compare the results with the outcomes when travel contagion is not considered (e.g., $\beta^T=0$). We can see that the two systems differ significantly and the results suggest that we may underestimate the risks of an urban disease outbreak if travel contagion is ignored, or equivalently we may overestimate the transmissibility of an infectious disease if conventional disease models are fitted to the historical data in urban areas. And the results therefore highlight the importance of considering travel contagion in transit systems for the most accurate understanding of urban disease dynamics and devising proper intervention and control strategies. Moreover, we find that, given the same population distribution and mobility patterns, the network structure of urban transit systems may have great impacts on the disease trajectories as shown in Figure~\ref{fig:three_city}. The network layouts of the three cities reflect different planning philosophies regarding the trade-off between accessibility and system efficiency. Network B represents the highest accessibility between trip ODs but also the highest operation costs with numerous direct transit routes. On the other hand, network C achieves the maximum transit usage with the minimum number of transit lines, but also leads to the highest number of passengers sharing overlapping trip hence the greatest risk of travel contagion. Based on the results of the toy network, we see that the number of secondary infections in network C may be 7.4\% higher than that of network B and 3\% higher than that of network A. As all these networks will reach the endemic equilibrium, the excessive contacts during travel in network C may increase the total infected population of network B by over 7.26\% and result in the arrival of the peak nearly 30 days earlier. And the early peak is primarily driven by the spatial synchronizations of the disease dynamics which is facilitated by the travel contagion, as shown in Figure~\ref{fig:sync}. In particular, we measure the rate of synchronization as the standard deviation of the change rates of the total infectious population of each zone. Higher std stands for the larger discrepancy among the zonal change rates and hence the disease dynamics are less synchronized. As the spread of disease usually starts with the first few external visitors in local areas, the rate of spatial synchronization therefore determines the pace and the scale of the citywide outbreak. The results in Figure~\ref{fig:sync} suggest that the disease dynamics across different zones are synchronized at an exponential rate, and the exponential decay rate for network C is 20\% higher than that without travel contagion or 10.2\% higher than that for network B, highlighting the catalyst effect of the urban transit system and travel contagion in promoting a faster pace for spatial synchronization. While urban transit systems have long been designed as an affordable mobility solution for the mass population, these results clearly assert an emerging need to rethink the planning and operation of the urban transit systems to balance the goal of efficiency maximization and the risk of infectious disease during extreme pandemics. 

\begin{figure}[ht!]
    \centering
    \subfloat[Disease dynamics of two scenarios in Network A\label{fig:sub_A}]{\includegraphics[width=0.6\linewidth]{figure/figure_city1_compare-eps-converted-to.pdf}}\\
    \subfloat[Comparison of E and I curves for different cities using disease parameters in case 2 \label{fig:three_city}]{\includegraphics[width=0.55\linewidth]{figure/figure_threecities-eps-converted-to.pdf}}
    \subfloat[Synchronization among different zones \label{fig:sync}]{\includegraphics[width=.4\linewidth]{figure/figure_synch-eps-converted-to.pdf}}
    \caption{Disease dynamics in two scenarios}
    \label{fig:sample_shape}
\end{figure}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figure/figure_travel_contagion_dynamics-eps-converted-to.pdf}
    \caption{Cumulative dynamics of infected population, activity contagion and travel contagion in the three toy networks.}
    \label{fig:trans_dynamics}
\end{figure}

The previous discussion demonstrates the significant role played by the urban transportation system in boosting the spread of infectious diseases. Nevertheless, we further report that direct transmission during travel in the public transit systems may not constitute a major source of infections during an urban disease outbreak. To see this, we summary the cumulative dynamics of the total number of infectious (as the percentage of the total population), direct travel contagion and activity contagion, and the results can be found in Figure~\ref{fig:trans_dynamics}. It is observed that, depending on the particular network layout, direct travel contagion may account for a small proportion (10.0\% - 17.6\%) of total infected cases and the majority of the infections arise from non-travel related activity engagement such as work and entertainment. The reason is that the number of travelers in the transit system and the exposure duration are both lower than those during regular activities. While direct travel contagion is the most straightforward measure to quantify the impacts of the urban transportation system, the metric is not comprehensive as it does not capture the secondary cases produced by travel infections. To this end, we introduce the notion of induced travel contagion to measure the amount of infected population who are transmitted at activity locations by contacting people who are infected during travel. The induced travel contagion is calculated as the difference between the amount of activity contagion with and without travel infections, and the results are shown in Figure~\ref{fig:induced}. We note that the induced travel contagion in these three networks may account for an additional 4.27\% to 5.55\% of new infections. This implies that travel-related contagion may contribute to 16.9\% to 25.6\% of the total infections. Moreover, all the results are carried out based on the assumption that the transmission rate in the transit system is half of that at activity locations. We further illustrate how travel-related contagion may change by altering the travel transmission rate, and the results are shown in Figure~\ref{fig:sensitivity}. Specifically, we vary the travel transmission rate from 50\% to 250\% of the base travel transmission rate, and we observe that direct travel contagion increases linearly with respect to higher travel transmission rate, while the induced travel rate is found to be a concave function of the travel transmission rate. We further note that the linear relationship is only a local property within the evaluated range of travel transmission rate, which will turn into a concave function as we further increase the transmission rate. And the results suggest that, if we consider that the strengths of travel transmission and activity transmission being the same, the total travel-related infections may eventually account for over 35\% of the total infected cases during an urban disease outbreak. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.4\linewidth]{figure/figure_travel_contagion_cumulative-eps-converted-to.pdf}
    \caption{Number of induced travel contagions in different cities.}
    \label{fig:induced}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figure/figure_trans_level_sensitivity-eps-converted-to.pdf}
    \caption{Sensitivity of travel contagion with respect to the change in transmission rate during travel ($\beta^T$)}
    \label{fig:sensitivity}
\end{figure}

\subsection{NYC experiments}
We use a combination of the United States 2010 census survey, 2010 NYC peripheral transportation study~\cite{nyc_periph_report2010}, NYC Neighborhood Tabulation Areas shapefile and the reported confirmed COVID-19 cases in NYC~\cite{nyc_covid_data} to prepare the data for our case study. To better account for the mobility dynamics, we set each step of the simulation as a 2-hour period and the modeling parameters are tailored to the time interval accordingly.  There are two sets of parameters to be calibrated. For the mobility dynamics, we use the 2010 census survey along with the 2010 peripheral transportation study, projected into 2020 population values, to obtain the population and the travel rate between nodes in the network. The mobility model at equilibrium estimates around 2.7 million daily commuters within NYC, and this number agrees with the value of the peripheral transportation study~\cite{nyc_periph_report2010}. For disease parameters, we set $\sigma$=$0.016$ (average duration of incubation period being 5.1 days~\cite{lauer2020incubation}) and $\gamma=0.013$ (average duration of recovery or death of 6.5 days) based on the calibrated parameters from the reported data in Hubei province, China~\cite{yang2020modified}. 

As the focus of our study is to understand the impacts of travel contagion rather than predicting the trajectories of the disease dynamics, we calibrate the disease transmission rate and the average number of contacts through a simple line search. And the parameters are finalized when the model is observed to align with the trend of the reported confirmed cases in general. The outputs from the calibrated model and its comparison with the reported confirmed cases in NYC can be seen in Figures~\ref{fig:nyc_all_trend} and~\ref{fig:nyc_borough}. In general, we find that the Trans-SEIR model may well capture the COVID-19 dynamics based on the calibrated parameters from the NYC census and travel data for daily commuting patterns. We observe that the dynamics of cumulative confirmed cases match well with the period between March 20 to April 5 when a large number of tests were performed so that the reported values were closer to the actual disease dynamics. Moreover, the model results are also consistent with the reported cases in each borough. This suggests the potential of the Trans-SEIR model for prediction tasks if more rigorous parameter calibration may be conducted. The disease dynamics is highly spatially heterogeneous. Following equation~\ref{eq:R0_value}, the model gives the $R_0$ value of 3.295 and the similar values were also reported in the literature~\cite{liu2020reproductive}. But this value only represents the average level of secondary infections over the entire NYC, and the values are significantly higher in certain boroughs. Specifically, we see that the transmission rates in Bronx, Brooklyn and Queens are over 30\% higher than that of Manhattan, despite Manhattan being the most densely populated borough. There are several possible reasons that may result in this observation. For instance, one possible explanation is the under-reporting or lack of testing in Manhattan. However, there may be other factors such as the differences in income level, level of education, age group, and the adoption of early preventative measures among the boroughs that lead to this high discrepancy. These other factors may worth further investigation.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.6\linewidth]{figure/NYC_shape.pdf}
    \caption{Network layout for the NYC case study}
    \label{fig:nyc_net}
\end{figure}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.4\linewidth]{figure/nyc_all-eps-converted-to.pdf}
    \caption{Fitted data for the Covid-19 case}
    \label{fig:nyc_all_trend}
\end{figure}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figure/nyc_borough-eps-converted-to.pdf}
    \caption{Fitted data for the Covid-19 case}
    \label{fig:nyc_borough}
\end{figure}

Since the Trans-SEIR model considers the spatial movement of urban travelers, the results also allow for revealing the travel segments and activity locations that are associated with the greatest number of infections and we visualize the results in Figure~\ref{fig:travel_flow}. The strong spatial heterogeneity in terms of both activity and travel contagion can be readily observed in Figure~\ref{fig:nyc_hist}, where total contagion during travel may account for 28.8\% of the total cases in NYC as of March 26 but the values differ based on the residential locations of the commuters. In particular, Staten Island is the place with the minimum travel contagion as most of the trips are within the same area and travelers are least dependent on public transit. On the contrary, the north Manhattan area has the highest ratio of travel contagion with its heavy usage of buses and metros. For commuters of the same residential location, the split ratios of travel contagion and activity contagion also vary significant based on their activity locations. Figure~\ref{fig:nyc_travel} presents the relative proportion of travelers (represented as the thickness of the flow curves) who are residents of zones in the top and get infected in the transit system while traveling to and from the bottom zones. It can be observed that east Manhattan is the activity location that is associated with the highest number of the infected population during travel. Moreover, east Manhattan is also the primary destination that contributes to the highest number of travel contagions for residents of each zone except for Staten Island where most of the commuting trips take place within the same area. The major reasons behind this observation are threefold: east Manhattan is the major trip attractor for other areas in NYC, transit such as bus and metro are the major modes for commuting to the area, and long commuting trips are expected for people living outside the Manhattan area. These lead to both high population density and prolonged contact duration for the transit routes linking to east Manhattan which significantly exacerbates the contagion risk level. Besides, we find that west \& lower Manhattan and Ft. Greene/Bay of Brooklyn are the other two major destination locations for infections during travel. The source of travel contagions who arrive at west \& lower Manhattan are again the commuters from outside Manhattan. But the corresponding source of travelers who arrive at Ft. Greene/Bay of Brooklyn are primarily the residents within the Brooklyn area, and similar patterns are observed for the other activity locations. The distribution of activity contagion largely resembles that of travel contagion as shown in Figure~\ref{fig:nyc_act}. The major difference is that activity locations are mostly observed within the same location for areas such as Ft.Greene of Brooklyn, northwest Queens and the Bronx. The reason is that majority of the residents in these locations also have activity locations in the same areas, and trips within these areas are mostly made by private vehicles so that travel contagion is not the major threat. Based on these findings, we arrive at a better understanding of the spatial trajectories of the disease dynamics where the east and west \& lower Manhattan areas are likely the intermediate stops before the disease reaches every corner of NYC. This also hints at the potential locations where entrance screening may be placed to mitigate the spread of the diseases, which require further validation based on the results of the optimal control problem. 

\begin{figure}[htbp!]
    \centering
    \subfloat[Number of travel contagion and activity contagion in each area\label{fig:nyc_hist}]{\includegraphics[width=0.8\linewidth]{figure/nyc_travelcon_hist-eps-converted-to.pdf}}\\
    \subfloat[Alluvial flow diagram for the amount of travel contagion between pairs of zones.\label{fig:nyc_travel}]{\includegraphics[angle=-90,width=0.8\linewidth]{figure/trans_flow-eps-converted-to.pdf}}\\
    \subfloat[Alluvial flow diagram for the amount of activity contagion between pairs of zones.\label{fig:nyc_act}]{\includegraphics[angle=-90,width=0.8\linewidth]{figure/nyc_act_contagion-eps-converted-to.pdf}}
    \caption{The distributions of travel contagion and activity contagion during the COVID-19 outbreak in NYC, measured by the amount of people in latent class (E) as of March 26. }
    \label{fig:travel_flow}
\end{figure}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.4\linewidth]{figure/nyc_control-eps-converted-to.pdf}
    \caption{Effectiveness of transportation control with different budget level}
    \label{fig:nyc_control}
\end{figure}

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/budget_control-eps-converted-to.pdf}
    \caption{Distribution of control resources under different budget level}
    \label{fig:nyc_budget_allocation}
\end{figure}

We summarize the results of optimal entrance control in Figures~\ref{fig:nyc_control} and~\ref{fig:nyc_budget_allocation}. We report that entrance control for urban transit system can be a highly effective countermeasure against the outbreak of infectious diseases in urban areas, for both preventative and reactive purposes. If limited resources are distributed in an optimal manner, we are able to curb the disease and drive it to the disease-free equilibrium state, and will contribute to a significant reduction in the number of total infections. To validate the proposed solution approach, we compare the effectiveness among optimal control as devised in our study and two other benchmark methods: the uniform control where equal resources are distributed among all travel segments and the high-demand control where travel segments with higher demand are prioritized for resources. The measure of effectiveness is the $R_0$ value after control as shown in Figure~\ref{fig:nyc_control}, where the x-axis denotes the number of resources spent (manpower used for screening travelers). We observe that, by only focusing on medium and high capacity modes and if we can distribute the resources optimally, we are able to lower the $R_0$ to 1.2 by screening approximately 10,000 daily travelers per time step, or less than 4.5\% of total daily commuters. While the screening of 10,000 travelers can be expensive in practice and may lead to excessive externalities such as heavy delay, we also find that an exponential rate of reduction in $R_0$ can be achieved with optimal control strategy for a small number of initial efforts. If we may perform the screening of 2000 travelers with a success rate of 70\%, we will be able to lower the $R_0$ in NYC to 2.32 which represents a 29.6\% reduction in the number of secondary infections and implies significant potential saving of lives and medical resources.  Note that this level of control effectiveness is achieved through the compartment model and control strategy being implemented at the aggregate level, an encouraging finding is that the outcomes of the optimal control approach are comparable to that of the target control strategy at the individual level with perfect information on the contact network structure and the state of each travelers~\cite{qian2020scaling}.  Meanwhile, the other two benchmark approaches are found to be barely effective. Despite direct and induced travel contagions, we need to pay attention to the case that infectious people will need to travel using the urban transit system to further spread the disease. If the resources and screening manpower can be optimally allocated, we can effectively identify these infectious travelers, put them into quarantine and stop them from producing new infections. To this end, we also visualize the optimal distribution of resources across the travel segments as shown in Figure~\ref{fig:nyc_budget_allocation}. The major findings echo to the general observations in Figure~\ref{fig:nyc_all_trend}, where east Manhattan is the target area to place the majority of the resources and should be exclusively controlled with very limited resources (budget<5000). Moreover, for commuters with east Manhattan as the activity location, the optimal solution suggests targeting those from Staten Island, Queens and the Bronx with top priority. This can help to prevent infectious travelers from resulting in secondary cases within their areas where massive activity contagions are observed. With more resources available, the optimal solution recommends focusing on residents of the above-mentioned areas who have their activity locations in west \& and lower Manhattan and part of the Brooklyn area, before placing stricter screening for residents within the Manhattan area due to the relatively low activity contagion rates. In conclusion, the results of the optimal control method suggest a highly promising direction for the control of urban transportation systems in densely populated areas. And the Trans-SEIR model with the travel control approach may have significant implications towards the operation of public transit systems after the reopening of businesses to mitigate further risks of the COVID-19 outbreak. 

==> part B disease_network/results.tex <==
\section{Results}

\subsection{Experiment setting}
The numerical experiments are conducted on a desktop with @3.5 GHz CPU and $32GB$ RAM. The codes are written in C++ and compiled with gcc in Linux system. The MPFR library is used for interval arithmetic and the Flow* library is used for doing TM flowpipe construction. The numerical experiments have three major parts. The first part is to compare the results on disease dynamics with and without modeling urban transportation system, including the difference in disease equilibrium patterns and the impact on $R_0$ values. The second part focuses on the performance of the reachability analysis, where the computational performances as well as the tightness of the overapproximation is discussed. Finally, we investigate how disease outbreaks evolution may vary based on different urban structures. For the first two parts, we mainly focus on the test network as shown in Figure~\ref{fig:smallnetwork}. The network has 3 nodes and 9 OD pairs, meaning that each node is accessible from the other. As each OD pair may have four states (S,E,I,R), the ODE system of this test network therefore has 36 state variables and 36 system equations. We consider the invasion of H1N1 influenza in 2009 as the case study for the test networks. According to the literature~\cite{tuite2010estimated}, the disease has the contact rate $\beta$ of $0.585$, $\gamma$ being $0.09$, and $\sigma$ being $0.47$, which suggests that H1N1 has an average latent period of 2 days and recovery time of 10 days. And based on the epidemic parameters, our objective is to compare how disease dynamics may vary in three different systems: the SEIR system without travel contagion, the SEIR system with travel contagion but no intervention strategies, and the SEIR system with travel contagion and entry control strategies. In particular, for the control strategies, we consider three different level of controls, namely the high level of control that may possibly eliminate 50\% of suspicious travelers from entering the system, the medium level of control that may eliminate 30\% of infected travelers, and the low control level where only 10\% of infectious population may be identified. And different control strategies may have different impact on the travel time for the corresponding travel modes. The third part of the experiment setting will focus on a different set of networks, as shown in Figure~\ref{fig:urbannetwork}. For this part, we consider networks that represent three different urban structures: the stripe-shaped network such as Shenzehen, China, the single-centered network including Paris and New York City, and the multi-centered networks (in this study we consider dual centers for simplicity) such as Beijing and Shanghai, China. And we analyze how effective are various control strategies in controlling these networks.

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=50mm]{results/network.png}
	\caption{Test network with 3 nodes}
	\label{fig:smallnetwork}
\end{figure}

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=150mm]{results/urban_network.png}
	\caption{Networks with three different urban structures}
	\label{fig:urbannetwork}
\end{figure}


\subsection{Case study: 2003 SARS outbreak in Beijing}
One major difficulty related to mathematical modeling of infectious diseases is the validity of the developed models. In general, it is not possible yet ethical to validate the fidelity of the model with field experiments. And in this study, we investigate the validity of our model by measuring the alignment of its predicted results with the real-world ground data during the 2003 Severe Acute Respiratory Syndrome (SARS) outbreak in Beijing, China.

The 2003 Beijing SARS outbreak is one of the few disease outbreaks within urban areas that has documented the daily progress of the disease pattern. There were 2523 probable cases of SARS reported from March 5, 2003 to May 29, 2003~\cite{pang2003evaluation}. Multiple control measures had been implemented during the outbreak, including the set up of dedicated SARS hospital, information dissemination of real-time SARS pattern, and the closing of public facilities. As for the transit system, surveillance sites had been set at the airport, major train stations, and 71 roads that connect Beijing to peripheral areas. The metro system improved its ventilation system, and more frequent and thorough disinfections were conducted for both metro compartments and buses. In addition, staffs of bus and metro systems had been trained to identify and take immediate actions against probable patients during travel.  

\begin{figure}[htbp!]
	\centering
	\subfloat[Disinfection of metro compartment taking place on April 21, 2003]{\includegraphics[width=75mm]{results/beijing_metro_disinfection.jpg}}  
	\subfloat[Body temperature screening at the train station]{\includegraphics[width=70mm]{results/beijing_temperature.jpg}}
	\caption{Measures were taken in mass transit systems to identify probable cases of SARS in Beijing}
	\label{fig:sars_measures}
\end{figure}

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=100mm]{results/peknet.pdf}
	\caption{The Beijing network with 5 nodes}
	\label{fig:beijing}
\end{figure}

To model the SARS outbreak, we first divide Beijing into 5 areas as shown in Figure~\ref{fig:beijing}. Among the 14 million population in Beijing by the end of 2003, 40\% of them reside inside the third ring road of Beijing (which corresponds to center area 3 in Figure~\ref{fig:beijing}). And we consider the rest 4 areas have similar population size, with each accounts for 15\% of total population of Beijing. Due to lack of daily commuting data in 2003, we assume that the 70\% of the activities for people living in area 3 are within area 3, and 40\% of the activities are within the same area for the other 4 areas. This gives the vector of departure rate $g=[0.6,0.6,0.3,0.6,0.6]$. For each OD pair, we consider the return rate being $0.9$. For residents of area 3 who leave the area for daily activities, we assume that they have equal chances to reach all other 4 areas. And for residents of area 1,2,4, and 5, we consider that they have 40\% of chance to visit area 3, and 20\% for other three places. Three transit modes are considered with capacity ranging from high to low, and the ratio of travel time for the same OD pair are set to 5:8:6. Considering various efforts made in mitigating disease spreading within transit system, we assume that the high capacity and medium capacity modes have 20\% probability for identifying the probable case during travel. For the disease parameters, the typical incubation time for SARS is reported to be within 2-7 days, with 3-5 days being most common~\cite{SARS_CDC}. Consequently, we set $\sigma=1/3$ for the case study. Different from the its typical definition, the recovery state R in this case study should refer to the state where an infectious individual or probable case of SARS is identified and isolated from the mass population. Due to the effectiveness of information dissemination and increasing alertness of people to SARS, it is reasonable to consider that any people with symptoms may get easily identified as long as they take part in any social activities. This value along with the infectious rate $\beta$ are usually identified through curve fitting from real-world data. The recovery rate is set to $0.6$ in our study, meaning that in 60\% of the cases the infectious individual will be identified and hospitalized. The infectious rate $\beta$ was reported to take values between $0.57$ to $1$ in various cases~\cite{colizza2007predictability,ng2003double}. But this value is temporally varying and is sensitive to the control measures being taken. In our study, we consider the infectious rate being $0.71$ for the entire population, and therefore the effective transmission rate per contact being $5.07e-8$. Based on the parameter setting, we constructed the epidemic model of 100 dimensions for 25 OD pairs and the results are simulated using ODE45 simulator in MATLAB, as shown in Figure~\ref{fig:case_sum} and Figure~\ref{fig:case_daily}.

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=100mm]{results/cum.eps}
	\caption{Cumulative SARS cases since April-20, 2013, Beijing, China}
	\label{fig:case_sum}
\end{figure}

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=100mm]{results/daily_increase.eps}
	\caption{Daily increases of SARS cases since April-20, 2013, Beijing, China}
	\label{fig:case_daily}
\end{figure}

We use the official data from Chinese Ministry of Health as the baseline observations, which gives the daily number of probable SARS cases starting from April 20, 2003 to June 12, 2003. While the number of infectious and latent population were unknown, we assume $E(0)=420, I(0)=223$, and $R(0)=210$, and these people are evenly distributed in all 5 areas, where the simulated results well match the statistics reported in the first day (April-20, 2003). It can be verified from the results that the simulated curve for the number of cumulative cases may well approximate the actual observations reported, especially within the first 15 days. Moreover, the total number of cases based on the simulation is 2745, which is only 8.8\% higher than the actual total cases. As for the daily number of cases, though the deterministic model may not be able to capture the stochasticity that takes place in the real-world, the simulated results still follow the trend similar to the actual observations. It provides a very good sense on how the disease may propagate over days with limited inputs, and the differences between simulation results and observations for daily increases is smaller than 15 cases in 47 out of the 65 days. In addition, if we only apply the conventional SEIR model in this case, the corresponding $R_0$ value is $0.71/0.6=1.183$, which implies that the disease will invade the entire population which is entirely different from the actual observations. On the other hand, if we match the the $R_0$ value of SEIR model with our proposed model ($R_0=0.836$ in this case), the limiting number of cases will become 3774 cases, which is significantly higher than the observed value. And the SEIR model may be able to give a closer estimation of 2472 cases only if we set $\gamma=0.97$, which implies that we are able to hospitalize the patients as soon as they get infected and such scenario is barely possible for any real-world disease outbreaks. Consequently, these results may well support the fidelity of our developed approach and reveal the potential of our model for predicting the propagation of disease outbreaks that take place in urban areas.

\subsection{The role of contagion within transportation system}

\begin{figure}[htbp!]
	\centering
	\subfloat[Disease A with $\beta=0.7$]{\includegraphics[width=80mm]{results/highinfect_I.eps}}
	\subfloat[Disease B with $\beta=0.25$]{\includegraphics[width=80mm]{results/lowinfect_I.eps}}
	\caption{Total infected population over time}
	\label{fig:disease_pattern_compare_I}
\end{figure}

We next assess the importance of modeling travel contagion during urban disease outbreaks. We mainly focus on comparing the results from three different models: the disease model without modeling travel contagion (MWOTC), the disease model that models travel contagion but no interventions introduced (MWTC), and the disease model that model travel contagion and considers control measures over traffic modes (MWTC-CM). Note that MWOTC ad MWTC are special cases of MWTC-CM, where MWTC-CM reduces to MWTC when the vector $d$ is set to unity, and the MWTC can be reduced to MWOTC by let $\beta_{tra}=0$. We investigate the differences in the disease dynamics among the three models from two aspects: the disease dynamics of different infectious diseases and the change of $R_0$ with respect to different diseases. The same network as in the 2003 Beijing SARS case study is used in this section. For simplicity, we set total population to be 1 instead of 4, and assume that at the beginning only patch 1 has infectious people that account for 1\% of the population, and all remaining people are in the susceptible state. 

We first present the propagation dynamics associated with highly infectious and lowly infectious diseases. We assume that the incubation period is 4 days, and the average time of recovery is 5 days. The highly infectious disease A has $\beta=0.7$ and the $\beta$ for lowly infectious disease B is 0.25. In addition, we consider $20\%$ of travel control effectiveness for both diseases. The results of total infected population of the entire urban area are presented in Figure~\ref{fig:disease_pattern_compare_I}. For disease A, the corresponding $R_0$ values for MWOTC,MWTC and MWTC-CM are 1.639, 2.013, and 1.834 respectively. And those of disease B are 1.051, 1.172, and 0.998. These two cases prove the correctness of our derivation of $R_0$, where the disease is endemic and persists in the population when $R_0>1$, and the system converges to the DFE state when $R_0<1$ (MWTC-CM for disease B). And in both cases, we observe that the equilibrium points are stable. 

As can be seen in both cases, without considering travel contagion, it is likely that we will underestimate the peak number of infected population and obtain a delayed prediction of the peak time. And such gaps are more obvious during the outbreak of the less infectious disease B. It is not difficult to interpret the higher peak of infected population, since by modeling travel contagion we are considering an additional layer of interactions between susceptible and infected people during their travels. And for the early arrival of the disease peak, it is due to the faster synchronization of disease pattern over the urban area with the help of travel contagion. This effect is illustrated in Figure~\ref{fig:disease_pattern_sync}, where the total number of infected people in each patch of the network is presented. At time step 0, the patch one start with 1\% of infected people and all other patches are free of disease. As time progresses, we observe the infected population of patch 1 first drops and then starts to increase. But the point where the change of gradient takes place is quite different in the two cases. Without travel contagion, the infected population in patch 1 starts to increase around time step 30, while the corresponding time step is around time step 15 if the travel contagion is modeled. In addition, since patch 1,2,4,and 5 have similar population size and travel pattern, we observe that their disease dynamics start to converge after the initial several steps. And model with travel contagion reaches this convergence earlier than without modeling travel contagion. All of these suggest the faster synchronization of disease pattern due to the existence of travel contagion. On the other hand, if we place control measures to our transit system to make it more invulnerable to infectious diseases, we are able to effectively reduce the peak size of the diseases, as well as the total number of infected people over the entire disease outbreak. But more importantly, it can be verified that by controlling the transit system through moderate efforts, it is possible to change the state of the disease from endemic to DFE, which results in the elimination of the disease overtime. This is especially meaningful for diseases such as influenza where people are paying less attention to due to comparatively insignificant consequences and we barely have effective measures for its eradication besides mass annual vaccination. 

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=150mm]{results/disease_synchronization.png}
	\caption{Total number of infected people in each patch}
	\label{fig:disease_pattern_sync}
\end{figure}

We next evaluate how the two key parameters $R_0$ and $R_\infty$ may differ in the three models with respect to different disease infectious rates, as shown in Figure~\ref{fig:r0}. It is known that $R_0=1$ is the threshold of disease invasion, and by modeling travel contagions, it is likely that the disease tends to be endemic while the result reported without travel contagion is disease free. And the gap between with and without travel contagion in $R_0$ tends to increase as $\beta$ increase, meaning that it is even more crucial to consider the travel contagion for diseases with higher transmission rate. Moreover, while disease pattern may change from DFE to equilibrium by considering travel contagion, a moderate control intervention (eliminating 20\% of infected population) may driver bring the disease back to the DFE state, as shown in Figure~\ref{fig:r0}(b). And the control strategy is increasingly effective as $\beta$ changes from 0.1 to 0.4, where we may reduce the total infected population during endemic by over 50\%. 

\begin{figure}[htbp!]
	\centering
	\subfloat[Change of $R_0$ with different $\beta$ values]{\includegraphics[width=80mm]{results/beta_R0.png}}
	\subfloat[Change of total infected population at equilibrium with different $\beta$ values]{\includegraphics[width=80mm]{results/w_versus_wo.png}}\\
	\caption{The change of $R_0$ by modeling urban travel}
	\label{fig:r0}
\end{figure}

Finally, we would like to evaluate how different control strategies may be effective under different urban structures. That is, the way people travel and get in contact may be different with different urban structures. We consider the three networks as introduced before, and vary control effectiveness for medium and high capacity modes, from 0\% to 100\% effective, and the results are shown in Figure~\ref{fig:compare}. There are clearly boundaries on the effectiveness of the controlling strategies, as increasing the effectiveness will add extra travel times thus driving travelers to other modes. Therefore, for the particular disease, we see that the least $R_0$ achieved is approximately 0.7 in Figure~\ref{fig:compare}(c). And we can further see the decreasing marginal effectiveness of the control strategies, e.g. with 80\% control for mode 2 in single center network, the effectiveness does not change at all if we increase the level of control for mode 1 from 40\% to 0\%. But most importantly, given the same level of control, there are clear differences of $R_0$ value if the urban structure is different. In general, the city with single center is more vulnerable to the invade of infectious diseases due to most activities are centered in the middle of the city, which is reflected by both highest $R_0$ and lowest $R_0$ possible in the figure. And without any intervention, the urban structure with multiple nodes tend to have the lowest $R_0$ of 1.0, while the value is $1.1$ for stripe-shaped and single center networks. 
\begin{figure}[htbp!]
	\centering
	\subfloat[Control over stripe-shaped city]{\includegraphics[width=90mm]{results/stripecityR0.eps}}
	\subfloat[Control over cities with single center]{\includegraphics[width=90mm]{results/singlecityR0.eps}}\\
	\subfloat[Control over cities with dual centers]{\includegraphics[width=90mm]{results/dualcityR0.eps}}
	\caption{Comparison of no-control scheme versus hybrid system setting}
	\label{fig:compare}
\end{figure}

% \subsection{Reachability analysis}

% We next discuss the impact of modeling parameters and their impacts on the accuracy and computation time of the constructed flowpipe over-approximation. In particular, we focus on the order of TMs and the precision of cut-off threshold, which are the two major factors that may affect the tightness of the estimation. 

% \begin{table}[htbp!]
% \centering
% \caption{Computational efficiency of the Taylor model approach with different parameter settings}
% \label{tab:cpu_time}
% \begin{tabular}{cccccc}
% \toprule
% Case & Network nodes & Dimension & Cut-off  & Taylor\_Order & Time per step(s) \\
% \midrule
% 1    & 4             & 64        & 1.00E-06 & 5             & 812.73           \\
% 2    & 4             & 64        & 1.00E-06 & 4             & 577.25           \\
% 3    & 4             & 64        & 1.00E-06 & 3             & 515.25           \\
% 4    & 4             & 64        & 1.00E-08 & 5             & 604.42           \\
% 5    & 4             & 64        & 1.00E-08 & 4             & 533.53           \\
% 6    & 4             & 64        & 1.00E-08 & 3             & 515.08           \\
% 7    & 4             & 64        & 1.00E-10 & 5             &  1939.09                \\
% 8    & 4             & 64        & 1.00E-10 & 4             & 493.98                 \\
% 9    & 4             & 64        & 1.00E-10 & 3             & 481.27          \\
% \bottomrule
% \end{tabular}
% \end{table}

% Table~\ref{tab:cpu_time} presents the computational time spent for the four-network which has 64 dimensions and state variables, and we vary the parameter setting to compare the resulting level of accuracy of the constructed flowpipes and the corresponding CPU time in seconds. In all cases, the symbolic remainder approach~\cite{chen2016decomposed} is adopted with the queue length equals to one-third of the total number of estimation steps, for the sake of reducing numerical errors due to wrapping effects. The 64-dimensional nonlinear ODE system is in general a huge system and often computational expensive to evaluate numerically, but our results suggest that the TM approach complete the over-approximation in an efficient manner, where the time required for computing each time step (corresponding to one day in our case) ranges from 480 to 813 seconds depending on the system parameter setting. That is, we may analyze the disease outbreaks and predict the flowpipe of the disease trend for upcoming 100 days in approximately 14 hours, which is a reasonable amount of time for any practical implementation considering its property of guaranteed safety. And this computation time may be significantly improved if the current sequential construction of TM model is extended to allow for parallelization to make more sufficient use of the computing power available.  

% \begin{figure}[htbp!]
% 	\centering  
% 	\subfloat[Cutoff threshold=10e-6, and vary TM from 3 to 5]{\includegraphics[width=80mm]{results/cut6_TM345.eps}}
% 	\subfloat[Cutoff threshold=10e-6, and vary TM from 3 to 5 (zoom)]{\includegraphics[width=80mm]{results/cut6_TM345_zoom.eps}}\\
% 	\subfloat[TM=4, and vary cutoff threshold from 10e-6 to 10e-10]{\includegraphics[width=80mm]{results/TM4_cut6810.eps}}
% 	\subfloat[TM=4, and vary cutoff threshold from 10e-6 to 10e-10(zoom)]{\includegraphics[width=80mm]{results/TM4_cut6810_zoom.eps}}\\
% 	\caption{Accuracy with different cutoff thresholds and Taylor model orders}
% 	\label{fig:tm_cut}
% \end{figure}

% Figure~\ref{fig:tm_cut} illustrates the impact of different TM orders and cutoff sizes on the tightness of the over-approximation results. Since the ODE system involves mostly bilinear terms, we start with TM order of 3 and cutoff size being 1e-6, and then increase the TM order and reduce the cutoff threshold to compare the gain over the level of accuracy versus the additional computation time spent. It is observed that by increasing TM order from 3 to 4, there is a notable improvement on the tightness of the over-approximation as shown in Figure~\ref{fig:tm_cut}(a)-(b). This suggests that TM order 3 may produce overly conservative results and a higher order is expected. If we further increase the TM order from 4 to 5, the gain is only minimal as compared to over 40\% increase in the computation time. These imply that TM order 4 is sufficient to obtain accurate results for the ODE system that we study. On the other hand, we fix TM order to 4 and investigate how the overapproximation results change with respect to the cutoff threshold. As shown in Figure~\ref{fig:tm_cut}(c)-(d), a large cutoff threshold (e.g., 10e-6) will lead to significantly overestimated upper and lower bounds. But if we reduce the cutoff threshold by 2 orders, we may obtain a very tight over-approximation, and the difference is hardly distinguishable if we use a even smaller cutoff threshold. These results suggest higher TM orders and smaller cutoff threshold will improve the tightness of the over-approximation, but the marginal gain may be diminishing rapidly. Consequently, TM order of 4 and cutoff threshold being 10e-8 would be one of the optimal parameter settings for the flowpipe construction of our ODE system. And similar evaluation approach may be adopted if the different ODE systems are investigated. 

% For Figure~\ref{fig:compare} (a)-(d), they show the reachable set when starting from the infected states, where the infected population $\in[0.18,0.2]$. It can be verified that the traffic control does help to eliminate the disease and reduce the spread of the disease. In particular, for $I_{11}$, it can be seen that at the end of the time interval the infected population is reduced to $[0.07,0.09]$, while for the no control case there is a clear sign of disease outbreak since there are 50\% more infected people. Similarly, for $I_{12}$, the control helps to reduce the infected population to less than $0.02$, and the overall trend is monotonically decreasing, but the no control case has a larger population of infectious people and the amount of infected people increases towards the end. As for $I_{33}$, it starts from the DFE state, and the no control case clearly shows the pattern of disease outbreak, while for the controlled system there are much fewer infected population. Also, the amount of infected people tends to decrease if we enlarge the time interval. 

% One key concern related to interval arithmetic approaches for over-approximating ODE systems is the wrapping effect. And it is practically inevitable that the TM may produce extra residuals due to overly wrapping the original system of equations at each time step, unless the ODE system itself is exactly the TM. Since the numerical residue may carry over to the calculations in following steps, a small wrapping residual may have bull-whip effect on the constructed over-approximating flowpipe. Since we have shown only the first 60 steps of the ODE system, readers may be curious to see if the over-approximation flowpipe may eventually explode as the time progresses. We investigate this issue numerically by comparing the constructed flowpipe with the results from the ODE simulator and evaluating the residual error $\bar{e_t}$ at each time step which is measured as:
% \begin{equation}
% \bar{e_t}=\frac{v_t^m-v_t'}{v_t'}
% \end{equation}
% where $v_t^m$ is the estimated upper bound of the ODE system from model $m$ (e.g., model with TM order 3 and cutoff threshold $10e-6$) at time $t$, and $v_t'$ is the estimated upper bound of the ODE system from the benchmark model. Since we shall never know the exact upper bound of the flowpipe, we need to specify the benchmark model which may produce highly tight estimation of the actually upper bound. In our numerical experiments, we set the benchmark model to the one with TM order 5 and cutoff threshold being $10e-10$, and compare all other models listed in in Table~\ref{tab:cpu_time}. The results are shown in Figure~\ref{fig:wrap_resid}. There are two important observations related to the results. First, as compared to the benchmark model, it can be seen that the error $\bar{e}$ increases rapidly in the first few time steps, but has a concave shape which eventually gets stabilized overtime. That is, while the rate of error is increasing initially, the error is shown to converge to a certain value as time progresses. The second observation is related to the value of such error. Since we consider a unit of population in our experiment, even an error of 1e-3 may lead to a difference of 10,000 infected people to an urban area with over 10 million population, which may render the plausibility of the over-approximation. From these experiments, it can be seen that for lower TM order and larger cutoff size, such error may be as high as 0.1 as compared to the base model, which is equivalent to around 7000 difference of infected population at the disease peak for 10 million population. By improving the order of TM and cutoff threshold, this error may be significantly reduced and may be as small as $e^{-8}$ in our case as compared to the base model, so that the difference is around 20 people at the disease peak. These imply that the residual errors due to wrapping effects are very well addressed with the TM approach and the resulting over-approximating flowpipe has high fidelity when it is applied to estimate the upper and lower bound of infected population size. 

% \begin{figure}[htbp!]
% 	\centering
% 	\includegraphics[width=120mm]{results/wrap_resid.eps}
% 	\caption{Evaluation of successive errors (in log scale) due to wrapping effect at each time step}
% 	\label{fig:wrap_resid}
% \end{figure}


% Finally, we compare the resulted over-approximation flowpipes with that generated from the ODE solvers in MATLAB. In particular, we choose the ode15s considering the stiff nature of the disease models, where a small change in parameter settings and initial conditions may result in very different system dynamics~\cite{dukic2012tracking}. A typical misconception regarding the numerical evaluation of the SEIR system is that the constructed trajectory via numerical solver may accurately represent the disease dynamics. However, in reality, we will never have the exact information on the initial condition of the disease pattern. Instead, the decision maker may only have a rough estimate of the total infected population at current time step, e.g., 100-200 people, and this initial interval will be projected into a wide range regarding the number of infected people at the disease peak. Under such circumstances, it may require infinite number of trajectories to be constructed by originating from the initial set. And the numerical solver also suffers from the remainder errors at each time step which will be accumulated towards the target value of estimation. As stated before, a small prediction error may result in a huge gap between the actual number of infected people versus the predicted value, not mentioning that there is no guarantee on the correctness of the solution from the numerical solver. On the contrary, the TM overapproximation ensures that the eventual state of disease is within the constructed flowpipe, thus the decision maker may clearly tell if the scale of the disease will be under control at certain time steps. We show the comparison of trajectories constructed by the ode15s with the TM flowpipe in Figure~\ref{fig:compare_ode15}. The initial set for the reachability analysis is a box, where we consider the total initial infected population is within the range $[0.002375,0.002625]$ and the initial set is box so that the total population still sums to one. And we simulated 100 and 500 trajectories using ode15s by starting from randomly selected points from the initial set. The computation time for each trajectory is 20.6 seconds for the 60 time steps, so that the flowpipe construction takes the time of approximately simulating 1450 trajectories. However, even simulating such many trajectories may only result in a biased understanding of the disease pattern, as we can seen from the gap between the trajectories and the shaded area, and that some trajectories are lied outside of the boundary of the constructed flowpipe. Therefore, we may falsely interpret the disease peak as well the time of the peak by simply using the numerical ode solvers. And this comparison clearly illustrates the necessary of flowpipe overapproximation for real-world applications of disease modeling in populated urban areas.

% \begin{figure}[htbp!]
% 	\centering  
% 	\subfloat[100 Trajectories from ODE15s and the shaded area of TM flowpipe]{\includegraphics[width=80mm]{results/100trajectories_stiff.eps}}
% 	\subfloat[100 Trajectories from ODE15s and the shaded area of TM flowpipe (zoom)]{\includegraphics[width=80mm]{results/100trajectories_stiff_zoom.eps}}\\
%     	\subfloat[500 Trajectories from ODE15s and the shaded area of TM flowpipe]{\includegraphics[width=80mm]{results/500trajectories_stiff.eps}}
% 	\subfloat[500 Trajectories from ODE15s and the shaded area of TM flowpipe (zoom)]{\includegraphics[width=80mm]{results/500trajectories_stiff_zoom.eps}}\\
% 	\caption{Accuracy with different cutoff thresholds and Taylor model orders}
% 	\label{fig:compare_ode15}
% \end{figure}


==> results.tex <==
\section{Results}

\subsection{Experiment setting}
The numerical experiments are conducted on a desktop with @3.5 GHz CPU and $32GB$ RAM. The codes are written in C++ and compiled with gcc in Linux system. The MPFR library is used for interval arithmetic and the Flow* library is used for doing TM flowpipe construction. The numerical experiments have three major parts. The first part is to compare the results on disease dynamics with and without modeling urban transportation system, including the difference in disease equilibrium patterns and the impact on $R_0$ values. The second part focuses on the performance of the reachability analysis, where the computational performances as well as the tightness of the overapproximation is discussed. Finally, we investigate how disease outbreaks evolution may vary based on different urban structures. For the first two parts, we mainly focus on the test network as shown in Figure~\ref{fig:smallnetwork}. The network has 3 nodes and 9 OD pairs, meaning that each node is accessible from the other. As each OD pair may have four states (S,E,I,R), the ODE system of this test network therefore has 36 state variables and 36 system equations. We consider the invasion of H1N1 influenza in 2009 as the case study for the test networks. According to the literature~\cite{tuite2010estimated}, the disease has the contact rate $\beta$ of $0.585$, $\gamma$ being $0.09$, and $\sigma$ being $0.47$, which suggests that H1N1 has an average latent period of 2 days and recovery time of 10 days. And based on the epidemic parameters, our objective is to compare how disease dynamics may vary in three different systems: the SEIR system without travel contagion, the SEIR system with travel contagion but no intervention strategies, and the SEIR system with travel contagion and entry control strategies. In particular, for the control strategies, we consider three different level of controls, namely the high level of control that may possibly eliminate 50\% of suspicious travelers from entering the system, the medium level of control that may eliminate 30\% of infected travelers, and the low control level where only 10\% of infectious population may be identified. And different control strategies may have different impact on the travel time for the corresponding travel modes. The third part of the experiment setting will focus on a different set of networks, as shown in Figure~\ref{fig:urbannetwork}. For this part, we consider networks that represent three different urban structures: the stripe-shaped network such as Shenzehen, China, the single-centered network including Paris and New York City, and the multi-centered networks (in this study we consider dual centers for simplicity) such as Beijing and Shanghai, China. And we analyze how effective are various control strategies in controlling these networks.

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=50mm]{results/network.png}
	\caption{Test network with 3 nodes}
	\label{fig:smallnetwork}
\end{figure}

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=150mm]{results/urban_network.png}
	\caption{Networks with three different urban structures}
	\label{fig:urbannetwork}
\end{figure}


\subsection{Case study: 2003 SARS outbreak in Beijing}
One major difficulty related to mathematical modeling of infectious diseases is the validity of the developed models. In general, it is not possible yet ethical to validate the fidelity of the model with field experiments. And in this study, we investigate the validity of our model by measuring the alignment of its predicted results with the real-world ground data during the 2003 Severe Acute Respiratory Syndrome (SARS) outbreak in Beijing, China.

The 2003 Beijing SARS outbreak is one of the few disease outbreaks within urban areas that has documented the daily progress of the disease pattern. There were 2523 probable cases of SARS reported from March 5, 2003 to May 29, 2003~\cite{pang2003evaluation}. Multiple control measures had been implemented during the outbreak, including the set up of dedicated SARS hospital, information dissemination of real-time SARS pattern, and the closing of public facilities. As for the transit system, surveillance sites had been set at the airport, major train stations, and 71 roads that connect Beijing to peripheral areas. The metro system improved its ventilation system, and more frequent and thorough disinfections were conducted for both metro compartments and buses. In addition, staffs of bus and metro systems had been trained to identify and take immediate actions against probable patients during travel.  

\begin{figure}[htbp!]
	\centering
	\subfloat[Disinfection of metro compartment taking place on April 21, 2003]{\includegraphics[width=75mm]{results/beijing_metro_disinfection.jpg}}  
	\subfloat[Body temperature screening at the train station]{\includegraphics[width=70mm]{results/beijing_temperature.jpg}}
	\caption{Measures were taken in mass transit systems to identify probable cases of SARS in Beijing}
	\label{fig:sars_measures}
\end{figure}

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=100mm]{results/peknet.pdf}
	\caption{The Beijing network with 5 nodes}
	\label{fig:beijing}
\end{figure}

To model the SARS outbreak, we first divide Beijing into 5 areas as shown in Figure~\ref{fig:beijing}. Among the 14 million population in Beijing by the end of 2003, 40\% of them reside inside the third ring road of Beijing (which corresponds to center area 3 in Figure~\ref{fig:beijing}). And we consider the rest 4 areas have similar population size, with each accounts for 15\% of total population of Beijing. Due to lack of daily commuting data in 2003, we assume that the 70\% of the activities for people living in area 3 are within area 3, and 40\% of the activities are within the same area for the other 4 areas. This gives the vector of departure rate $g=[0.6,0.6,0.3,0.6,0.6]$. For each OD pair, we consider the return rate being $0.9$. For residents of area 3 who leave the area for daily activities, we assume that they have equal chances to reach all other 4 areas. And for residents of area 1,2,4, and 5, we consider that they have 40\% of chance to visit area 3, and 20\% for other three places. Three transit modes are considered with capacity ranging from high to low, and the ratio of travel time for the same OD pair are set to 5:8:6. Considering various efforts made in mitigating disease spreading within transit system, we assume that the high capacity and medium capacity modes have 20\% probability for identifying the probable case during travel. For the disease parameters, the typical incubation time for SARS is reported to be within 2-7 days, with 3-5 days being most common~\cite{SARS_CDC}. Consequently, we set $\sigma=1/3$ for the case study. Different from the its typical definition, the recovery state R in this case study should refer to the state where an infectious individual or probable case of SARS is identified and isolated from the mass population. Due to the effectiveness of information dissemination and increasing alertness of people to SARS, it is reasonable to consider that any people with symptoms may get easily identified as long as they take part in any social activities. This value along with the infectious rate $\beta$ are usually identified through curve fitting from real-world data. The recovery rate is set to $0.6$ in our study, meaning that in 60\% of the cases the infectious individual will be identified and hospitalized. The infectious rate $\beta$ was reported to take values between $0.57$ to $1$ in various cases~\cite{colizza2007predictability,ng2003double}. But this value is temporally varying and is sensitive to the control measures being taken. In our study, we consider the infectious rate being $0.71$ for the entire population, and therefore the effective transmission rate per contact being $5.07e-8$. Based on the parameter setting, we constructed the epidemic model of 100 dimensions for 25 OD pairs and the results are simulated using ODE45 simulator in MATLAB, as shown in Figure~\ref{fig:case_sum} and Figure~\ref{fig:case_daily}.

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=100mm]{results/cum.eps}
	\caption{Cumulative SARS cases since April-20, 2013, Beijing, China}
	\label{fig:case_sum}
\end{figure}

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=100mm]{results/daily_increase.eps}
	\caption{Daily increases of SARS cases since April-20, 2013, Beijing, China}
	\label{fig:case_daily}
\end{figure}

We use the official data from Chinese Ministry of Health as the baseline observations, which gives the daily number of probable SARS cases starting from April 20, 2003 to June 12, 2003. While the number of infectious and latent population were unknown, we assume $E(0)=420, I(0)=223$, and $R(0)=210$, and these people are evenly distributed in all 5 areas, where the simulated results well match the statistics reported in the first day (April-20, 2003). It can be verified from the results that the simulated curve for the number of cumulative cases may well approximate the actual observations reported, especially within the first 15 days. Moreover, the total number of cases based on the simulation is 2745, which is only 8.8\% higher than the actual total cases. As for the daily number of cases, though the deterministic model may not be able to capture the stochasticity that takes place in the real-world, the simulated results still follow the trend similar to the actual observations. It provides a very good sense on how the disease may propagate over days with limited inputs, and the differences between simulation results and observations for daily increases is smaller than 15 cases in 47 out of the 65 days. In addition, if we only apply the conventional SEIR model in this case, the corresponding $R_0$ value is $0.71/0.6=1.183$, which implies that the disease will invade the entire population which is entirely different from the actual observations. On the other hand, if we match the the $R_0$ value of SEIR model with our proposed model ($R_0=0.836$ in this case), the limiting number of cases will become 3774 cases, which is significantly higher than the observed value. And the SEIR model may be able to give a closer estimation of 2472 cases only if we set $\gamma=0.97$, which implies that we are able to hospitalize the patients as soon as they get infected and such scenario is barely possible for any real-world disease outbreaks. Consequently, these results may well support the fidelity of our developed approach and reveal the potential of our model for predicting the propagation of disease outbreaks that take place in urban areas.

\subsection{The role of contagion within transportation system}

\begin{figure}[htbp!]
	\centering
	\subfloat[Disease A with $\beta=0.7$]{\includegraphics[width=80mm]{results/highinfect_I.eps}}
	\subfloat[Disease B with $\beta=0.25$]{\includegraphics[width=80mm]{results/lowinfect_I.eps}}
	\caption{Total infected population over time}
	\label{fig:disease_pattern_compare_I}
\end{figure}

We next assess the importance of modeling travel contagion during urban disease outbreaks. We mainly focus on comparing the results from three different models: the disease model without modeling travel contagion (MWOTC), the disease model that models travel contagion but no interventions introduced (MWTC), and the disease model that model travel contagion and considers control measures over traffic modes (MWTC-CM). Note that MWOTC ad MWTC are special cases of MWTC-CM, where MWTC-CM reduces to MWTC when the vector $d$ is set to unity, and the MWTC can be reduced to MWOTC by let $\beta_{tra}=0$. We investigate the differences in the disease dynamics among the three models from two aspects: the disease dynamics of different infectious diseases and the change of $R_0$ with respect to different diseases. The same network as in the 2003 Beijing SARS case study is used in this section. For simplicity, we set total population to be 1 instead of 4, and assume that at the beginning only patch 1 has infectious people that account for 1\% of the population, and all remaining people are in the susceptible state. 

We first present the propagation dynamics associated with highly infectious and lowly infectious diseases. We assume that the incubation period is 4 days, and the average time of recovery is 5 days. The highly infectious disease A has $\beta=0.7$ and the $\beta$ for lowly infectious disease B is 0.25. In addition, we consider $20\%$ of travel control effectiveness for both diseases. The results of total infected population of the entire urban area are presented in Figure~\ref{fig:disease_pattern_compare_I}. For disease A, the corresponding $R_0$ values for MWOTC,MWTC and MWTC-CM are 1.639, 2.013, and 1.834 respectively. And those of disease B are 1.051, 1.172, and 0.998. These two cases prove the correctness of our derivation of $R_0$, where the disease is endemic and persists in the population when $R_0>1$, and the system converges to the DFE state when $R_0<1$ (MWTC-CM for disease B). And in both cases, we observe that the equilibrium points are stable. 

As can be seen in both cases, without considering travel contagion, it is likely that we will underestimate the peak number of infected population and obtain a delayed prediction of the peak time. And such gaps are more obvious during the outbreak of the less infectious disease B. It is not difficult to interpret the higher peak of infected population, since by modeling travel contagion we are considering an additional layer of interactions between susceptible and infected people during their travels. And for the early arrival of the disease peak, it is due to the faster synchronization of disease pattern over the urban area with the help of travel contagion. This effect is illustrated in Figure~\ref{fig:disease_pattern_sync}, where the total number of infected people in each patch of the network is presented. At time step 0, the patch one start with 1\% of infected people and all other patches are free of disease. As time progresses, we observe the infected population of patch 1 first drops and then starts to increase. But the point where the change of gradient takes place is quite different in the two cases. Without travel contagion, the infected population in patch 1 starts to increase around time step 30, while the corresponding time step is around time step 15 if the travel contagion is modeled. In addition, since patch 1,2,4,and 5 have similar population size and travel pattern, we observe that their disease dynamics start to converge after the initial several steps. And model with travel contagion reaches this convergence earlier than without modeling travel contagion. All of these suggest the faster synchronization of disease pattern due to the existence of travel contagion. On the other hand, if we place control measures to our transit system to make it more invulnerable to infectious diseases, we are able to effectively reduce the peak size of the diseases, as well as the total number of infected people over the entire disease outbreak. But more importantly, it can be verified that by controlling the transit system through moderate efforts, it is possible to change the state of the disease from endemic to DFE, which results in the elimination of the disease overtime. This is especially meaningful for diseases such as influenza where people are paying less attention to due to comparatively insignificant consequences and we barely have effective measures for its eradication besides mass annual vaccination. 

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=150mm]{results/disease_synchronization.png}
	\caption{Total number of infected people in each patch}
	\label{fig:disease_pattern_sync}
\end{figure}

We next evaluate how the two key parameters $R_0$ and $R_\infty$ may differ in the three models with respect to different disease infectious rates, as shown in Figure~\ref{fig:r0}. It is known that $R_0=1$ is the threshold of disease invasion, and by modeling travel contagions, it is likely that the disease tends to be endemic while the result reported without travel contagion is disease free. And the gap between with and without travel contagion in $R_0$ tends to increase as $\beta$ increase, meaning that it is even more crucial to consider the travel contagion for diseases with higher transmission rate. Moreover, while disease pattern may change from DFE to equilibrium by considering travel contagion, a moderate control intervention (eliminating 20\% of infected population) may driver bring the disease back to the DFE state, as shown in Figure~\ref{fig:r0}(b). And the control strategy is increasingly effective as $\beta$ changes from 0.1 to 0.4, where we may reduce the total infected population during endemic by over 50\%. 

\begin{figure}[htbp!]
	\centering
	\subfloat[Change of $R_0$ with different $\beta$ values]{\includegraphics[width=80mm]{results/beta_R0.png}}
	\subfloat[Change of total infected population at equilibrium with different $\beta$ values]{\includegraphics[width=80mm]{results/w_versus_wo.png}}\\
	\caption{The change of $R_0$ by modeling urban travel}
	\label{fig:r0}
\end{figure}

Finally, we would like to evaluate how different control strategies may be effective under different urban structures. That is, the way people travel and get in contact may be different with different urban structures. We consider the three networks as introduced before, and vary control effectiveness for medium and high capacity modes, from 0\% to 100\% effective, and the results are shown in Figure~\ref{fig:compare}. There are clearly boundaries on the effectiveness of the controlling strategies, as increasing the effectiveness will add extra travel times thus driving travelers to other modes. Therefore, for the particular disease, we see that the least $R_0$ achieved is approximately 0.7 in Figure~\ref{fig:compare}(c). And we can further see the decreasing marginal effectiveness of the control strategies, e.g. with 80\% control for mode 2 in single center network, the effectiveness does not change at all if we increase the level of control for mode 1 from 40\% to 0\%. But most importantly, given the same level of control, there are clear differences of $R_0$ value if the urban structure is different. In general, the city with single center is more vulnerable to the invade of infectious diseases due to most activities are centered in the middle of the city, which is reflected by both highest $R_0$ and lowest $R_0$ possible in the figure. And without any intervention, the urban structure with multiple nodes tend to have the lowest $R_0$ of 1.0, while the value is $1.1$ for stripe-shaped and single center networks. 
\begin{figure}[htbp!]
	\centering
	\subfloat[Control over stripe-shaped city]{\includegraphics[width=90mm]{results/stripecityR0.eps}}
	\subfloat[Control over cities with single center]{\includegraphics[width=90mm]{results/singlecityR0.eps}}\\
	\subfloat[Control over cities with dual centers]{\includegraphics[width=90mm]{results/dualcityR0.eps}}
	\caption{Comparison of no-control scheme versus hybrid system setting}
	\label{fig:compare}
\end{figure}

% \subsection{Reachability analysis}

% We next discuss the impact of modeling parameters and their impacts on the accuracy and computation time of the constructed flowpipe over-approximation. In particular, we focus on the order of TMs and the precision of cut-off threshold, which are the two major factors that may affect the tightness of the estimation. 

% \begin{table}[htbp!]
% \centering
% \caption{Computational efficiency of the Taylor model approach with different parameter settings}
% \label{tab:cpu_time}
% \begin{tabular}{cccccc}
% \toprule
% Case & Network nodes & Dimension & Cut-off  & Taylor\_Order & Time per step(s) \\
% \midrule
% 1    & 4             & 64        & 1.00E-06 & 5             & 812.73           \\
% 2    & 4             & 64        & 1.00E-06 & 4             & 577.25           \\
% 3    & 4             & 64        & 1.00E-06 & 3             & 515.25           \\
% 4    & 4             & 64        & 1.00E-08 & 5             & 604.42           \\
% 5    & 4             & 64        & 1.00E-08 & 4             & 533.53           \\
% 6    & 4             & 64        & 1.00E-08 & 3             & 515.08           \\
% 7    & 4             & 64        & 1.00E-10 & 5             &  1939.09                \\
% 8    & 4             & 64        & 1.00E-10 & 4             & 493.98                 \\
% 9    & 4             & 64        & 1.00E-10 & 3             & 481.27          \\
% \bottomrule
% \end{tabular}
% \end{table}

% Table~\ref{tab:cpu_time} presents the computational time spent for the four-network which has 64 dimensions and state variables, and we vary the parameter setting to compare the resulting level of accuracy of the constructed flowpipes and the corresponding CPU time in seconds. In all cases, the symbolic remainder approach~\cite{chen2016decomposed} is adopted with the queue length equals to one-third of the total number of estimation steps, for the sake of reducing numerical errors due to wrapping effects. The 64-dimensional nonlinear ODE system is in general a huge system and often computational expensive to evaluate numerically, but our results suggest that the TM approach complete the over-approximation in an efficient manner, where the time required for computing each time step (corresponding to one day in our case) ranges from 480 to 813 seconds depending on the system parameter setting. That is, we may analyze the disease outbreaks and predict the flowpipe of the disease trend for upcoming 100 days in approximately 14 hours, which is a reasonable amount of time for any practical implementation considering its property of guaranteed safety. And this computation time may be significantly improved if the current sequential construction of TM model is extended to allow for parallelization to make more sufficient use of the computing power available.  

% \begin{figure}[htbp!]
% 	\centering  
% 	\subfloat[Cutoff threshold=10e-6, and vary TM from 3 to 5]{\includegraphics[width=80mm]{results/cut6_TM345.eps}}
% 	\subfloat[Cutoff threshold=10e-6, and vary TM from 3 to 5 (zoom)]{\includegraphics[width=80mm]{results/cut6_TM345_zoom.eps}}\\
% 	\subfloat[TM=4, and vary cutoff threshold from 10e-6 to 10e-10]{\includegraphics[width=80mm]{results/TM4_cut6810.eps}}
% 	\subfloat[TM=4, and vary cutoff threshold from 10e-6 to 10e-10(zoom)]{\includegraphics[width=80mm]{results/TM4_cut6810_zoom.eps}}\\
% 	\caption{Accuracy with different cutoff thresholds and Taylor model orders}
% 	\label{fig:tm_cut}
% \end{figure}

% Figure~\ref{fig:tm_cut} illustrates the impact of different TM orders and cutoff sizes on the tightness of the over-approximation results. Since the ODE system involves mostly bilinear terms, we start with TM order of 3 and cutoff size being 1e-6, and then increase the TM order and reduce the cutoff threshold to compare the gain over the level of accuracy versus the additional computation time spent. It is observed that by increasing TM order from 3 to 4, there is a notable improvement on the tightness of the over-approximation as shown in Figure~\ref{fig:tm_cut}(a)-(b). This suggests that TM order 3 may produce overly conservative results and a higher order is expected. If we further increase the TM order from 4 to 5, the gain is only minimal as compared to over 40\% increase in the computation time. These imply that TM order 4 is sufficient to obtain accurate results for the ODE system that we study. On the other hand, we fix TM order to 4 and investigate how the overapproximation results change with respect to the cutoff threshold. As shown in Figure~\ref{fig:tm_cut}(c)-(d), a large cutoff threshold (e.g., 10e-6) will lead to significantly overestimated upper and lower bounds. But if we reduce the cutoff threshold by 2 orders, we may obtain a very tight over-approximation, and the difference is hardly distinguishable if we use a even smaller cutoff threshold. These results suggest higher TM orders and smaller cutoff threshold will improve the tightness of the over-approximation, but the marginal gain may be diminishing rapidly. Consequently, TM order of 4 and cutoff threshold being 10e-8 would be one of the optimal parameter settings for the flowpipe construction of our ODE system. And similar evaluation approach may be adopted if the different ODE systems are investigated. 

% For Figure~\ref{fig:compare} (a)-(d), they show the reachable set when starting from the infected states, where the infected population $\in[0.18,0.2]$. It can be verified that the traffic control does help to eliminate the disease and reduce the spread of the disease. In particular, for $I_{11}$, it can be seen that at the end of the time interval the infected population is reduced to $[0.07,0.09]$, while for the no control case there is a clear sign of disease outbreak since there are 50\% more infected people. Similarly, for $I_{12}$, the control helps to reduce the infected population to less than $0.02$, and the overall trend is monotonically decreasing, but the no control case has a larger population of infectious people and the amount of infected people increases towards the end. As for $I_{33}$, it starts from the DFE state, and the no control case clearly shows the pattern of disease outbreak, while for the controlled system there are much fewer infected population. Also, the amount of infected people tends to decrease if we enlarge the time interval. 

% One key concern related to interval arithmetic approaches for over-approximating ODE systems is the wrapping effect. And it is practically inevitable that the TM may produce extra residuals due to overly wrapping the original system of equations at each time step, unless the ODE system itself is exactly the TM. Since the numerical residue may carry over to the calculations in following steps, a small wrapping residual may have bull-whip effect on the constructed over-approximating flowpipe. Since we have shown only the first 60 steps of the ODE system, readers may be curious to see if the over-approximation flowpipe may eventually explode as the time progresses. We investigate this issue numerically by comparing the constructed flowpipe with the results from the ODE simulator and evaluating the residual error $\bar{e_t}$ at each time step which is measured as:
% \begin{equation}
% \bar{e_t}=\frac{v_t^m-v_t'}{v_t'}
% \end{equation}
% where $v_t^m$ is the estimated upper bound of the ODE system from model $m$ (e.g., model with TM order 3 and cutoff threshold $10e-6$) at time $t$, and $v_t'$ is the estimated upper bound of the ODE system from the benchmark model. Since we shall never know the exact upper bound of the flowpipe, we need to specify the benchmark model which may produce highly tight estimation of the actually upper bound. In our numerical experiments, we set the benchmark model to the one with TM order 5 and cutoff threshold being $10e-10$, and compare all other models listed in in Table~\ref{tab:cpu_time}. The results are shown in Figure~\ref{fig:wrap_resid}. There are two important observations related to the results. First, as compared to the benchmark model, it can be seen that the error $\bar{e}$ increases rapidly in the first few time steps, but has a concave shape which eventually gets stabilized overtime. That is, while the rate of error is increasing initially, the error is shown to converge to a certain value as time progresses. The second observation is related to the value of such error. Since we consider a unit of population in our experiment, even an error of 1e-3 may lead to a difference of 10,000 infected people to an urban area with over 10 million population, which may render the plausibility of the over-approximation. From these experiments, it can be seen that for lower TM order and larger cutoff size, such error may be as high as 0.1 as compared to the base model, which is equivalent to around 7000 difference of infected population at the disease peak for 10 million population. By improving the order of TM and cutoff threshold, this error may be significantly reduced and may be as small as $e^{-8}$ in our case as compared to the base model, so that the difference is around 20 people at the disease peak. These imply that the residual errors due to wrapping effects are very well addressed with the TM approach and the resulting over-approximating flowpipe has high fidelity when it is applied to estimate the upper and lower bound of infected population size. 

% \begin{figure}[htbp!]
% 	\centering
% 	\includegraphics[width=120mm]{results/wrap_resid.eps}
% 	\caption{Evaluation of successive errors (in log scale) due to wrapping effect at each time step}
% 	\label{fig:wrap_resid}
% \end{figure}


% Finally, we compare the resulted over-approximation flowpipes with that generated from the ODE solvers in MATLAB. In particular, we choose the ode15s considering the stiff nature of the disease models, where a small change in parameter settings and initial conditions may result in very different system dynamics~\cite{dukic2012tracking}. A typical misconception regarding the numerical evaluation of the SEIR system is that the constructed trajectory via numerical solver may accurately represent the disease dynamics. However, in reality, we will never have the exact information on the initial condition of the disease pattern. Instead, the decision maker may only have a rough estimate of the total infected population at current time step, e.g., 100-200 people, and this initial interval will be projected into a wide range regarding the number of infected people at the disease peak. Under such circumstances, it may require infinite number of trajectories to be constructed by originating from the initial set. And the numerical solver also suffers from the remainder errors at each time step which will be accumulated towards the target value of estimation. As stated before, a small prediction error may result in a huge gap between the actual number of infected people versus the predicted value, not mentioning that there is no guarantee on the correctness of the solution from the numerical solver. On the contrary, the TM overapproximation ensures that the eventual state of disease is within the constructed flowpipe, thus the decision maker may clearly tell if the scale of the disease will be under control at certain time steps. We show the comparison of trajectories constructed by the ode15s with the TM flowpipe in Figure~\ref{fig:compare_ode15}. The initial set for the reachability analysis is a box, where we consider the total initial infected population is within the range $[0.002375,0.002625]$ and the initial set is box so that the total population still sums to one. And we simulated 100 and 500 trajectories using ode15s by starting from randomly selected points from the initial set. The computation time for each trajectory is 20.6 seconds for the 60 time steps, so that the flowpipe construction takes the time of approximately simulating 1450 trajectories. However, even simulating such many trajectories may only result in a biased understanding of the disease pattern, as we can seen from the gap between the trajectories and the shaded area, and that some trajectories are lied outside of the boundary of the constructed flowpipe. Therefore, we may falsely interpret the disease peak as well the time of the peak by simply using the numerical ode solvers. And this comparison clearly illustrates the necessary of flowpipe overapproximation for real-world applications of disease modeling in populated urban areas.

% \begin{figure}[htbp!]
% 	\centering  
% 	\subfloat[100 Trajectories from ODE15s and the shaded area of TM flowpipe]{\includegraphics[width=80mm]{results/100trajectories_stiff.eps}}
% 	\subfloat[100 Trajectories from ODE15s and the shaded area of TM flowpipe (zoom)]{\includegraphics[width=80mm]{results/100trajectories_stiff_zoom.eps}}\\
%     	\subfloat[500 Trajectories from ODE15s and the shaded area of TM flowpipe]{\includegraphics[width=80mm]{results/500trajectories_stiff.eps}}
% 	\subfloat[500 Trajectories from ODE15s and the shaded area of TM flowpipe (zoom)]{\includegraphics[width=80mm]{results/500trajectories_stiff_zoom.eps}}\\
% 	\caption{Accuracy with different cutoff thresholds and Taylor model orders}
% 	\label{fig:compare_ode15}
% \end{figure}

